Logical Characterization of Coherent Uninterpreted Programs

An uninterpreted program (UP) is a program whose semantics is defined over the theory of uninterpreted functions. This is a common abstraction used in equivalence checking, compiler optimization, and program verification. While simple, the model is sufficiently powerful to encode counter automata, and, hence, undecidable. Recently, a class of UP programs, called coherent, has been proposed and shown to be decidable. We provide an alternative, logical characterization, of this result. Specifically, we show that every coherent program is bisimilar to a finite state system. Moreover, an inductive invariant of a coherent program is representable by a formula whose terms are of depth at most 1. We also show that the original proof, via automata, only applies to programs over unary uninterpreted functions. While this work is purely theoretical, it suggests a novel abstraction that is complete for coherent programs but can be soundly used on arbitrary uninterpreted (and partially interpreted) programs.

==> abstraction-background.tex <==
\subsection{Abstractions}

We may verify properties of transition systems by considering their abstractions.
An abstraction function that abstracts the configurations of a program induces an abstract transition system in which 
each abstract transition corresponds to a concrete transition followed by applying the abstraction on the resulting configuration.
The formal definition follows.
\sharon{do we want to say that the abstractions leave the program statement $s$ and the state $q$ intact, but abstract the path condition.
It is not needed now, but it may let us state more things generally -- need to check}

\begin{definition}
\label{def:abstract-TS-general}
Given a transition system $\TS = (\Conf, \initconf,\Tr)$
and a (possibly partial) abstraction function $\genAbs: \Conf \to \Conf$, the corresponding \emph{abstract transition system} 
is $\TSGenAbs = (\Conf, \initconfGenAbs, \TrGenAbs)$, where
\begin{itemize}
\item $\initconfGenAbs = \genAbs(\initconf)$
\item  $\TrGenAbs = \{(c,c') \mid \exists \tilde{c}.~c \to \tilde{c}~\land~c' = \genAbs(\tilde{c}) \}$
\end{itemize}
We write $c \toGenAbs c'$ when $(c,c') \in \TrGenAbs$. While $\genAbs$ may be a partial function,
we require that it is defined for $\initconf$.
\end{definition}

%In the sequel we consider several abstraction functions and discuss their properties.
%\sharon{I want to revise this to mention $\equiv_\sharp$}
%%Each abstraction preserves a certain class of EUF properties that are true in the configuration.
%%We denote by $\equiv_\sharp$
%In all cases, the resulting abstract transition systems simulate the concrete transition system.
%In the interesting cases, the abstract and the concrete transition systems are in fact bisimilar.
%Simulation and bisimulation ensure that temporal properties are preserved from the abstract transition system
%to the concrete transition system, where the basis ensures that properties of configurations are preserved.
%The definition therefore assumes an equivalence relation $\equiv$ (for bisimulation),
%respectively a preorder $\leq$ (for simulation), between configurations, which we will define later.
%%We therefore first define a partial order and an equivalence relation between configurations which capture properties that are preserved between them.
%\sharon{I don't know if talking about equiv and pre-order is really needed, but this is the analogue to the req that the atomic propositions agree}

Weak, respectively strong, preservation of properties between the abstract and the concrete transition systems 
are ensured by the notions of \emph{simulation}, respectively \emph{bisimulation}.

\begin{definition}[\cite{DBLP:books/daglib/0067019}]
Let $\TS = (\Conf, \initconf, \Tr)$ and $\TSGenAbs = (\Conf, \initconfGenAbs, \TrGenAbs)$
be transition systems. A relation  $B \subseteq \Conf \times \Conf$ is a \emph{simulation} from $\TS$ to $\TSGenAbs$,
if for every $(c,c_\sharp) \in B$:
\begin{itemize}
\item if $c \to c'$ then there exists $c_\sharp'$ such that $c_\sharp \toGenAbs c_\sharp'$ and $(c',c_\sharp') \in B$.
\end{itemize}
$B \subseteq \Conf \times \Conf$ is a \emph{bisimulation} from $\TS$ to $\TSGenAbs$ if 
$B$ is a simulation from $\TS$ to $\TSGenAbs$ and 
$B^{-1}\eqdef \{(c_\sharp,c) \mid (c,c_\sharp) \in B \}$ is a simulation from $\TSGenAbs$ to $\TS$. 
We say that $\TSGenAbs$ \emph{simulates}, respectively \emph{is bisimilar to}, $\TS$ if there exists
a simulation, respectively, a bisimulation, $B$ from $\TS$ to $\TSGenAbs$ such that $(\initconf, \initconfGenAbs) \in B$.
\end{definition}
\hg{Why do we need $\toGenAbs$? From definition 2, it seemed like $\to$ is enough. }


==> abstraction.tex <==
\section{Abstraction}
Given a symbolic state $q$, we define the \emph{store set}, denoted $\strset_q$, as the set of constants stored in $q$:
\[
\strset_q = \{ X \mid \exists v \cdot q[v] = X \}    
\]
Note that the elements of the store set are always constants because we always use a fresh constant in assignment statements. 

Given a program configuration $\langle\mathunderscore, q, pc \rangle$, we denote the set of equalities that hold between the elements of stored set using $E_{\langle q, pc \rangle}$:
\[
E_{\langle q, pc \rangle} =  \{ (t_1, t_2) \mid pc \models (t_1 = t_2) \text{ and } t_1, t_2 \in \strset_q \}
\]
Note that $E_{\langle q, pc \rangle}$ is a finite set and can be represented as a conjunction of literals. Similarly, we denote the set of inequalities that hold between the elements of the stored set using $D_{\langle q, pc \rangle}$:
\[
D_{\langle q, pc \rangle} =  \{ (t_1, t_2) \mid pc \models (t_1 \neq t_2) \text{ and } t_1, t_2 \in \strset_q \}
\]

We define the store set abstraction of path condition as $\alpha(q, pc) = E_{\langle q, pc \rangle} \wedge D_{\langle q, pc \rangle}$. We omit $q$ and write $\alpha(pc)$ when $q$ is obvious from context.
\begin{lemma}
Given a configuration $\langle \mathbf{assume}(x = y), q, pc \rangle$ in a coherent program, where $pc$ is satisfiable, $q[x] = X$, and $q[y] = Y$. $pc \wedge X = Y$ is unsatisfiable if and only if $\alpha(pc) \wedge X = Y$ is unsatisfiable.
\end{lemma}
\begin{proof}
\textbf{only if direction} Since all the literals in $E_{\langle q, pc \rangle} \wedge D_{\langle q, pc \rangle}$ are implied by $pc$, if the abstraction is unsatisfiable, so is $pc$.

\textbf{if direction} Since $pc \wedge X = Y$ is unsatisfiable, $pc \models X \neq Y$. Therefore $D_{\langle q, pc \rangle} \models X \neq Y$. Hence $D_{\langle q, pc \rangle} \wedge X = Y$ will also be unsatsifiable.
\iffalse
\textbf{if direction} Let $pc \wedge X = Y \models t_j = t_k$ as well as $pc \wedge X = Y \models t_j \neq t_k$. Since $pc$ by itself is satisfiable, it has to be case that $t_j, t_k$ are superterms of $X, Y$ modulo $pc$. By the early assumes property, there are constants $J, K \in \strset_q$ such that $pc \models J = t_j$ and $pc \models K = t_k$. Hence $pc \models J = K$. Therefore $E_{\langle q, pc \rangle} \models J = K$. By the same argument, $D_{\langle q, pc \rangle}\models J \neq K$. Hence the abstraction is also unsatisfiable.  
\fi
\end{proof}

\begin{lemma}
Given a configuration $\langle \mathbf{assume}(x \neq y), q, pc \rangle$ in a coherent program, where $pc$ is satisfiable, $q[x] = X$, and $q[y] = Y$. $(pc \land X \neq Y)$ is unsatisfiable if and only if $\alpha(pc) \wedge X\neq Y)$ is unsatisfiable.
\end{lemma}
\begin{proof}
\textbf{only if direction} Since all the literals in $E_{\langle q, pc \rangle} \wedge D_{\langle q, pc \rangle}$ are implied by $pc$, if the abstraction is unsatisfiable, so is $pc$.

\textbf{if direction} Since $pc \wedge X \neq Y$ is unsatisfiable, $pc \models X = Y$. Therefore $E_{\langle q, pc \rangle} \models X = Y$. Hence $E_{\langle q, pc \rangle} \wedge X \neq Y$ will also be unsatsifiable.
\end{proof}

\begin{theorem}
Given a coherent program, any program configuration $\langle \mathunderscore, q, pc \rangle$ is feasible if and only if $\alpha(pc)$ is satisfiable.
\end{theorem}

The abstraction did not make use of any property of coherant programs. The benefit of coherant programs is that we can keep track of this abstraction using simple abstract transformers.

\iffalse
\begin{example}
Consider the coherent program 
\[ 
\begin{array}{ll}
1.&\mathbf{assume}(x = y);\\
2.&x := f(p, x);\\
3.&y := f(q, y);\\
4.&\mathbf{assume}(p = q);\\
5.&\mathbf{assume}(x \neq y);
\end{array}
\]
The symbolic state after each line of execution is
\[ 
\begin{array}{ll}
1.&\langle [x: X_0,  y: Y_0, p: P_0, q: Q_0], X_0 = Y_0\rangle\\
2.&\langle [x: X_1,  y: Y_0, p: P_0, q: Q_0], pc_1 \wedge X_1 = f(P_0, X_0)\rangle\\
3.&\langle [x: X_1,  y: Y_1, p: P_0, q: Q_0], pc_2 \wedge Y_1 = f(Q_0, Y_0)\rangle\\
4.&\langle q_3, pc_3 \wedge P_0 = Q_0\rangle\\
5.&\langle q_3, pc_4 \wedge X_1 \neq Y_1 \rangle
\end{array}
\]
abstracting each state gives us
\[ 
\begin{array}{ll}
1.&\langle [x: X_0, y: Y_0, p: P_0, q: Q_0], X_0 = Y_0\rangle\\
2.&\langle [x: X_1,  y: Y_0, p: P_0, q: Q_0], X_1 = f(P_0, Y_0)\rangle\\
3.&\langle [x: X_1,  y: Y_1, p: P_0, q: Q_0], X_1 = f(P_0, Y_0) \wedge Y_1 = f(Q_0, Y_0)\rangle\\
4.&\langle q_3,P_0 = Q_0 \wedge X_1 = X_2 \wedge X_1 = f(P_0, Y_0) \wedge Y_1 = f(Q_0, Y_0) \rangle\\
5.&\langle q_3, \bot \rangle
\end{array}
\]
Arie: abstracting each state gives us
\[ 
\begin{array}{ll}
1.&\langle [y_1 \to \hat{Y}_1,  y_2 \to \hat{Y}_2, x_1 \to \hat{X}_1, x_2 \to \hat{X}_2], \hat{Y}_1 = \hat{Y}_2\rangle\\
2.&\langle [y_1 \rightarrow Y_1,  y_2 \rightarrow \hat{Y}_2, x_1 \to \hat{X}_1, x_2 \to \hat{X}_2 ], Y_1 = f(\hat{X}_1, \hat{Y}_2)\rangle\\
3.&\langle [y_1 \rightarrow Y_1,  y_2 \rightarrow Y_2, x_1 \to \hat{X}_1, x_2 \to \hat{X}_2 ], Y_1 = f(\hat{X}_1, \hat{Y}_2) \wedge Y_2 = f(\hat{X}_2, \hat{Y}_2)\rangle\\
4.&\langle q_3,\hat{X}_1 = \hat{X}_2 \wedge Y_1 = Y_2 \wedge Y_1 = f(\hat{X}_1, \hat{Y}_2) \wedge Y_2 = f(\hat{X}_2, \hat{Y}_2)\rangle\\
5.&\langle q_3, \bot \rangle
\end{array}
\]
Abstract state 3 is wrong according to the definition of $\strset_q$.
\end{example}

Given a program configuration $\langle s, q, pc\rangle$, we define the \emph{stored set abstraction} as the abstract state $\langle s, q, E_{\langle q, pc \rangle} \wedge D_{\langle q, pc \rangle}\rangle$. The abstraction can be extended to terminal configurations in the same way. To define the abstract semantics of a program, we change the semantics of the assume and assignment statement to:
\[
\begin{array}{c}
     \infer{\langle \mathbf{assume}(c), q, pc \rangle \to \langle q, E_{\langle q, pc'\rangle} \wedge D_{\langle q, pc'\rangle}\rangle}{\langle c, q\rangle\Downarrow v\quad pc' = pc \wedge v}\\[1ex]
     \infer{\langle x := e, q, pc \rangle \to \langle q', E_{\langle q', pc'\rangle } \wedge D_{\langle q', pc'\rangle}\rangle}{\langle e, q\rangle \Downarrow v \quad \text{X is fresh} \quad q' = q[x \mapsto X] \quad pc' = pc \wedge X = v}\\[1ex]
\end{array}
\]

\begin{theorem}
A coherant program is safe if and only if it is safe relative to abstract semantics.
\end{theorem}
assume(x = y)
[x = X0, y = Y0], X0 = Y0

x := f(x)
[x = X1, y = Y0], X0 = Y0 && X1 = f(X0)
[x = X0, y = Y0], X0 = f(Y0)


y := f(y)
[x = X1, y = Y1], X0 = Y0 && X1 = f(X0) && Y1 = f(Y0)
[x = X0, y = Y0], Y0 = X0

x := f(x)
[x = X2, y = Y1], X0 = Y0 && X1 = f(X0) && X2 = f(X1) && Y1 = f(Y0)
[x = X2, y = Y1], X2 = f(Y1)



y := f(y)
[x = X2, y = Y2], X0 = Y0 && X1 = f(X0) && X2 = f(X1)
                          && Y1 = f(Y0) && Y2 = f(Y1)
pc_{abs} = abs(\cong_{pc})                    
[x = X0, y = Y0], Y0 = X0


assume(x != y)
[x = X2, y = Y2], X0 = Y0 && X1 = f(X0) && X2 = f(X1) 
                          && Y1 = f(Y0) && Y2 = f(Y1) 
                          && Y2 != X2
                          
[x = X0, y = Y0], Y0 = X0 && X0 != Y0
\fi

==> abstraction2.tex <==
\section{Store set abstraction}
Given a symbolic state $q$, we define the \emph{store set}, denoted $\strset_q$, as the set of constants stored in $q$:
\[
\strset_q = \{ X \mid \exists v \cdot q[v] = X \}    
\]
Note that the elements of the store set are always constants because we always use a fresh constant in assignment statements. 

Given a conjunction of literals $pc$ and a set of constants $V$, we define the \emph{store set} abstraction of $pc$, denoted $\alpha(pc)$, as the strongest subterm closed subset of $pc^*$ such that $V \cap \terms(\alpha(pc)) = V \cap pc$. 

\begin{lemma}
For a coherant program $P$, let $\langle \mathbf{assume}(x = y), q, pc \rangle$ be a reachable configuration such that $pc$ is satisfiable, $q[x] = X$, and $q[y] = Y$. Then $pc \wedge X = Y$ is unsatisfiable if and only if $\alpha(pc) \wedge X = Y$ is unsatisfiable.
\end{lemma}
\begin{proof}
\textbf{only if direction} Since all the literals in $\alpha(pc)$ are implied by $pc$, if the abstraction is unsatisfiable, so is $pc$.

\textbf{if direction} We know that congruence closure is complete for EUF~\cite{DBLP:conf/ijcai/Shostak77}. Let $cc(S)$ denote the congruence closure of $S$ as defined in~\cite{DBLP:conf/ijcai/Shostak77}.

If $pc \wedge X = Y$ is unsatisfiable, its either the case that $X \neq Y \in pc$ or $t_j = t_k \in cc(pc \wedge X = Y)$ and $t_j \neq t_k \in pc$. Here $t_j$ has to be a superterm of $X$ modulo $pc$ and $t_k$ has to be a superterm of $Y$ modulo $pc$. If this were not the case, $t_j = t_k \in cc(pc)$ and therefore $pc$ would be unsatisfiable. 

We prove the lemma by doing an induction on the number of times the congruence axiom is applied. We prove that all the literals used to derive $t_j = t_k$ are in $\alpha(pc)$. The base case is when $X \neq Y \in pc$. In this scenario, it holds that $X \neq Y \in \alpha(pc)$. To prove the inductive step, assume that all literals required to derive $u_j = v_j$ are in $\alpha(pc)$, forall $1 \leq j \leq n$, and that we need to apply the congruence axiom to prove that $f(u_1, \ldots, u_n) = f(v_1,\ldots, v_n)$. Since $f(u_1, \ldots, u_n)$ and $f(v_1,\ldots,v_n)$ are superterms of $X,Y$ modulo $pc$, by the early assumes property, $pc$ should contain equalities $U = f(u_1, \ldots, u_n)$ and $V = f(v_1,\ldots,v_n)$ where $U,V \in S_q$. Hence $f(u_1, \ldots, u_n), (v_1,\ldots,v_n) \in \alpha(pc)$. Therefore, $\alpha(pc) \wedge X = Y \models t_j = t_k$ and is unsatisfiable.
\end{proof}
\begin{lemma}
For a coherant program $P$, let $\langle \mathbf{assume}(x \neq y), q, pc \rangle$ be a reachable configuration such that $pc$ is satisfiable, $q[x] = X$, and $q[y] = Y$. Then $pc \wedge X \neq Y$ is unsatisfiable if and only if $\alpha(pc) \wedge X \neq Y$ is unsatisfiable.
\end{lemma}
\begin{proof}
The only way to derive false is that $pc \models X \eq Y$. Since $X$ and $Y$ are constants, this is possible only if either $X = Y \in pc$ or $X = f(u_1,\ldots, u_n) \in pc$, $Y = f(v_1,\ldots, v_n) \in pc$ and $pc \models u_i = v_i$ for all $i$. In the first case, $\alpha(pc)$ should also conatain the equality $X = Y$. In the second case, since $\alpha(pc)$ is subterm closed, $u_i = v_i \in \alpha(pc)$. Therefore $\alpha(pc) \models X = Y$ in both cases.  
\end{proof}
\begin{theorem}
For a coherant program $P$, let $\langle s, q, pc \rangle$ be a reachable configuration such that $pc$ is satisfiable. Then $pc \wedge c$ is unsatisfiable if and only if $\alpha(pc) \wedge c$ is unsatisfiable.
\end{theorem}

==> abstransformer.tex <==
\section{Abstract transformer}
We define the \emph{superterm set}, denoted $\suptermset_q$, as union of $\strset_q$ and any superterms that can be constructed from it:
\[
\suptermset_q = \strset_q \cup \{ f(t_1, \ldots, t_n) \mid \exists i \cdot t_i \in \strset_q\text{ and } f, t_1, \ldots, t_n \in \terms(\Sigma)\}
\]
%\sharon{need to be more precise. here it looks like you only allow one application of $f$. do you mean any number of nested applications? (otherwise the set is finite, but then why is the set of equalities infinite? also, what about other arguments of $f$?}
Note that the terms $t_i$ can be \emph{any} terms including applications of $f$.

Given a program configuration $\langle\mathunderscore, q, pc \rangle$, we denote the set of equalities that hold between the elements of the superterm set of $q$ using $E_{\langle q, pc \rangle}$:
\[
E^\uparrow_{\langle q, pc \rangle} =  \{ (t_1, t_2) \mid pc \models (t_1 = t_2) \text{ and } t_1, t_2 \in \suptermset_q \}
\]
Note that $E^\uparrow_{\langle q, pc \rangle}$ may be infinite. \hg{WHY CAN WE WRITE IT DOWN AS FORMULAS?\cite{DBLP:conf/cade/BachmairT00}}.
Similarly, we denote the set of inequalities that hold between the elements of the superterm set using $D_{\langle q, pc \rangle}$:
\[
D^\uparrow_{\langle q, pc \rangle} =  \{ (t_1, t_2) \mid pc \models (t_1 \neq t_2) \text{ and } t_1, t_2 \in \suptermset_q \}
\]
Now we define \emph{superterm abstract semantics} of a program by changing the semantics of the assume and assignment statement to:
\[
\begin{array}{c}
     \infer{\langle \mathbf{assume}(c), q, pc \rangle \to \langle q, E^\uparrow_{\langle q, pc'\rangle} \wedge D^\uparrow_{\langle q, pc'\rangle}\rangle}{\langle c, q\rangle\Downarrow v\quad pc' = pc \wedge v}\\[1ex]
     \infer{\langle x := e, q, pc \rangle \to \langle q', E^\uparrow_{\langle q', pc'\rangle } \wedge D^\uparrow_{\langle q', pc'\rangle}\rangle}{\langle e, q\rangle \Downarrow v \quad \text{X is fresh} \quad q' = q[x \mapsto X] \quad pc' = pc \wedge X = v}
\end{array}
\]

\begin{example}
Consider the coherent program
\[
\begin{array}{ll}
1.&\mathbf{assume}(x = y);\\
2.&x := f(p, x);\\
3.&y := f(q, y);\\
4.&\mathbf{assume}(p = q);\\ % at this point, postcondition is  X1 == f(P0, W_X_F_1) && Y1 == f(Q0, W_X_F_1) ;; (oldState) && (forall W :: \neg newStates )
% P0 == Q0 ==> X1 == Y1
% from Cesare, we know that interpolant in EUF is Horn clauses of the form (/\ EQ ==> EQ)
% if all function symbols are unary, then the interpolant is of the form (/\ EQ) over shared signature
% in UP paper, all function symbols in all examples are unary (n(x))
% 
5.&\mathbf{assume}(x \neq y);
\end{array}
\]
The symbolic state after each line of execution is
\[
\begin{array}{ll}
1.&\langle [x: X_0,  y: Y_0, p: P_0, q: Q_0], X_0 = Y_0\rangle\\
2.&\langle [x: X_1,  y: Y_0, p: P_0, q: Q_0], pc_1 \wedge X_1 = f(P_0, X_0)\rangle\\
3.&\langle [x: X_1,  y: Y_1, p: P_0, q: Q_0], pc_2 \wedge Y_1 = f(Q_0, Y_0)\rangle\\
4.&\langle q_3, pc_3 \wedge P_0 = Q_0\rangle\\
5.&\langle q_3, pc_4 \wedge X_1 \neq Y_1 \rangle
\end{array}
\]
The execution according to superterm abstract semantics is 
\[
\begin{array}{ll}
1.&\langle [x: X_0, y: Y_0, p: P_0, q: Q_0], X_0 = Y_0\rangle\\
2.&\langle [x: X_1,  y: Y_0, p: P_0, q: Q_0], X_1 = f(P_0, Y_0)\rangle\\
3.&\langle [x: X_1,  y: Y_1, p: P_0, q: Q_0], X_1 = f(P_0, Y_0) \wedge Y_1 = f(Q_0, Y_0)\rangle\\
4.&\langle q_3,P_0 = Q_0 \wedge X_1 = X_2 \wedge X_1 = f(P_0, Y_0) \wedge Y_1 = f(Q_0, Y_0) \rangle\\
5.&\langle q_3, \bot \rangle
\end{array}
\]
\end{example}

\begin{theorem}
A coherent program is safe according to the concrete semantics if and only if it is safe according to the superterm abstract semantics.
\end{theorem}
\begin{proof}
%\sharon{didn't check. def of abstraction is missing. why is it enough to look at the corresponding abstract configuration? (or in other words, what does "corresponding" mean here)}
The abstraction does not change either the structure of derivation trees or symbolic state. The only possibility is that some configurations are feasible in one semantics but not in the other. Since we have restricted the conditionals of assumes to be equalities or inequalities over program variables, we do not require path conditions in both semantics to be equivalent to preserve safety. Instead, all we have to prove is that, given a concrete program configuration $\langle s, q, pc_c\rangle$ and the corresponding abstract program configuration $\langle s, q, pc_a\rangle$, $pc_c \models \ell$ iff $pc_a \models \ell$ where $\ell = q[v_1] \sim q[v_2]$, $\sim$ is either $=$ or $\neq$.

Let $pc_c, pc_a$ be the path conditions before a rule is applied and let $pc_c'. pc_a'$ be the path conditions after the rule is applied. For each rule, we assume that $pc_c \models \ell$ iff $pc_a \models \ell$ and show that $pc_c' \models \ell$ iff $pc_a' \models \ell$.

Under our assumption, it holds that $pc_a' \models \ell$ then $pc_c' \models \ell$.  This is because, for all literals $c$ in $pc_a'\setminus pc_a$ it holds that $pc_c' \models c$.

To prove the other direction, we examine each changed rule individually:
\paragraph{assignment} 
\[
\begin{array}{c}
      \infer{\langle x := e, q, pc_c \rangle \to \langle q', pc_c'\rangle}{\langle e, q\rangle \Downarrow v \quad \text{X is fresh}\quad q' = q[x \mapsto X] \quad pc_c' = pc_c \wedge X = v} \\[1ex]
  \infer{\langle x := e, q, pc_a \rangle \to \langle q', pc_a'\rangle}{\langle e, q\rangle \Downarrow v \quad \text{X is fresh} \quad q' = q[x \mapsto X]\quad pc_a^1 = pc_a \wedge X = v \\[1ex]\hfill pc_a' = E_{\langle q', pc_a^1\rangle } \wedge D_{\langle  q', pc_a^1\rangle}}
\end{array}
\]
Since the constant $X$ is fresh, the only new equalities implied by $pc_c'$ are of the form $X = t$ where $t \in \terms(pc_c)$ and $pc_c \models t = v$. By the memoizing property, it holds that there exists a variable $v$ such that $pc_c \models t = q[v]$. Hence $pc_a' \models X = t$.
\paragraph{assume(x = y)} Let $q[x] = X$ and $q[y] = Y$. Let $s_X, s_Y$ be superterms of $X, Y$ in $pc_c$. By the early assumes property, both $s_X$ and $s_Y$ are stored in variables. Let $c$ be a literal implied by $pc_c'$ by not by $pc_c$. $c$ has to be of the form $f(\ldots, s_X, \ldots) = f(\ldots, s_Y, \ldots)$. Since both of these terms are in $\suptermset_q$, $pc_a' \models c$
\end{proof} 

==> background.tex <==
\section{Background}
\label{sec:background}

We assume that the reader is familiar with the basics of First Order Logic
(FOL), and the theory of Equality and Uninterpreted Functions (EUF). We use
$\Sigma = (\consts, \funs, \{\eq, \deq\})$ to denote a FOL signature with
constants $\consts$, functions $\funs$, and predicates $\{\eq, \deq\}$,
representing equality and disequality, respectively. A term is a constant or
(well-formed) application of a function to terms. A literal is either $x \eq y$
or $x \deq y$, where $x$ and $y$ are terms. A formula is a Boolean combination
of literals. We assume that all formulas are in Negation Normal Form (NNF), so
negation is defined as a shorthand: $\neg (x \eq y) \eqdef x \deq y$, and $\neg
(x \deq y) \eqdef x \eq y$. Throughout the paper, we use $\bowtie$ to indicate a
predicate in $\{\eq, \deq\}$. For example, $\{x \bowtie y\}$ means $\{x \eq y, x
\deq y\}$. We write $\bot$ for false, and $\top$ for true.

We do not differentiate between sets of literals $\Gamma$ and their conjunction
$(\bigwedge \Gamma)$. We write $\depth(t)$ for the maximal depth of function
applications in a term $t$:
\[\depth(t) = \begin{cases}
    0  & \text{if $t \in \consts$}\\
    1 + \max_i(\depth(t_i)) & \text{if $t = f(t_0, \ldots, t_k)$}
  \end{cases}
\]

We write $\terms(\varphi)$, $\consts(\varphi)$, and $\funs(\varphi)$ for the set
of all terms, constants, and functions, in $\varphi$, respectively, where
$\varphi$ is either a formula or a collection of formulas

\newcommand{\peuf}{\mathcal{P}_{\euf}}

For a literal $\ell$, we write $\Gamma \models \ell$ if $\Gamma$ \emph{entails}
$\ell$. We use a proof system $\peuf$ for EUF shown in Fig.~\ref{fig:peuf}. The
$\textsc{Refl}$ ensures that the only new terms introduced by a derivation are
constructed from some existing terms in $\Gamma$. We write $\Gamma \vdash \ell$,
pronounced $\ell$ is \emph{derived} from $\Gamma$, if a literal $\ell$ is
derivable from $\Gamma$ by $\mathcal{P}_{\euf}$. %
A deductive (\euf) closure, $\Gamma^*$, of a set of literals $\Gamma$ is defined
as: $\Gamma^* \eqdef \{\ell \mid \Gamma \vdash \ell\}$. % A set $\Gamma$ is
% deductively closed if $\Gamma = \Gamma^*$.
%
By refutational completeness of $\peuf$, $\Gamma$ is unsatisfiable
iff $\Gamma \vdash \bot$.

For a satisfiable set $\Gamma$ of EUF literals, and $a, b \in \terms(\Gamma)$:
\begin{enumerate}[(1)]
  \item $\Gamma \models a \eq b$ iff $a \eq b \in \Gamma^*$
  \item $\Gamma \models a \deq b$ iff $\bot \in (\Gamma \cup \{a \eq b\})^*$
\end{enumerate}

Note that $\Gamma \models a \deq b$ does not imply $\Gamma \vdash a \deq b$,
since $\peuf$ has no \textsc{Hyp} and \textsc{Contra} proof rules. The \textsc{PMod} is a form of paramodulation that is used to derive new literals by substituing equal for equal. It is useful for interpolation. 
% That is, deductive closure deduces all equalities, but not all inequalities.
% This is not useful, but just a fact to keep in mind.

%\ag{Needed?} Let $V$ be a set of constants, a restriction of $\Gamma$ to $V$, $\Gamma_{|V}$,
%is the set of all literals in $\Gamma$ that have a constant in $V$ as a subterm:
%\[
%   \Gamma_{|V} = \{\ell \in \Gamma \mid V \cap \terms(\ell) \neq \emptyset \}
% \]

% \ag{Needed?}
% If $\Gamma$ is satisfiable, then the following are true:
% \begin{enumerate}[(1)]
% \item $\Gamma \models a \eq b$ iff $(\Gamma^*)_{|\{a, b\}} \models a \eq b$
% \item $\Gamma \models a \deq b$ iff $(\Gamma^*)_{|\{a, b\}} \models a \deq b$
% \end{enumerate}
% This property will be used to prove that deciding equality requires only superterms.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> bisimul-old.tex <==
\section{Finite Bismulation of CUP}
\label{sec:extabase}

\ag{this paragraph needs work} In Sec.~\ref{sec:abs}\ag{be more direct}, we
provided a logical characterization for arbitrary UP programs, using the cover
and renaming abstractions, which induce a bisimilar transition system. The
characterization was given provided that the bisimilar transition system has
finitely many reachable configurations. In the sequel, we follow a similar
recipe to provide a finite bismulation relation for \emph{any} CUP program.
\sharon{slight rephrasing here (to show that this is done in two parts):}First,
in this section, we propose an abstraction function that is used instead of the
cover abstraction to eliminate some (but not all) of the constants that are not
assigned to program variables. The abstraction does not maintain
$\consts(q)$-equivalence of the path conditions like the cover abstraction.
Nonetheless, it results in a bisimilar transition system for CUP programs
(albeit only simulating the original transition system of arbitrary UP
programs). Unlike the cover abstraction, which may result in terms of unbounded
depth, the proposed abstraction ensures that the depth of terms is bounded. As
such, when followed by the renaming abstraction, the obtained transition system
is finite, thus establishing that any CUP is bisimilar to a finite transition
system. In section~\ref{sec:char}, we use this result to show decidability of
the reachability problem for CUPs, as well as to logically
characterize CUPs.


Intuitively, the abstraction ``truncates'' the congruence graph induced by
a path condition in nodes that have no representative in the set of constants
assigned to the program variables ($V$ in the following definition), and assigns
to the truncated nodes fresh constants (from $W$ in the following definition).

Congruence closure procedures for EUF use a \emph{congruence graph} to concisely
represent the deductive closure of a set of EUF
literals~\cite{DBLP:journals/jacm/NelsonO80,DBLP:conf/rta/NieuwenhuisO05}. Here,
we use a logical characterization of a congruence graph, called an
\emph{$V$-basis}. Let $\Gamma$ be a set of EUF literals, a triple
$\langle W, \beta, \delta \rangle$ is a $V$-basis of $\Gamma$ relative
to a set of constants $V$, written $\langle W, \beta, \delta \rangle =
\base(\Gamma, V)$, iff (a) $W$ is a set of fresh constants not in
$\consts(\Gamma)$, and $\beta$ and $\delta$ are conjunctions of EUF literals; (b)
$(\beta \land \delta) \equiv_V \Gamma$; (c) $\beta \eqdef \beta_{\eq} \cup
\beta_{\deq} \cup \beta_{\funs}$ and $\delta \eqdef \delta_{\deq} \cup
\delta_{\funs}$, where
\begin{align*}
  \beta_{\eq} &\subseteq \{u \eq v \mid u, v \in V\} \qquad \beta_{\deq}\subseteq \{u \deq v \mid u, v \in V\} \\
  \beta_{\funs} &\subseteq \{v \eq f(\Vec{w}) \mid v \in V, \Vec{w} \subseteq V \cup W, \Vec{w} \cap V \neq \emptyset\}\\
  %\beta_{\deq}&\subseteq \{u \deq v \mid u, v \in V\}\\
  \delta_{\deq} &\subseteq \{u \deq w \mid u \in W, w \in W \cup V\}\\
  \delta_{\funs} &\subseteq \{ u \eq f(\Vec{w}) \mid u \in W, \Vec{w} \subseteq V \cup W\}
\end{align*}
%\hg{missing $\delta_\eq \subseteq \{w \eq t \mid  w\in W, t \in \terms(\Sigma) \setminus V\}$}
and (d) $W$, $\beta$, and $\delta$ are minimal, i.e., they cannot be represented
with fewer literals or fewer fresh constants. Note that we represent both
equalities and disequalities in the $V$-basis as common in implementations (but
not in the theoretical presentations) of the congruence closure algorithm.
Intuitively, $V$ are constants in $\consts(\Gamma)$ that represent equivalence
classes in $\Gamma$, and $W$ are constants added to represent equivalence
classes that do not have a representative in $V$. A $V$-basis is unique up to
renaming of constants in $W$ and ordering of equalities between constants in
$V$. In fact, given any two sets of literals, $\Gamma_1$ and $\Gamma_2$, with
$\langle W_1, \beta_1, \delta_1\rangle = \base(\Gamma_1, V)$ and $\langle W_2,
\beta_2, \delta_2\rangle = \base(\Gamma_2, V)$ s.t. $\beta_1 \equiv_V
\beta_2$, there is a set of literals $\beta$ over the constants $V \cup
W$ s.t. $\langle W\cup W_1', \beta, \delta_1'\rangle = \base(\Gamma_1, V)$
and $\langle W \cup W_2', \beta, \delta_2'\rangle = \base(\Gamma_2, V)$.
That is, there is a renaming of constants in $\beta_1$ and $\beta_2$ s.t.
their literals are syntactically identical.\sharon{took me a while to parse the last few sentences. It's really confusing. If we use base as a function, we can't change its result like that. Suggestion: change to $\langle W, \beta, \delta \rangle \in
\base(\Gamma, V)$ and slightly rephrase (we say "there is a set of literals $\beta$ over the constants $V \cup
W$" but we don't say where the other components, like $W$, but also $W_1',\delta_1'$... come from -- need to say that they also exist}
\sharon{must give an example!!}

\begin{definition}[$V$-base abstraction]
\label{def:vabst}
A $V$-base abstraction $\alpha_V$ for a set of constants $V$, is a function mapping a set of literals to a set of literals s.t.
for any sets of literals $\Gamma$ and $\Gamma'$:
\begin{enumerate}[(1)]
    \item $\alpha_V(\Gamma) \eqdef \beta$,  where  $\langle W, \beta, \delta\rangle = \base(\varphi, V)$,
    \item $\Gamma \equiv_V \Gamma'$, implies $\alpha_V(\Gamma) = \alpha_V(\Gamma')$.
\end{enumerate}
\end{definition}

\ag{new}
The second requirement of Def.~\ref{def:vabst} ensures that $V$-abstraction is
canonical for  $V$-equivalent formulas. We do not require
$\alpha_V$ to be computable in general. However, $\alpha_V$ is computable over finitely
many inputs by memoization.
\begin{example}
Let $\Gamma = \{x \eq f(a, v_1), y \eq f(b, v_2), v_1 \eq v_2\}$ and $V = \{a, b, x, y\}$. The $V$-basis of $\Gamma$ is $\langle W, \beta, \delta\rangle$, where $W = \{w\}$, $\beta = \{ x \eq f(a, w), y \eq f(b, w)\}$, $\delta = \{w \eq v_1, w \eq v_2\}$. The $V$-base abstraction of $\Gamma$ is $\alpha_V(\Gamma) = \{x \eq f(a, w), y \eq f(b, w)\}$. \hg{TODO: change definition of $\delta$ to accomodate this.}
\end{example}
\begin{definition}[Base abstraction]
  \label{def:alpha-abstraction}
  The base abstraction function $\exba: \Conf \to \Conf$ is defined for
  configurations of the form $\langle s, q, pc \rangle$ where $pc$ is a
  conjunction of literals. For such a configuration, we define: $\exba(\langle
  s, q, pc\rangle) \eqdef \langle s,q,\alpha_{\const(q)}(pc)\rangle$.
\end{definition}

Namely, the $\const(q)$-base abstraction $\alpha_{\const(q)}$ applied to the
path condition is determined by the state $q$ in the configuration. With abuse
of notation we sometimes write $\alpha_q(\varphi)$ as a shorthand for
$\alpha_{\consts(q)}(\varphi)$.
%\sharon{note that to apply the abstraction, we rely on $pc$ being a conjunction of literals (at least this is an assumption in the current def of $V$-abstraction)}
%\sharon{claim that the set of reachable states of the abstract transition system is finite.
%  Actually, it is not finite per-se because we don't restrict the fresh constants that appear in the abstraction (and in the transitions).
%  If we say that they are existentially quantified, then it is clear. Otherwise, should we say something about it?
%  Should we define some kind of equivalence?
%  (basically, the width of the transition relation is infinite because we can choose different constants each time)}
%\ag{Under current definition of abstraction, it is finite. That was the main point behind the change to the new definition that restricts (declaratively) what constants are chosen.}


% \sharon{removed "finite"}
\ag{Highlight that this is main theorem}
Next, we show that, given a CUP $P$, the abstract transition system
$\exba(\TS_P) = (\Conf, \initconf^\exba, \Tr^\exba)$ is bisimilar to the
concrete transition system $\TS_P = (\Conf, \initconf, \Tr)$.
%\sharon{we should
%  also show that we get a simulation relation for any program, not just
%  coherent}

\begin{theorem}
  \label{thm:main}
  Let $\langle s, q, pc\rangle$ be a reachable configuration of a CUP $P$. Then,
  \begin{enumerate}[(1)]
  \item $\langle s, q, pc\rangle \to \langle s', q', pc \land pc'\rangle$ iff\\
    $\langle s, q, \alpha_q(pc)\rangle \to \langle s', q', \alpha_{q}(pc) \land
    pc'\rangle$, and
  \item $\alpha_{q'}(pc \land pc') = \alpha_{q'}(\alpha_q(pc) \land pc')$.
  \end{enumerate}
\end{theorem}

The proof of Thm.~\ref{thm:main} is not complicated, but it is tedious and technical. It depends on many basic properties of EUF. We summarize the key results that we require in the following lemmas. The proofs of the lemmas are provided in App.~\ref{sec:proofs}.

We begin by defining a \emph{purifier} -- a set of constants  sufficient to represent a set of EUF literals with terms of depth one.
\begin{definition}[Purifier]
  \label{def:purifier}
  We say that a set of constants $V$ is a \emph{purifier} of a constant $a$ in
  a set of literals $\Gamma$, if $a \in V$ and for every term $t \in \terms(\Gamma)$ s.t. $\Gamma \vdash t \eq s[a]$,  $\exists v \in V$ s.t. $\Gamma \vdash v \eq t$.
\sharon{notation $s[a]$ wasn't defined}
\end{definition}

For example, if $\Gamma = \{ c \eq f(a), d \eq f(b), d \deq e\}$. Then, $V = \{a, b, c\}$ is  a purifier for $a$, but  not a purifier for $b$, even though $b \in V$.

In all the following lemmas,  $\Gamma$, $\varphi_1$, $\varphi_2$ are sets
of literals; $V$ a set constants; $a, b \in \const(\Gamma)$; $u, v, x, y \in V$; $V$ is a purifier for $\{x, y\}$ in $\Gamma$, $\varphi_1$, and in $\varphi_2$; $\beta = \alpha_V(\Gamma)$; and $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$.\sharon{if we have time I suggest to group the conditions less aggressively. For example, $V$ is not used in the first lemma and it is confusing}

Lemma~\ref{lm:sprtrm} says that anything newly derivable from $\Gamma$ and a new equality $a \eq b$ is derivable using superterms of $a$ and $b$:
\begin{slemma}\label{lm:sprtrm}
  Let $t_1$ and $t_2$ be two terms in $\terms(\Sigma)$ s.t. $\Gamma
  \not\vdash (t_1 \eq t_2)$. Then, $(\Gamma \land a \eq b) \vdash (t_1 \eq
  t_2)$, for some constants $a$ and $b$ in $\consts(\Gamma)$, iff there are two
  superterms, $s_1[a]$ and $s_2[b]$, of $a$ and $b$, respectively, s.t. (i)
  $\Gamma \vdash (t_1 \eq s_1[a])$, (ii) $\Gamma \vdash (t_2 \eq s_2[b])$, and
  (iii) $(\Gamma \land a \eq b ) \vdash (s_1[a] \eq s_2[b])$.
\end{slemma}
Lemma~\ref{lm:Visenough} and Lemma~\ref{lm:Visenoughdeq} say that all relevant consequences of $\Gamma$\sharon{relevant to what? can we rephrase "all consequences of $\Gamma$ that are relevant to $V$ are..."} are present in $\beta = \alpha_V(\Gamma)$ as well.
\begin{slemma}\label{lm:Visenough}
  $(\Gamma \land x \eq y \vdash u \eq v) \iff (\beta \land x \eq y \vdash u \eq
  v) $.
\end{slemma}
\begin{slemma}\label{lm:Visenoughdeq}
$(\Gamma \land x \eq y \vdash u \deq v) \iff ( \beta \land x \eq y \vdash u \deq v)$.
\end{slemma}
Lemma~\ref{lm:pur} says that $\beta = \alpha_V(\Gamma)$ can be described using terms of depth one using constants in $V$.
\begin{slemma}\label{lm:pur}
  $V$ is a purifier for $x \in V$ in $\beta$.
\end{slemma}
Lemma~\ref{lm:idem} says that $\alpha_V$ is idempotent.
\begin{slemma}\label{lm:idem}
  $\alpha_V(\Gamma) = \alpha_V(\alpha_V(\Gamma))$.
\end{slemma}
Lemma~\ref{lm:eqpres1v} and Lemma~\ref{lm:subset} say that $\alpha_V$ preserves addition of new literals and dropping of constants.
\begin{slemma}\label{lm:eqpres1v}
   $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_2 \land x \eq y)$.
\end{slemma}
\begin{slemma}\label{lm:subset}
   If $U \subseteq V$, then \[(\alpha_V(\varphi_1)= \alpha_V(\varphi_2)) \Rightarrow (\alpha_U(\varphi_1) = \alpha_U(\varphi_2))\]
\end{slemma}
Lemma~\ref{lm:deqpres1v} and Lemma~\ref{lm:propequiv} extend the preservation results to disequalities, and for equalities involving a fresh constant.
In Lemma~\ref{lm:deqpres1v} and Lemma~\ref{lm:propequiv},
$V$ is a set of constants, $x, y \in V,
 \Vec{y}\subseteq V$. $V$ is not required to be a purifier (as it was in the previous
 lemmas). $x'$ is a constant s.t. $x' \not \in \const(\varphi_1) \cup
 \const(\varphi_2)$, $V' = V \cup\{x'\}$, and $f(\Vec{y})$ is a term not in
 $\terms(\varphi_1) \cup \terms(\varphi_2)$.\sharon{same as before: most of the conditions are only for lemma 9, I suggest to move them there}
\begin{slemma}\label{lm:deqpres1v}
 $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_2 \land x \deq y)$.
\end{slemma}
\begin{slemma}\label{lm:propequiv}
  \begin{align*}
  \tag{1}\alpha_{V'}(\varphi_1 \land x' \eq y) &= \alpha_{V'}(\varphi_2 \land x' \eq y)\\
  \tag{2}\alpha_{V'}(\varphi_1 \land x' \eq f(\Vec{y})) &= \alpha_{V'}(\varphi_2 \land x' \eq f(\Vec{y}))
  \end{align*}
\end{slemma}

We are now ready to present the proof of Thm.~\ref{thm:main}:
\begin{proof}[Theorem~\ref{thm:main}]
  In the proof, we use $x = q(\pv{x})$, and $y =
  q(\pv{y})$.
%
  For part (1), we only show the proof for $s = \textbf{assume}(\pv{x} \bowtie
  \pv{y})$ since the other cases are trivial.

  The only-if direction follows since $\alpha_q(pc)$ is weaker than $pc$.
%
  For the if direction, $pc \not\vdash \bot$ since it is part of a reachable configuration. Then, there are two cases:
\begin{itemize}
  \item case $s = \textbf{assume}(\pv{x}=\pv{y})$.
  Assume $(pc \land x \eq y) \models \bot$. Then, $(pc \land x \eq y) \vdash t_1 \eq t_2$ and $pc \vdash t_1 \deq t_2$ for some $t_1, t_2 \in \terms(pc)$. By Lemma~\ref{lm:sprtrm}, in
    any new equality $(t_1 \eq t_2)$ that is implied by $pc \land (x \eq y)$
    (but not by $pc$), $t_1$ and $t_2$ are equivalent (in $pc$) to superterms of
    $x$ or $y$. By the early assume property of CUP, $\consts(q)$ purifies $\{x,
    y\}$ in $pc$. Therefore, every superterm of $x$ or $y$ is equivalent (in
    $pc$) to some constant in $\consts(q)$. Thus,  $(pc \land x \eq y) \vdash u \eq v$ and $(pc \land x \eq y)  \vdash u \deq v$ for some $u, v \in \consts(q)$.
    By Lemma~\ref{lm:Visenough}, $(\alpha_q(pc) \land x \eq y) \vdash u \eq v$.
    By Lemma~\ref{lm:Visenoughdeq}, $(\alpha_q(pc) \land x \eq y) \vdash u \deq v$. Thus, $(\alpha_q(pc)\land x \eq y) \models \bot$.
  \item case $s = \textbf{assume}(\pv{x}\neq\pv{y})$. $(pc \land x \deq y)
    \models \bot$ if and only if $pc \vdash x \eq y$. Since $x, y \in \consts(q)$,
    $\alpha_q(pc) \vdash x \eq y$.
\end{itemize}

For part (2), we only show the cases for assume and assignment statements, the
other cases are trivial.
\begin{itemize}
\item case $s = \textbf{assume}(\pv{x} = \pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \eq y) = \alpha_{q}(\alpha_q(pc)
  \land x \eq y)$. From the early assumes property, $\const(q)$
  purifies $\{x, y\}$ in $pc$.
  By Lemma~\ref{lm:pur}, $\consts(q)$ purifies $\{x, y\}$ in $\alpha_q(pc)$ as well.
  By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  By Lemma~\ref{lm:eqpres1v}, $\alpha_q(pc \land x \eq y) = \alpha_q(\alpha_q(pc) \land x \eq y)$.
  %\ag{NO CLUE WHAT THIS IS}
\item case $s = \textbf{assume}(\pv{x} \neq \pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \deq y) = \alpha_{q}(\alpha_q(pc)
  \land x \deq y)$. By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$. By Lemma~\ref{lm:deqpres1v}, $\alpha_{q}(pc \land x \deq y) = \alpha_{q}(\alpha_q(pc)
  \land x \deq y)$.

\item case $s = \pv{x} \gets \pv{y}$. W.l.o.g., assume $q' = q[\pv{x}\mapsto
  x']$, for some constant $x' \not\in \const(pc)$.
  %By Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$.
  By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  By Lemma~\ref{lm:propequiv} (case~1), $\alpha_{\consts(q)
    \cup \{x'\}}(pc \land x' \eq y) = \alpha_{\consts(q)
    \cup \{x'\}}(\alpha_q(pc) \land x' \eq y)$. By Lemma~\ref{lm:subset}, $\alpha_{q'}(pc \land x' \eq y ) = \alpha_{q'}(\alpha_q(pc) \land x' \eq y)$,
  since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$.
\item case $s = \pv{x} \gets f(\Vec{y})$. W.l.o.g., $q' = q[\pv{x}\mapsto
  x']$ for some constant $x' \not\in \const(pc)$. There are two cases: (a) there
  is a term $t \in \terms(pc)$ s.t. $pc \vdash t \eq f(\Vec{y})$, (b) there is no
  such term $t$.
  \begin{enumerate}[label=(\alph*)]
  \item By the memoizing property of CUP, there is a program variable $\pv{z}$
    s.t. $q(\pv{z}) = z$ and $pc \vdash z \eq f(\Vec{y})$. Therefore, by
    definition of $\alpha_q$, $\alpha_q(pc) \vdash z \eq f(\Vec{y})$. The rest
    of the proof is identical to the case of $s = \pv{x} \gets \pv{z}$.
  \item Since there is no term $t\in\terms(pc)$ s.t. $pc \vdash t \eq f(\Vec{y})$, $f(\Vec{y}) \not \in\terms(pc)$ as well as $f(\Vec{y}) \not \in \terms(\alpha_q(pc))$. By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  %\hg{changed $pc^*$ to $pc$}\ag{What happens if the term in not in $\terms(pc)$ but there is an equivalent term. For example, say there is $f(z)$ somewhere in the $pc$ and $z \eq y$, which case is that?}\hg{this would be the first case as $pc \vdash f(z) \eq f(y)$. By memoization, since $f(z) \in \terms(pc)$, there has to be a variable in $q$ that stores $f(z)$.} and, therefore, not in
    %By Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$.
    %\ag{how is the jump to $q'$ justified}
    By Lemma~\ref{lm:propequiv} (case~2), $\alpha_{\const(q)\cup \{x'\}}(pc \land x \eq f(\Vec{y})) = \alpha_{\const(q)\cup \{x'\}}(\alpha_q(pc) \land x \eq f(\Vec{y}))$.
    By Lemma~\ref{lm:subset}, $\alpha_{q'}(pc \land x \eq f(\Vec{y}))
    = \alpha_{q'}(\alpha_q(pc) \land x \eq f(\Vec{y}))$ since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$.\hfill\ProofSymbol
    \end{enumerate}
    \end{itemize}
  \end{proof}


\begin{corollary}
\label{cor:main}
  For a CUP $P$, the relation $\rho \eqdef \{(c, \exba(c)) \mid c \in
  \Reach(\TS_P)\}$ is a bisimulation from $\TS_P$ to $\exba(\TS_P)$.
\end{corollary}

The path condition in configurations of $\exba(\TS_P)$ is restricted to terms of depth one. However, since at every assignment to a variable $\pvx$, a fresh constant $x'$ is used to represent the new value of $\pvx$,\sharon{and since the $W$-constants introduced by $\alpha_b$ (\Cref{def:vabst}) may be different in each configuration,} the number of configurations is not bounded. As before, this is easy to fix by renaming all constants in the path condition to be in $\consts_0$\sharon{ and renaming all the $W$-variables to be taken from one set of constants}, after the abstraction.

\ag{The jump between $b$ abstraction and $q$ abstraction is hard to follow}
Let $\alpha_{b,\rn}$ be the composition of the renaming and
base abstractions, i.e.,  $\alpha_{b,\rn} \eqdef \alpha_b \circ \alpha_\rn$.\sharon{(from Arie + my suggestion to extend) where $\rn'$ is the renaming abstraction from \Cref{def:rename-abstraction} that additionally renames all constants in $W$s to ensure canonicity of the resulting formulas. Note that (1) the renaming of $\consts(q)$ to $\consts_0$ does not introduce new constants (since a constant from $\consts_0$ may only appear in $\alpha_q(pc)$  if it is still assigned to $\pvv$, in which case no renaming is needed), and (2) \Cref{def:vabst} ensures that the number of $W$ variables in $\alpha_q(pc)$, and accordingly in $\rn_0(\alpha_q(pc), q)$, is bounded by a function of the number of program variables. As a result, the range of the renaming abstraction is finite.}
Recall that $\rn_0(pc, q)$\sharon{should it be $\rn_0(\alpha_q(pc), q)$?}\hg{no, this was just meant to recall the definition of $\rn_0$. Maybe I shouldn't have used $pc$} renames all constants in $\const(q)$ with their
corresponding constants from $\const_0$. However, $\rn_0$ can introduce
new constants not in $\const(pc)$\sharon{should it be $\consts(\alpha_q(pc))$?}, if (a) $pc$\sharon{$\alpha_q(pc)$?} contains
a constant $v_0 \in \const_0$ and (b) $q(\pv{v}) \neq v_0$. However,
$\alpha_q(pc)$ does not contain any constant in $\const(pc)\setminus \const(q)$.
In particular, $v_0 \in \const(\alpha_q(pc))$ iff $q(\pv{v}) = v_0$.
Therefore, $\rn_{0}(\alpha_q(pc), q)$ does not introduce any new constants:
$\const(\rn_{0}(\alpha_q(pc), q)) = \const(\alpha_q(pc)) \cup \const_0$.\sharon{so what is the benefit? we wanted to get rid of some of the constants...
I think we need a finer claim: $\const(\rn_{0}(\alpha_q(pc), q)) = (\const(\alpha_q(pc)) \setminus \consts(q)) \cup \consts_0$}


Let $V$ be a finite set of constants and let $W$ be a possibly infinite set of
constants. There are only finitely many formulas of depth at most 1 over
constants $V \cup W$ such that they are not $V$ equivalent.\sharon{it's confusing to go back to $V,W$ after being concrete. Can we at least use $\consts_0$ instead of $V$?} \sharon{By \Cref{def:vabst},}If two formulas
$pc_1$ and $pc_2$ are $q$-equivalent, then $\alpha_q(pc_1) = \alpha_q(pc_2)$ and,
hence, $\rn_{0}(\alpha_q(pc_1), q) = \rn_{0}(\alpha_q(pc_2), q)$.\sharon{the last two paragraphs can be improved significantly. too complicated and hard to follow.
In particular, your argument was that it doesn't matter if $W$ is infinite, so why is it important that renaming doesn't add new constants?
I actually think it is wrong since $\alpha$ is applied before renaming, so there is no guarantee that it maps "equivalent" configurations to the same thing (it uses a different set of constants!)}
%Here's my understanding: after renaming, all configurations are of the form $\langle s, \qinit, pc \rangle$, where $pc$ is a conjunction of literals of depth at most $1$ over $\consts_0 \cup W$, for some (possibly infinite) $W$. Since there are only finitely many $\consts_0$-equivalent such $pc$ formulas, and $\alpha_{\qinit}$ maps each two $\consts_0$-equivalent formulas to the same formula, we get that }
Therefore, $\alpha_{b,\rn}$ is finite, and induces a finite bisimulation:
\begin{corollary}
\label{cor:finite-bis}
 For a CUP $P$, $\rho \eqdef \{(c, \alpha_{b, \rn}(c)) \mid c \in
 \Reach(\TS_P)\}$ is a finite bisimulation from $\TS_P$ to
 $\alpha_{b, \rn}(\TS_P)$.
\end{corollary}


\Cref{cor:finite-bis} ensures that $\alpha_{b, \rn}$
is sound and complete for CUP. Furthermore, $\alpha_{b, \rn}$ is sound (but not complete) for any UP:
$\alpha_{b, \rn}(c)$ induces a finite simulation for any UP
(since $\alpha_b$ only weakens path conditions).

\Cref{cor:finite-bis} suggests that CUPs are essentially finite state systems. Thus, reachability, and, more generally, temporal model checking, for them are decidable.  The only issue is that we have not established the computability of  $\exba$. We address this complication in \Cref{sec:char}.


%\ag{Hint about decidability}
%\ag{move this to section 6: add corollary that we can characterize reachable states / invariant using a formula in EUF. in text}


==> congcls.tex <==

\textbf{Deductive closure} Given a set of literals $S$, we define the \emph{deductive closure} of $S$, denoted $S^*$, as the smallest set of literals such that: 
\begin{itemize}
    \item $S \subseteq S^*$
    \item $t_1 = t_2, t_2~op~t_3 \in S^* \Rightarrow t_1~op~t_3 \in S^*  \quad (op \in \{=, \neq\})$ 
    \item $f(u_1,\ldots, u_n) = f(v_1,\ldots, v_n) \in S^*$ whenever $\forall i \cdot u_i = v_i \in S^*$, and $f(u_1,\ldots,u_n), f(v_1\ldots,v_n) \in \terms(S)$
\end{itemize}
 It holds that $\terms(S^*) \subseteq \terms(S)$ and that if $S \models \ell$ where $\terms(\ell) \subseteq \terms(S)$ then $\ell \in S^*$. In fact, we can use these property to define $S^*$:
 \[
 S^* = \{\ell \mid \terms(\ell) \subseteq \terms(S), S \models \ell\}
 \]
 
 \textbf{Subterm closed} Let $A$ be a set of literals. A set $B \subseteq A$ is \emph{subterm closed} with respect to $A$ if, for any literal $\ell \in B$ and term $t \in \terms(\ell)$, if $t~op~t_1 \in A$ then $t~op~t_1 \in B$.
 \begin{example}
 Let $A = \{f(x, y) = g(x, z), x \neq p, g(y) = r\}$ then a set $B_1 = \{f(x, y) = g(x, z)\}$ is not subterm closed with respect to $A$ because it does not contain the literal $x \neq p$. Adding this literal to $B_1$ does make it subterm closed.
 \end{example}

==> decidingcup.tex <==
\section{Verifying CUP}
\begin{theorem}
Given a coherent program $P$, the problem of verifying $P$ is decidable. 
\end{theorem}
\begin{proof}
By Algorithm.
\end{proof}
\begin{theorem}
Given a coherent program $P$ with only unary functions, the problem of verifying $P$ is PSPACE-complete.
\end{theorem}

==> definitions.tex <==
\subsection{Programs}
We assume a signature $\Sigma = (\mathcal{C}, \mathcal{F})$ with constants symbols $\mathcal{C}$, (uninterpreted) function symbols $\mathcal{F}$ and no relation symbols. We fix $V = \{v_1, \ldots, v_n\}$ to be the set of variables in a program. We assume that a program uses special constants $\hat{V} = \{\hat{v} \mid v \in V\}$, $\hat{V} \subseteq \mathcal{C}$, to initialize its variables. We also assume that all function symbols in the program are in $\mathcal{F}$. $\terms$ are the set of all terms over $\Sigma$.

The \emph{syntax} of programs is
\begin{align*}
    \langle stmt \rangle ::=\; &\mathbf{skip} \mid x := e \mid x := f(x) \mid \\ 
               &\mathbf{assume}\;(\langle cond \rangle) \mid \langle stmt \rangle; \langle stmt \rangle \mid \\ 
               &\mathbf{if}\;(\langle cond \rangle ) \;\mathbf{then} \;\langle stmt \rangle  \;\mathbf{else}\; \langle stmt \rangle \mid \\ 
               &\textbf{while}\;(\langle cond \rangle) \;\langle stmt \rangle\\
    \langle cond\rangle ::=\; &x = y \mid c = d \mid \langle cond \rangle \vee \langle cond\rangle \mid \neg \langle cond \rangle
\end{align*}
An \emph{execution} over a finite set of variable $V$ is a word over the alphabet 
\begin{multline*}
\Pi = \{``x:= y", ``x := f(z)", ``\mathbf{assume}(x = y)",\\ ``\mathbf{assume}(x \neq y)" \mid x,y,z \in V \}
\end{multline*}
\emph{Complete executions} of programs that manipulate a set of variables $V$ are executions over $V$ defined as:
\begin{alignat*}{2}
    \text{Exec}(\mathbf{skip}) &=\;&& \epsilon \\
    \text{Exec} (x := y)  &=\;&& ``x := y"\\
    \text{Exec} (x := f(x)) &=\;&& ``x := f(z)" \\
    \text{Exec} (\mathbf{assume}(c)) &=\;&& ``\mathbf{assume}(c)" \\
    \text{Exec} (\mathbf{if}\;(c)\;\mathbf{then}\; s_1 \;\mathbf{else} \;s_2) &=\;&& ``\mathbf{assume}(c)"\cdot \text{Exec}(s_1) \cup \hphantom{a} \\
    &\hphantom{=}&&``\mathbf{assume}(\neg c)" \cdot \text{Exec}(s_2)\\
    \text{Exec} (s_1;s_2) &=\;&& \text{Exec}(s_1)\cdot \text{Exec}(s_2)\\
    \text{Exec} (\textbf{while}(c) s) &=\;&& [``\textbf{assume}(c)"\cdot \text{Exec}(s)]^*\cdot\\ &\hphantom{=}&&``\textbf{assume}(\neg c)"
\end{alignat*}
A \emph{partial execution} is any prefix of a complete execution. 

The term assigned to a variable $x$ after some partial execution is captured using the function $\text{Comp} : \Pi^* \times V \mapsto \terms$ defined as:
\begin{alignat*}{3}
    \text{Comp}(\epsilon, x) &=\;&& \mathrlap{\hat{x}} \\
    \text{Comp} (\rho \cdot ``x := y", x)  &=\;&& \mathrlap{\text{Comp}(\rho, y)}\\
    \text{Comp} (\rho \cdot ``x := y", x')  &=\;&& \text{Comp}(\rho, x') && x' \neq x\\
    \text{Comp} (\rho \cdot ``x := \func(\vz)", x)  &=\;&& \func(\text{Comp}(\rho, z_1),\ldots,\text{Comp}(\rho, z_n)) && \text{where } \vz = z_1, \ldots, z_n\\
    \text{Comp} (\rho \cdot ``x := \func(\vz)", x')  &=\;&& \text{Comp}(\rho, x') && x' \neq x\\
    \text{Comp} (\rho \cdot ``assume(x = y)", x)  &=\;&& \mathrlap{\text{Comp}(\rho, x)}\\
    \text{Comp} (\rho \cdot ``assume(x \neq y)", x)  &=\;&& \mathrlap{\text{Comp}(\rho, x)}\\
\end{alignat*}

The \emph{term graph} is a 5 tuple $(\nodes,\dedges,\eqedges,\deqedges,\tags)$ where $\nodes \subseteq \terms$ is a set of nodes, $\dedges \subseteq \nodes \times \nodes$ is a set of directed edges denoting the subterm relation, $\eqedges \subseteq \nodes \times \nodes$ is a set of equality edges, $\deqedges \subseteq \nodes \times \nodes$ is a set of disequality edges, and $\tags$ is a \emph{partial} function $\nodes \mapsto V$ that maps some nodes to program variables.

Now we define the term graph of an execution $\sigma$. If $\sigma = \epsilon$, we initialize the term graph as:
\begin{alignat*}{2}
    \text{\tg}(\epsilon) &=\;&& (\hat{V}, \emptyset, \emptyset, \emptyset,\{\hat{v}\mapsto v\mid v \in V\} ) \\
\end{alignat*}

In the following, we assume that $\sigma = \rho \cdot s$ and $\text{\tg}(\rho) = (\nodes,\dedges,\eqedges,\deqedges,\tags)$.

If $s = ``x := y"$, then we update the term graph to $(\nodes,\dedges,\eqedges,\deqedges,\tags')$ where $\tags' = \tags \setminus \{(n, x) \mid (n, x) \in \terms \} \cup \{(n, x) \mid (n, y) \in \terms\}$. 

If $s = ``x := \func(\vz)"$, then we add a new vertex for $t = \text{Comp}(\sigma, x)$, add subterm edges $(t, \text{Comp}(\rho, z))$ for each $z \in \vz$, remap $x$ variable as we did in the previous case, and update the equality edges by doing a \emph{congruence closure} on the previous term graph. That is, we update term graph to $(\nodes',\dedges',\eqedges',\deqedges,\tags')$ where 
\begin{align*}
    \nodes' =& \nodes \cup \{t\}\\
    \dedges' =& \dedges \cup \{(t, \text{Comp}(\rho, z)) \mid z \in \vz\} \\
    \eqedges =& \eqedges \cup \{(\func(\vz), \func(\vk)) \mid \vz = (z_1, \ldots, z_n) \wedge \vk = (k_1, \ldots, k_n) \wedge \\
    &\forall i \cdot (z_i, k_i) \in \eqedges \wedge \func(\vk) \in \nodes\} \\
    \tags =& \tags \setminus \{(n, x) \mid (n, x) \in \terms \} \cup \{(n, x) \mid (n, y) \in \terms\} 
\end{align*}

If $s = ``\textbf{assume}(x = y)"$ and $n_1 = \text{Comp}(\rho, x)$, $n_2 = \text{Comp}(\rho, y)$ then we update the term graph to $(\nodes,\dedges,\eqedges',\deqedges,\tags)$ where $\eqedges' = \eqedges \cup \{(n_1, n_2)\} \cup \{(n_1, n_3) \mid (n_2, n_3) \in \eqedges\} \cup \{(n_2, n_3) \mid (n_1, n_3) \in \eqedges\}$.

If $s = ``\textbf{assume}(x \neq y)"$ then we update $\deqedges$ to $\deqedges \cup \{ (n_1, n_2) \mid n_1 = \text{Comp}(\rho, x) \wedge n_2 = \text{Comp}(\rho, y)\}$.

==> extbase.tex <==
\section{Abstraction}

In this section we introduce several abstractions of UPL programs.
Each abstraction is obtained by applying a different abstraction function to the configurations of the program.
\sharon{do we want to add this? where the abstractions leave the program statement $s$ and the state $q$ intact, but abstract the path condition.
It is not needed now, but it may let us state more things generally -- need to check}
The abstract transitions are obtained by taking a concrete transition and applying the abstraction on the resulting configuration.
The formal definition follows.

\begin{definition}
\label{def:abstract-TS-general}
Given a transition system $\TS = (\Conf, \initconf,\Tr)$
and a (possibly partial) abstraction function $\genAbs: \Conf \to \Conf$, we define the abstract transition system
$\TSGenAbs = (\Conf, \initconfGenAbs, \TrGenAbs)$ as follows.
The abstract initial configuration is $\initconfGenAbs = \genAbs(\initconf)$, and the abstract transition relation
is $\TrGenAbs = \{(c,c') \mid \exists \tilde{c}.~c \to \tilde{c}~\land~c' = \genAbs(\tilde{c}) \}$.
We write $c \toGenAbs c'$ when $(c,c') \in \TrGenAbs$. While $\genAbs$ may be a partial function,
we require that it is defined for $\initconf$.
\end{definition}

In the sequel we consider several abstraction functions and discuss their properties.
\sharon{I want to revise this to mention $\equiv_\sharp$}
%Each abstraction preserves a certain class of EUF properties that are true in the configuration.
%We denote by $\equiv_\sharp$ 
In all cases, the resulting abstract transition systems simulate the concrete transition system.
In the interesting cases, the abstract and the concrete transition systems are in fact bisimilar.
Simulation and bisimulation ensure that temporal properties are preserved from the abstract transition system
to the concrete transition system, where the basis ensures that properties of configurations are preserved.
The definition therefore assumes an equivalence relation $\equiv$ (for bisimulation),
respectively a preorder $\leq$ (for simulation), between configurations, which we will define later.
%We therefore first define a partial order and an equivalence relation between configurations which capture properties that are preserved between them.
\sharon{I don't know if talking about equiv and pre-order is really needed, but this is the analogue to the req that the atomic propositions agree}

\begin{definition}[\cite{DBLP:books/daglib/0067019}]
Let $\TS = (\Conf, \initconf, \Tr)$ and $\TSGenAbs = (\Conf, \initconfGenAbs, \TrGenAbs)$
be transition systems. A relation  $B \subseteq \Conf \times \Conf$ is a \emph{bisimulation} relation from $\TS$ to $\TSGenAbs$,
if for every $(c,c_\sharp) \in B$:
\begin{enumerate}[(a)]
\item $c \equiv c_\sharp$, and
\item if $c \to c'$ then there exists $c_\sharp'$ such that $c_\sharp \toGenAbs c_\sharp'$ and $(c',c_\sharp') \in B$, and
\item if $c_\sharp \toGenAbs c_\sharp'$ then there exists $c'$ such that $c \to c'$ and $(c',c_\sharp') \in B$.
\end{enumerate}
$B \subseteq \Conf \times \Conf$ is a \emph{simulation} relation from $\TS$ to $\TSGenAbs$ if for every $(c,c_\sharp) \in B$:
\begin{enumerate}[(a)]
\item $c \leq c_\sharp$, and
\item if $c \to c'$ then there exists $c_\sharp'$ such that $c_\sharp \toGenAbs c_\sharp'$ and $(c',c_\sharp') \in B$.
\end{enumerate}
$\TSGenAbs$ \emph{is bisimilar}, respectively \emph{simulates}, $\TS$ if there exists
a bisimulation, respectively, a simulation, relation $B$ from $\TS$ to $\TSGenAbs$ such that $(\initconf, \initconfGenAbs) \in B$.
\end{definition}


%Given two \euf formulas $\varphi_1$ and $\varphi_2$ and a set of constants $V$, we say that the formulas are $V$-equivalent, denoted $\varphi_1 \equiv_V \varphi_2$, if, for all \euf formulas $\psi$ such that $\const(\psi) \subseteq V$, $(\varphi_1 \wedge \psi) \models \bot$  if and only if $(\varphi_2 \wedge \psi) \models \bot$.
%\sharon{for the simulation we need one direction?? (a partial order). not sure if I'm over-complicating things, so not adding for now}
%
%\begin{example}
%Let $\varphi_1 = \{x_1 \eq f(p_0, x_0), y_1 \eq f(q_0, y_0), x_0 \eq y_0\}$, $\varphi_2 = \{x_1 \eq f(p_0, w), y_1 \eq f(q_0, w)\}$, $\varphi_3 = \{x_1 \eq f(p_0, x_0), y_1 \eq f(q_0, y_0)\}$, and $V = \{x_1, y_1, p_0, q_0\}$. $\varphi_1 \equiv_V \varphi_2$ but $\varphi_1 \not\equiv_V \varphi_3$.
%\end{example}
%
%Given a state $q$, we denote the set of all constants that represent current variable assignments in $q$
%by $\consts(q) = \{c \mid \exists v \cdot q[v] = c\}$.
%% the set of all constants that represent current variable assignments in $q$.
%
%
%\begin{definition}[Configuration Equivalence]
%Let $c= \langle s, q, pc \rangle$ and $c' = \langle s, q, pc' \rangle$ be configurations in $\Conf$.
%$c,c'$ are called \emph{variable-equivalent}, denoted $c \equiv c'$, if
%$pc \equiv_\consts(q) pc'$.
%\end{definition}
%Note that equivalence requires that both configurations share the same program statement and state.
%Further, the set of constants by which the equivalence is defined is determined by the state $q$ in the configurations.

\begin{definition}[NAME ME]
\label{def:alpha-abstraction}
The abstraction function $\alpha: \Conf \to \Conf$ is defined for configurations of the form
$\langle s, q, pc \rangle$ where $pc$ is a conjunction of literals.
For such a configuration, we define
\[
\alpha(\langle s, q, pc\rangle) = \langle s,q,\alpha_{\consts(q)}(pc)\rangle
\]
where $\consts(q) = \{c \mid \exists v \cdot q[v] = c\}$ is the set of all constants that represent current variable assignments in $q$.
\end{definition}
Namely, the abstraction $\alpha_q$ applied to the path condition is determined by the state $q$ in the configuration.
With abuse of notation we sometimes write $\alpha_q(\varphi)$ as a shorthand for $\alpha_{\consts(q)}(\varphi)$.

%Given a state $q$, we abstract the path condition of configurations that consist of $q$
%using the constants that represent program variable assignments in $q$.
%Formally, we denote the set of all constants that represent current variable assignments in $q$
%by $\consts(q) = \{c \mid \exists v \cdot q[v] = c\}$.
%% the set of all constants that represent current variable assignments in $q$.
%For a formula $\varphi$, we define $\alpha_q(\varphi)$ to be $\alpha_{\consts(q)}(\varphi)$.
%\begin{definition}[Constants Abstraction]\sharon{another name}
%\label{def:q-abstraction}
%The \emph{constants abstraction function} $\alpha: \Conf \to \Conf$ is defined as follows:
%\[
%\alpha(\langle s, q, pc\rangle) = \langle s,q,\alpha_q(pc)\rangle.
%\]
%\end{definition}
%Note that the abstraction $\alpha_q$ applied to the path condition is determined by the state $q$ in the configuration.


%\sharon{defined the abstract transition system. If we have a (semi) characterization of the abstract configurations (i.e., of $\beta$), we can use it to define the set of configurations to be more restricted than in the case of a transition system. We can also use $\alpha(\Conf)$ -- it is now well defined}
%For a UPL program $P$ and the corresponding transition system $\TS_P = \tuple{\Conf,\initconf,\Tr}$
%defined over signature $\Sigma$,
%the \emph{abstraction of $\TS_P$}\sharon{give the abstraction a name?? the 1-depth abstraction?}
%is the transition system $\TSAbs_P = \tuple{\Conf,\initconfAbs,\TrAbs}$,
%where $\initconfAbs = %\alpha_{q_{\mathit{init}}}(\initconf)$ and $\TrAbs = \{(c,c') \mid c \to \langle s, q, pc \rangle \land c' = \alpha_q(\langle s, q, pc \rangle) \}$.
%\alpha(\initconf)$ and $\TrAbs = \{(c,c') \mid c \to \tilde{c}~\land~c' = \alpha(\tilde{c}) \}$.
%Namely, each abstract transition corresponds to taking a concrete transition followed by applying the abstraction.
%We write $c \toAbs c'$ when $(c,c') \in \TrAbs$.
%%where $q$ is the state obtained after making the concrete transition.

\sharon{note that to apply the abstraction, we rely on $pc$ being a conjunction of literals (at least this is an assumption in the current def of $V$-abstraction)}

\sharon{claim that the set of reachable states of the abstract transition system is finite.
Actually, it is not finite per-se because we don't restrict the fresh constants that appear in the abstraction (and in the transitions).
If we say that they are existentially quantified, then it is clear. Otherwise, should we say something about it?
Should we define some kind of equivalence?
(basically, the width of the transition relation is infinite because we can choose different constants each time)} 
\ag{Under current definition of abstraction, it is finite. That was the main point behind the change to the new definition that restricts (declaratively) what constants are chosen.}

==> extbase2.tex <==
\section{Abstraction}

In this section we introduce several abstractions of UPL programs.


\label{sec:extabase}
Given two \euf formulas $\varphi_1$ and $\varphi_2$ and a set of constants $V$, we say that the formulas are $V$-equivalent, denoted $\varphi_1 \equiv_V \varphi_2$, if, for all \euf formulas $\psi$ such that $\const(\psi) \subseteq V$, $(\varphi_1 \wedge \psi) \models \bot$  if and only if $(\varphi_2 \wedge \psi) \models \bot$. \sharon{I suggest to add a footnote saying that this means that the formulas are equivalent when all constants other than $V$ are treated as existentially quantified variables. }\ag{That would not be true. We want a formula $A$ and its unifrom interpolant $U$ to be equivalent by our definitions. However, their existential closures are not equivalent}

\begin{example}
Let $\varphi_1 = \{x_1 \eq f(p_0, x_0), y_1 \eq f(q_0, y_0), x_0 \eq y_0\}$, $\varphi_2 = \{x_1 \eq f(p_0, w), y_1 \eq f(q_0, w)\}$, $\varphi_3 = \{x_1 \eq f(p_0, x_0), y_1 \eq f(q_0, y_0)\}$, and $V = \{x_1, y_1, p_0, q_0\}$. $\varphi_1 \equiv_V \varphi_2$ but $\varphi_1 \not\equiv_V \varphi_3$.
\end{example}

Congruence closure procedures for EUF use a \emph{congruence graph} to concisely
represent the deductive closure of a set of EUF
literals~\cite{DBLP:journals/jacm/NelsonO80,DBLP:conf/rta/NieuwenhuisO05}. In
this paper, we use a logical characterization of a congruence graph, called an
\emph{extensional basis}. Let $\Gamma$ be a set of EUF literals, a triple
$\langle W, \beta, \delta \rangle$ is an extensional basis of $\Gamma$ relative
to a set of constants $V$, written $\langle W, \beta, \delta \rangle =
\extbase(\Gamma, V)$, iff (a) $W$ is a set of fresh constants not in
$\consts(\Gamma)$\sharon{can we not require taht $W$ are fresh but only that $W \cap V = \emptyset$?} and $\beta$ and $\delta$ are conjunctions of EUF literals; (b)
$(\beta \land \delta) \equiv_V \Gamma$; (c) $\beta \eqdef \beta_{\eq} \cup
\beta_{\deq} \cup \beta_{\funs}$ and $\delta \eqdef \delta_{\deq} \cup
\delta_{\funs}$, where
\begin{align*}
  \beta_{\eq} &\subseteq \{u \eq v \mid u, v \in V\} \\
  \beta_{\funs} &\subseteq \{v \eq f(\Vec{w}) \mid v \in V, \Vec{w} \in V \cup W, \Vec{w} \cap V \neq \emptyset\}\\
  \beta_{\deq}&\subseteq \{u \deq v \mid u, v \in V\}\\
  \delta_{\deq} &\subseteq \{u \deq w \mid u \in W, w \in W \cup V\}\\
  \delta_{\funs} &\subseteq \{ u \eq f(\Vec{w}) \mid u \in W, \Vec{w} \in V \cup W\}
\end{align*}
and (d) $W$, $\beta$, and $\delta$ are minimal, i.e., they cannot be represented
by a fewer number of literals or fresh constants. Note that we represent both
equalities and disequalities in the extensional basis as common in
implementations (but not in the theoretical presentations) of the congruence closure
algorithm. Intuitively, $V$ are constants in $\consts(\Gamma)$ that represent equivalence classes in $\Gamma$, and $W$ are constants added to represent equivalence classes that do not have a representative in $V$.
%\hg{TODO: modify definition of $\beta_{\funs}$ to say that atleast one of the $\Vec{w} \in V$. If $\Gamma = v \eq f(x) \wedge v \eq f(y)$ and $V = \{v\}$, we want $\beta = \top$, not $v \eq f(w_1) \wedge v \eq f(w_2)$.}
%\sharon{also add $v \in V$ in this case?}
%\sharon{can we instead talk about the projection of the deductive closure to the constants in $\Gamma$? is it equivalent (for me it is easier to understand)}\ag{No, they are not equivalent, that's the point of uniform interpolation being a formula and not conjunction of literals}
An extensional basis is unique up to renaming of constants in
$W$ and ordering of equalities between constants in $V$. In fact, given any two sets of literals $\Gamma_1$ and $\Gamma_2$ with $\langle W_1, \beta_1, \delta_1\rangle = \extbase(\Gamma_1, V)$ and $\langle W_2, \beta_2, \delta_2\rangle = \extbase(\Gamma_2, V)$ such that $\beta_1 \equiv_V \beta_2$, we can have a set of literals $\beta$ over a set of constants $V \cup W$ such that $\langle W\cup W_1', \beta, \delta_1'\rangle = \extbase(\Gamma_1, V)$ as well as $\langle W \cup W_2', \beta, \delta_2'\rangle = \extbase(\Gamma_2, V)$. That is, we can rename the constants in $\beta_1$ and $\beta_2$ in such a way that all their literals are syntactically identical.

\begin{definition}\label{def:vabst}
Given a set of constants $V$, we define the $V$-abstraction function, denoted $\alpha_V$, as a function from a set of literals to a set of literals such that
\begin{enumerate}
    \item For any set of literals $\varphi$, $\alpha_V(\varphi) = \beta \text{ where } \langle W, \beta, \delta\rangle = \extbase(\varphi, V)$
    \item For any two sets of literals $\varphi_1$ and $\varphi_2$, such that $\varphi_1 \equiv_V \varphi_2$, we have $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$.
\end{enumerate}
\end{definition}
%\hg{TODO: decide between cube and set of literals}

\sharon{I put it here. need to connect the two}

\begin{definition}[NAME ME]
\label{def:alpha-abstraction}
The abstraction function $\alpha: \Conf \to \Conf$ is defined for configurations of the form
$\langle s, q, pc \rangle$ where $pc$ is a conjunction of literals.
For such a configuration, we define
\[
\alpha(\langle s, q, pc\rangle) = \langle s,q,\alpha_{\consts(q)}(pc)\rangle
\]
where $\consts(q) = \{c \mid \exists v \cdot q[v] = c\}$ is the set of all constants that represent current variable assignments in $q$.
\end{definition}
Namely, the abstraction $\alpha_q$ applied to the path condition is determined by the state $q$ in the configuration.
With abuse of notation we sometimes write $\alpha_q(\varphi)$ as a shorthand for $\alpha_{\consts(q)}(\varphi)$.

\sharon{note that to apply the abstraction, we rely on $pc$ being a conjunction of literals (at least this is an assumption in the current def of $V$-abstraction)}

\sharon{claim that the set of reachable states of the abstract transition system is finite.
Actually, it is not finite per-se because we don't restrict the fresh constants that appear in the abstraction (and in the transitions).
If we say that they are existentially quantified, then it is clear. Otherwise, should we say something about it?
Should we define some kind of equivalence?
(basically, the width of the transition relation is infinite because we can choose different constants each time)}
\ag{Under current definition of abstraction, it is finite. That was the main point behind the change to the new definition that restricts (declaratively) what constants are chosen.} 

\hg{rough idea. will refine later.}
Given a quantifier free formula $\varphi$, constants $a, b \in \const(\varphi)$ such that $a\neq b$, let $\varphi[a \rename b]$ denote $\varphi[b\mapsto x][a \mapsto b]$, where $x$ is a constant not in $\const(\varphi)$. For example, if $\varphi = (a \eq c \land b \eq d)$, $\varphi[a\rename b] = (b \eq c \wedge x \eq d)$. 

Given a path condition $pc$ and a state $q$, let $r_{init}(pc, q)$ denote the formula obtained by renaming all constants in $\const(q)$ using their initial values.
$r_{init}(pc, q) = pc[q[\pv{v}]\rename v_0]$ for all $v \in \vars$ such that $q[\pv{v}] \neq v_0$. 
\begin{definition}[renaming]
\label{def:rename-abstraction}
The abstraction function $\alpha_r: \Conf \to \Conf$ is defined for configurations of the form
$\langle s, q, pc \rangle$ where $pc$ is a conjunction of literals.
For such a configuration, we define
\[
\alpha_r(\langle s, q, pc\rangle) = \langle s,q_{init},r_{init}(pc, q)\rangle
\]
\end{definition}
The relation $R = \{(c, \alpha_r(c)\}$ is a bisimulation relation. 

$\alpha_q(pc)$ does not contain any constant in $\const(pc)\setminus \const(q)$. In particular, $v_0 \in \const(\alpha_q(pc))$ if and only if $q[\pv{v}] = v_0$. Therefore, $r_{init}(\alpha_q(pc), q)$ does not introduce any new constants: $\const(r_{init}(\alpha_q(pc), q)) = \const(\alpha_q(pc))$. The abstraction $\alpha_r(\alpha(c))$ is a finite abstraction modulo $w$.
\iffalse
\subsection{XXX}
\sharon{this is the main abstraction - give it a name}

Let $\Gamma$ be a set of literals, and $\Gamma^*$ be the deductive closure of
$\Gamma$\sharon{obtained by the rules... (otherwise, a deductive closure is everything that is
implied, not just using a certain proof system)}\ag{This is a repeat from background. Will be removed}. A set of literals $\beta$ is a basis for $\Gamma$, if $\beta^* =
\Gamma^*$, and for any strict subset $A \subset \beta$, $A^{*} \neq \Gamma^*$. That
is, $\beta$ represents the same (possibly infinite) set of literals as $\Gamma$,
and $\beta$ is an irreducible such set. A basis can be computed using the congruence
closure algorithm~\cite{abstractcongruenceclosure}

\ag{I think we do not need definition of $\base$. Current definition is broken
  since it might force $\beta$ to be infinite.}
Let $V$ be a set of constants, we write $\beta = \base(\Gamma, V)$ for a basis of
$\Gamma$ with representatives in $V$. That is, (a) $\beta$ is a basis for $\Gamma$, and if $v
\eq t \in \Gamma^*$ and $v \in V$, then there exists $u \in V$ such that (a) $u
\eq t \in \beta$; (b) $u = v$ or $u \eq v \in \beta$; and (c) $\forall \ell \in
\beta$ if $t \in \terms(\ell)$ then $\ell$ is $u \approx t$.
The last
condition ensures that a term $t$ that is equivalent to some constant $v$ is
always represented by a constant (possibly different from $v$ in case $t$ is
equivalent to multiple constants in $V$).

% A basis of $\Gamma$ can be represented in a normal form, that we call an
% \emph{extensional basis}, such that every term is of depth~1, and every
% equivalence class is represented by a constant. Let $V$ be a set of constants of
% interest, then $\langle W, \beta, \delta \rangle = \extbase(\Gamma, V)$ is an
% extensional base of $\Gamma$ relative to $V$ if (a) $\beta \eqdef \beta_{\eq} \cup
% \beta_{\neq} \cup \beta_{\funs} $, where
% \begin{align*}
%   \beta_{\eq} &\eqdef \{u \eq v \in \Gamma^{*} \mid u, v \in V\} \\
%   \beta_{\deq} &\eqdef \{u \deq v \in \Gamma^{*} \mid u, v \in V\}\\
%   \beta_{\funs} &\eqdef \{u \eq f(\Vec{v}) \in \Gamma^{*} \mid u, \Vec{v} \in V \cup W\}\\
% \end{align*}

An extensional base is a refactoring of a base to introduce representative
constants for every term. It is defined as a triple $(W, \delta, \beta) =
extbase(\Gamma, V)$, where $W$ is the set of new constants introduced by
refactoring, $\delta$ is a set of new definitions\sharon{maybe it would help to define $\delta$ explicitly:
for every term $t$ in $base(\Gamma, V)$ except for constants, introduce an equality $w_t \eq t$, right
We probably want to rewrite the defs to also use $W$ in function applications, but this can be done by computing the base:
Maybe define $extbase$ by base of $base(\Gamma, V) \cup \delta$ w.r.t. $V \cup W$? I think it will immediately imply that $V$ has priority
since the first base ensures that no definition will be added to something that is equal to a variable in $V$. This suggestion would
address my comment below. Also, I think it is good to explain that this does two things: uses $V$ when possible, and purifies other terms using $W$.
Maybe we can combine this with the def of purifier that appears later? I don't have a good concrete suggestion yet.}, and $\beta$ is as in
definition of $base(\Gamma, V)$. The requirement is that $\beta \cup \delta =
base(\Gamma \cup \delta, V \cup W)$. That is, the union of $\beta$ with the
definitions is the base of $\Gamma$ extended with the same definitions.\sharon{need to ensure that
no new literals over the terms of $\Gamma^*$ are added. That is, the projection of the closure to the terms of
$\Gamma^*$ is the same (I see now that it's written later, but I don't think the current def ensures it).
Maybe this can be achieved indirectly by requiring that $W$ or $\delta$ is minimal (which may also address the next sentence)} Also
need to ensure that constants in $V$ are used as representatives if at all
possible.

It holds that if $t_1 \eq t_2 \in (\Gamma \cup \delta)^*$ and $\terms(t_1) \cap W = \terms(t_2) \cap W = \emptyset$ then $t_1 \eq t_2 \in \Gamma^*$. Also, $\Gamma^* \subseteq (\Gamma \cup \delta)^*$.
%\sharon{this means that when projected to the original constants in $\Gamma$, $(\Gamma \cup \delta)^*$ is equal to $\Gamma^*$? i.e., no new equalities are added, just ones that refer to the new constants, but represent the same thing}

Our two desired abstractions are then defined as follows. A subset $A \subseteq
\Gamma$ is \emph{subterm closed} iff \[\forall \ell \in \Gamma \cdot \terms(\ell)
  \subseteq \terms(A) \implies \ell \in A\]
\sharon{this doesn't capture the case where one of the terms in $\ell$ is in $\terms(A)$ but the other isn't.
In that case, do we want to require that the literal is in $A$? I don't currently see the context, so keeping this question.} \ag{This was issue you pointed before. Our abstraction goes down from equalities between ``variables'' and other terms, and subterms, but not to the ``side''.}
\sharon{I am struggling with this (more precisely, with its usage and why the current def ensures what we needed when used -- see next comment). Can we simplify?}

First abstraction is, given a set of constants $V$, an abstraction
$\alpha_V(\Gamma)$ is the smallest subterm closed subset $A \subseteq \Gamma^*$
such that $\{ v \eq t \in base(\Gamma, V) \mid v \in V\} \subseteq A $.
%$\{ v \eq t \in base(\Gamma, V) \mid v \in V\} \subseteq A $.
\sharon{this is where I don't see why subterm closed gives us what we wanted:
suppose $v \eq f(t) \in base$ and $x \eq t \in base$ but $x \not \in V$ (meaning $t$ is not equivalent to any constant in $V$).
Then $A$ will not include $x \eq t$ or anything equivalent. Is that really the intention?}

Second abstraction is, let $V$ be a set of variables, and $(W, \delta, \beta) =
extbase(\Gamma, V)$, then, $\alpha_V(\Gamma) = \beta$.

\sharon{it is worth mentioning that $\beta$ can contain constants from $W$ (which are not in $\Gamma$).}

\hg{This paragraph is just to make sure that we are all on the same page. I am not going to use this in any of the proofs}
\textbf{Computing $\beta$} I intend to clarify the process of computing $\langle W, \beta, \delta \rangle = extbase(\Gamma, V)$. We look at the congruence closed graph $G$ representing $\Gamma^*$. $G$ is a set of labelled nodes. Each node denotes a term in $\Gamma^*$ and there are directed edges from nodes representing function applications to each of the function arguments. If $\Gamma^* \vdash t_1 \eq t_2$ then there is an equality edge between nodes of $t_1$ and $t_2$. If $t_1\deq t_2 \in \Gamma$, there is a disequlity edge between $t_1$ and $t_2$. A node corresponding to term $t$ is labelled using the representative, $rep(t)$, of the equivalence class $t$ belongs to. Representatives are in the set $V \cup W$: If $\Gamma^* \vdash v \eq t$ where $v \in V$, then $rep(t) = v$~(we use a fixed ordering on constants in $V$ to break ties), otherwise $rep(t) = w$ for some $w \in W$.
In this graph,
\begin{multline*}
    \beta = \{ v \eq u \in \Gamma^* \mid v,u \in V\} \cup \hphantom{a} \\
    \{v \deq u \mid v = rep(t_1), u = rep(t_2), t_1 \deq t_2 \in \Gamma, v, u \in V\} \cup \hphantom{a}\\
    \{ v \eq f(rep(t_1), \ldots, rep(t_n)) \mid v \eq f(t_1, \ldots, t_n) \in \Gamma^*, v \in V \}
\end{multline*}
\begin{multline*}
    \delta = \{w \eq u \in \Gamma^* \mid  u \text{ is a constant } \not \in V, w \in W \} \cup \hphantom{a}\\
                \{w \deq u \mid w = rep(t_1), u = rep(t_2), t_1 \deq t_2 \in \Gamma,\\
                \hfill w \in V, u \in V \cup W\} \cup \hphantom{a}\\
            \{ w \eq f(rep(t_1), \ldots, rep(t_n)) \mid w \eq f(t_1, \ldots, t_n) \in \Gamma^* \}
\end{multline*}



Next we define an abstraction function $\alpha$ for program configurations,
such that the abstract transition system induced by $\alpha$ per \Cref{def:abstract-TS-general}, denoted $\TSAbs = (\Conf, \initconfAbs,\TrAbs)$,
is bisimilar  to the concrete one whenever the program is coherent.
The abstraction function abstracts the path condition in each configuration
to only maintain certain correlations between the constants to which the program variables are mapped.

\begin{definition}\label{def:vabst}
Given a conjunction of literals $\Gamma$ and a set of constants $V \subseteq \consts$,
we define the $V$-abstraction, $\alpha_V(\Gamma)$, to be the extended basis of $\Gamma$ relative to $V$:
\[
\alpha_V(\Gamma) = \beta \text{ where } \langle W, \beta, \delta\rangle = extbase(\Gamma, V)
\]
\end{definition}

\fi 

==> invariants.tex <==
\section{Invariants of CUP}
\begin{theorem}
Let $P$ be a CUP. $P$ is safe iff there exists an inductive $Inv$ s.t. $\depth(Inv) \leq 1$.
\end{theorem}

==> kcup.tex <==
\section{k-CUP}


==> logical-old.tex <==
\section{Decidability and Logical Characterization}
\label{sec:char}
In section~\ref{sec:extabase}, we show that $\alpha_{b, \rn}$ induces a finite
bisimulation for CUPs. In this section, we show that the corresponding finite abstract transition system is computable, and use this to give a logical characterization of the reachable configurations of CUPs.

Recall that the $V$-base abstraction~(\Cref{def:vabst}) is canonical for $V$-equivalent formulas. This abstraction is not necessarily computable: while it is
straightforward to compute \emph{a} $V$-basis from the congruence closure graph,
it is difficult to ensure that the base is the same for all $V$-equivalent
formulas. However, $V$-base abstraction is computable on the fly for any finite
collection of formulas. Similarly, $\alpha_{b, \rn}$ is also computable for any finite
collection of configurations.

% $\Phi$: for each $\varphi \in
% \Phi$, \begin{inparaenum}[(1)]
% \item let $\beta$ be the $V$-basis for $\varphi$,
% \item if $\beta$ is $V$-equivalent to any other basis computed so
%   far, return the stored basis, otherwise,
% \item let $\beta$ be the $V$-abstraction of $\varphi$.
% \end{inparaenum}

% \ag{I added similar, but briefer statement after Def.~\ref{def:vabst}. We might want to keep both, we might not. I find detailed description of memoization unnecessary. There is a wikipedia page for that.}

% : For each configuration $\langle s, q, pc
% \rangle \in C$ \begin{inparaenum}
% \item compute an extensional basis for $pc$,
% \item rename the basis using $\rn_0$,
% \item if the renamed basis is $q_0$-equivalent to any of the basis computed so
%   far, return the stored basis, otherwise,
% \item store the computed basis of $pc$.
% \end{inparaenum}
% on the fly using a modified version of the above procedure. The
% modification is that, after computing an extensional basis, it is renamed using
% $\rn_0$, and the renamed basis is $q_0$-equivalent to the basis that have been
% stored.
% Since extensional basis are computed from congruence closure
% graphs, computing \emph{an} extensional basis is straightforward. But it is not
% straightforward to write an algorithm to compute the same basis for all
% $V$-equivalent formulas. That is, $V$-base abstraction is not necessarily
% computable.

Thus, given a CUP $P$, its finite bisimilar abstraction is computable. Hence,
\begin{theorem}
CUP reachability is decidable.
\end{theorem}
In fact, a stronger result follows immediately -- temporal logic model checking over CUP is decidable as well.

% \ag{I don't think this is true. Base abstraction does construct formulas of
%   depth-1, but this includes extra constants. So this, by itself, is not strong
%   enough for the conclusion. This needs a lot more motivation. Also need to
%   explain significance}
\hg{TODO: add motivation, explain significance}
% \hg{added} Our finite bisimulation results imply that CUP programs are
% essentially finite state. There are several model checking algorithms for finite
% state systems. However, without a logical characterization of CUP programs,
% these algorithms cannot be used directly to decide reachability of CUP programs.

\begin{theorem}[Logical Characterization of CUP]\label{th:lccup}
  For any CUP program $P$, there exists an inductive assertion map $\inv$, ranging over EUF formulas of depth at most 1, that characterizes the reachable configurations of $P$.
\end{theorem}

In other words, for any CUP program $P$, the strongest inductive invariant of $P$ is definable by EUF formulas over state variables of depth at most 1\sharon{emphasize that this is a \emph{finite} set of formulas}. This result is far from obvious. We split the proof into two cases: CUPs restricted to unary functions, and arbitrary CUPs.

Let 1-CUP denote the set of all CUP programs where only unary functions are allowed~(and, of course, constants).

\begin{proof}[Theorem~\ref{th:lccup}, 1-CUP]
  Let $\Sigma^1$ be a signature containing function symbols of arity atmost $1$,
  $\Sigma^1 \eqdef (\consts, \funs^1, \{\eq, \deq\})$. Let $\Gamma$ be a set of
  literals in $\Sigma^1$ and $V$ be a set of constants. By the definition of
  $V$-base abstraction~(Def.~\ref{def:vabst}), $\alpha_V(\Gamma) = \beta_\eq \land \beta_\deq \land \beta_\funs$. $\beta_\eq$ and $\beta_\deq$ are over constants in $V$. $\beta_\funs$ contains two types of literals:
$\beta_{\funs_V}$ and $\beta_{\funs_W}$. $\beta_{\funs_V}$ are 1 depth literals over constants in $V$. $\beta_{\funs_W}$ are literals of the form $v \eq f(\Vec{w})$ where $v \in V$ and $\Vec{w}$ is a list of constants, at least one of which is in $V$:
  $\Vec{w}\cap V \neq \emptyset$ and $\Vec{w}\not\subseteq V$. Since $\Gamma$
  can only have unary functions, $\beta_{\funs_W} = \emptyset$. Therefore all literals in $\alpha_V(\Gamma)$ are of depth at most 1 and only contain constants from $V$.
%~($v \eq f(\Vec{u})$ where $v \in V$ and $\Vec{u}\subseteq V$)
%  \ag{Rephrase above by saying which part of $\beta$ in the abstraction is
 %   empty. Cite cover paper for this.}\hg{rephrased. Don't understand why we
 %   need to cite cover paper. We don't apply cover in this proof.} \ag{Do not
 %   understand the rephrasing. There is no empty set, instead, there is repeat
 %   of the definition that is already in the paper.} \ag{You are right about
 %   cover paper citation. I was thinking that we have $w$ even in unary case
 %   and then eliminate them. But we changed definition of $\beta$ to push these
 %   literals into $\delta$.}
  Therefore,
\[
  \inv(s) \eqdef \bigvee \{ pc \mid \langle s, q_0, pc \rangle \in
  \Reach(\alpha_{b,\rn}(\TS_P))\}
\]
is an inductive assertion map that characterizes the
reachable configurations of $P$. Clearly, $\inv$ ranges over formulas of depth at most 1. Moreover, the size of each disjunct in
$\inv(s)$ is polynomial in the number of program variables and functions in $P$.
\end{proof}
A corollary of the above proof is that reachability of $1$-CUP is in PSPACE.

\ag{make cref use short names for Def. and Sec. and Fig.}
\begin{proof}[Theorem~\ref{th:lccup}, general case]
  The $V$-base abstraction~(\Cref{def:vabst}) introduces fresh constants. Let
  $W$ be the set of all constants introduced by the $V$-base abstraction. That
  is, for any set of literals $\Gamma$ and set of constants $V$,
  $\const(\alpha_V(\Gamma))\subseteq V \cup W$. We can use the cover
  abstraction~(Def.~\ref{def:cover-abs}) to eliminate all $W$ constants. Let
  $\alpha_{b,\rn,\cover}$ be the composition of the cover, renaming, and base
  abstractions: $\alpha_{b,\rn,\cover} \eqdef \alpha_b \circ \alpha_\rn \circ
  \alpha_\cover$. By Thm.~\ref{thm:cover-bisimilar}, $\alpha_{b, \rn,
    \cover}(\TS_P)$ is bisimilar to $\alpha_{b, \rn}(\TS_P)$.

  % From the definition of cover,
  % we have $\alpha_V(\Gamma) \equiv_V (\cover W \cdot \alpha_V(\varphi))$.
  % Therefore, for any configuration $c$, $c \in \Reach(\alpha_{b, \rn}(\TS_P))$
  % iff $c \in \Reach(\alpha_{b,\rn,\cover}(\TS_P))$, where $\alpha_{b,\rn,\cover}$
  % is the composition of the cover, renaming, and base abstractions:
  % \ag{I was expecting to use the fact that cover abstraction is bisimulation}
  % $\alpha_{b,\rn,\cover} \eqdef \alpha_b \circ \alpha_\rn \circ \alpha_\cover$.
  Hence,
\[
    \inv(s) \eqdef \bigvee \{ pc \mid \langle s, q_0, pc \rangle \in
    \Reach(\alpha_{b,\rn,\cover}(\TS_P))\}
\]
is an inductive assertion map that characterizes the reachable configurations of
$P$. The $V$-basis of any formula is at most of depth 1. Moreover, all the fresh
constants in the $V$-basis are arguments to function applications. Therefore,
the cover algorithm presented in~\cite{DBLP:conf/esop/GulwaniM08} does not
increase the depth of our formulas. Hence, $\inv$ ranges over formulas of depth at most 1.
\ag{Do not refer to the cover algorithm. Our proof is simpler, by enumerating all consequences}
\end{proof}
Consider the CUP shown in Fig.~\ref{fig:cup}. At line~9, the $\alpha_{b,\rn}$
abstraction produces the following abstract $pc$: $x_0 \eq f(a_0, w) \land y_0
\eq f(b_0, w) \land c_0 \eq d_0$. Using cover to eliminate the constant $w$
gives us $\cover w \cdot pc = (a_0 \eq b_0 \limp x_0 \eq y_0) \land c_0 \eq
d_0$, which is exactly the invariant assertion mapping $\inv(9)$ at line~9.
% Since reachability is in PSPACE,
% reachability for unary function is also in PSPACE. The inductive invariant is a
% disjuntion of reachable states which is also exponential in the number of
% variables.


% - Unary Signature is special. V-abstraction is easily computable. -
% Unary Logical Characterization: reachable states are expressible as formulas
% over 1-depth terms - This, btw, reachability PSPACE - General case: combine
% V-abstraction with Cover-abstraction. Claim that cover abstraction does not
% increase formula depth - Logical Characterization: reachable states are
% expressible as formulas over 1-depth terms - Note that cover causes a blowup
% between unary and general case. This we don't understand enough to phrase. -
% Somewhere in this section need to talk about bugs in POPL paper

% \cite{DBLP:journals/pacmpl/MathurMV19} claims to prove that the reachability
% problem for CUP is PSPACE-complete. The proof is done by constructing a finite
% automaton that accepts exactly the set of all reachable configurations in a CUP.
% However, their construction is unsound on CUP that have non-unary functions. In
% particular, the automata in~\cite{DBLP:journals/pacmpl/MathurMV19}, will be
% unsound for the CUP $P$ in Figure~\ref{ex:unsound}: the automaton corresponding
% to $P$ will not be empty even though $P$ has no complete executions.

% \hg{Attempt to explain how their automaton works. Possibly skip.} The problem is
% that their automaton only keeps track of the equalities and disequalities
% between program variables, and function applications on variables. At line 4,
% the $pc$ is $(x_0 \eq y_0 \land x_1 \eq f(a_0, x_0) \land y_1 \eq f(b_0, y_0))$.
% The automaton forgets the constants $x_0$ and $y_0$ after deriving all
% equalities and disequalities implied by them. In our case, no new equalities or
% disequalities are implied by $x_0\eq y_0$. Thus the automaton cannot infer
% $x_1\eq y_1$ at line 5.

% \begin{figure}
% \centering
% \begin{lstlisting}[numbers=left, xleftmargin=.2\textwidth]
%     assume(x == y);
%     x := f(a, x);
%     y := f(b, y);
%     assume(a == b);
%     assume(x != y)
%   \end{lstlisting}
%   \caption{A CUP whose terminal state is not reachable.}
%   \label{ex:unsound}
% \end{figure}

% Let $P$ be an UP. we already know that, for any state $\langle s, q, pc \rangle
% \in Reach(\TS^{\alpha_{br}}_P)$, $\depth(pc) \leq 1$ and $\const(pc)\subseteq
% \const(q_0)$. Therefore, size of $pc$ is $\bigoh(|\const(q_0)|^2 * |\funs^1|)$.
% Thus, the number of states in $Reach(\TS^{\alpha_{br}}_P)$ is exponential in
% $|\const(q_0)| + |\funs^1|$. Thus the reachability problem for
% $\TS^{\alpha_{br}}_P$ can be decided in PSPACE.


% Furthermore, we know that the rechability problem for 1-CUP is
% PSPACE-Hard~\cite{DBLP:journals/pacmpl/MathurMV19}. Thus,
% \begin{theorem}
%   The UP reachability problem for a 1-CUP program $P$, is PSPACE-complete.
% \end{theorem}


==> naryequivalence.tex <==
\section{Proving bisimulation}
 \sharon{title: Soundness and Completeness}
\sharon{(not sure if still relevant)
the signature was mentioned only in the previous section. Need to re-introduce it in this section}

In this section we show that, given a coherent UPL program $P$,
the \ag{finite} abstract transition system $\TSAbs_P = (\Conf, \initconfAbs, \TrAbs)$
is bisimilar to the concrete transition system $\TS_P = (\Conf, \initconf, \Tr)$.
\sharon{we should also show that we get a simulation relation for any program, not just coherent}
%
%\begin{definition}[\cite{DBLP:books/daglib/0067019}]
%$\TS_P = (\Conf, \initconf, \Tr)$ and $\TSAbs_P = (\Conf, \initconfAbs, \TrAbs)$ are bisimilar
%if there exists a relation $B \subseteq \Conf \times \Conf$ s.t.
%(i)~$(\initconf, \initconfAbs) \in B$, and
%(ii)~$B$ is a bisimulation relation, which means that for every $(c,c_\alpha) \in B$,
%\begin{itemize}
%\item if $c \to c'$ then there exists $c_\alpha'$ s.t. $c_\alpha \toAbs c_\alpha'$ and $(c',c_\alpha') \in B$, and
%\item if $c_\alpha \toAbs c_\alpha'$ then there exists $c'$ s.t. $c \to c'$ and $(c',c_\alpha') \in B$.
%\end{itemize}
%\end{definition}

The bisimulation relation is induced by the abstraction function $\alpha$ (\Cref{def:q-abstraction}).
However, since the abstraction introduces fresh constants
(which can be understood as existentially quantified variables),
we relax the relation using a notion of equivalence that we define next. \ag{This sentence needs to be updated to reflect current definition of $\alpha$.}

\sharon{my goal is to eventually  claim that $B = \{(c,c_\alpha) \mid c, c_\alpha \text{ are reachable and } c = \langle s, q, pc \rangle ~\land~ c_\alpha \equiv_{\consts(q)} \alpha(c)\}$ is a bisimulation relation.
Is this correct?}\ag{I would define $B \eqdef \{ (c, \alpha(c)) \mid c \text{ is reachable} \}$}


%\begin{definition}\label{def:vabst}
%Given a conjunction of literals $\Gamma$ and a set of constants $V$, we define the $V$-abstraction, $\alpha_V(\Gamma)$, to be the extended basis of $\Gamma$ relative to $V$:
%\[
%\alpha_V(\Gamma) = \beta \text{ where } \langle W, \beta, \delta\rangle = extbase(\Gamma, V)
%\]
%\end{definition}

%\begin{example}
%Let $\varphi_1 = x \deq y \land f(x) \eq f(y)$, $\varphi_2 = x\deq y \land f(x) \deq f(y)$, $\varphi_3 = \exists x, y\cdot \varphi_1$, and $\varphi_4 = \top$. Let $V = \{z\}$. All $\varphi_i$ are $V$-equivalent.\sharon{I think it's good to have an example, but this one doesn't give me any intuition. also, why quantifiers? I thought we insisted on quantifier-free. }
%\end{example}

Given two \euf formulas $\varphi_1$ and $\varphi_2$ and a set of constants $V$, we say that the formulas are $1$-depth $V$-equivalent, denoted $\varphi_1 \equiv^1_V \varphi_2$, if and only if they have the same $V$-abstractions: $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$.

\begin{example}
Let $\varphi_1 = x \eq f(f(y))$, $\varphi_2 = x \eq f(z)$, and $V = \{x, y\}$. The $V$-abstraction of $\varphi_1$ is $\alpha_V(\varphi_1) = x \eq f(w)$ and that of $\varphi_2$ is $\alpha_V(\varphi_2) = x \eq f(w)$. Therefore, $\varphi_1 \equiv^1_V \varphi_2$ but not $\varphi_1 \equiv_V \varphi_2$.
\end{example}

\ag{Restructure this section to have the main theorem as early as possible. Followed by all the lemmas. Followed by the proof.}

\begin{lemma}[Idempotence]\label{lm:idem}
  For any set of literals $\Gamma$ and any set of constants $V$,
  $\alpha_V(\Gamma) = \alpha_V(\alpha_V(\Gamma))$.
\end{lemma}
\begin{lemma}\label{lm:frshtrm}
Let $\Gamma$ be a set of literals, $V$ a set of constants, $\Vec{y} \subseteq V$, $x'$ a constant s.t. $x' \not\in \const(\Gamma) \cup V$, $V' = V \cup \{x'\}$, and $f(\Vec{y})$ be a term not in $\terms(\Gamma)$. Then,
\[
\alpha_V(\Gamma) ~\equiv_V~ \alpha_{V'}(\Gamma \land x' \eq f(\Vec{y}))
\]
\end{lemma}
%
\begin{proof}
  Let $\psi$ be a formula s.t. $\const(\psi) \subseteq V$. We show that
  $\alpha_V(\Gamma) \land \psi \models \bot$ iff $\alpha_{V'}(\Gamma \land x'
  \eq t) \land \psi \models \bot$.

  By definition of $V$-abstraction, $\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y})) =
  \alpha_V(\Gamma) \cup X_{def}$, where $X_{def}$ is
  \begin{multline*}
    \{x' \bowtie t \mid \alpha_V(\Gamma) \vdash f(\Vec{y}) \bowtie t, \depth(t) = 1,  \const(t) \cap \const(\Gamma) \subseteq V\}  
  \end{multline*}

Since, $\alpha_V(\Gamma) \subseteq
\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y}))$, if $\alpha_V(\Gamma) \land \psi
\models \bot$, then $\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y})) \land \psi \models
\bot$. For the other direction, assume $\alpha_{V'}(\Gamma \land x' \eq
f(\Vec{y})) \land \psi \models \bot$. Since $\alpha_{V'}(\Gamma \land x' \eq
f(\Vec{y})) \vdash x' \eq f(\Vec{y})$, $\alpha_{V'}(\Gamma \land x' \eq
f(\Vec{y}))[x'\mapsto f(\Vec{y})] \land \psi \models \bot$. Therefore, 
$\alpha_V(\Gamma) \land \psi \models \bot$. Hence, $\alpha_V(\Gamma) ~\equiv_V~
\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y}))$.
\end{proof}
\begin{lemma}\label{lm:frshvar}
Let $\Gamma$ be a set of literals, $V$ be any set of constants, $y \in V$, $x'$ be a constant s.t. $x' \not \in \const(\Gamma) \cup V$, and $V' = V \cup \{x'\}$. Then,
\[
\alpha_V(\Gamma) ~\equiv_V~ \alpha_{V'}(\Gamma \land x' \eq y)
\]
\end{lemma}
\begin{proof}
  Let $\psi$ be a formula s.t. $\const(\psi) \subseteq V$. We show that
  $\alpha_V(\Gamma) \land \psi \models \bot$ iff $\alpha_{V'}(\Gamma \land x'
  \eq y) \land \psi \models \bot$.

%Conjoining the equality $x'\eq y$ with $\Gamma$ is just like adding a new representative to the equivalence class represented by $y$. 
Let $L = \{\ell \mid \ell[x'\mapsto y] \in \alpha_V(\Gamma)\}$. By definition of
$V$-abstraction, $\alpha_{V'}(\Gamma \land x' \eq y) = \alpha_V(\Gamma) \cup L$.

Since $\alpha_V(\Gamma) \subseteq \alpha_{V'}(\Gamma \land x' \eq y)$, if
$\alpha_V(\Gamma) \land \psi \models \bot$, $\alpha_{V'}(\Gamma \land x' \eq y)
\land \psi \models \bot$. For the other direction, assume $\alpha_{V'}(\Gamma
\land x' \eq y) \land \psi \models \bot$. Since $\alpha_{V'}(\Gamma \land x' \eq
y) \vdash x' \eq y$, $\alpha_{V'}(\Gamma \land x' \eq y)[x'\mapsto y] \land \psi
\models \bot$. Therefore, we have $\alpha_V(\Gamma) \land \psi \models \bot$.
Hence $\alpha_V(\Gamma) ~\equiv_V~ \alpha_{V'}(\Gamma \land x' \eq y)$.
\end{proof}
\begin{lemma}\label{lm:propequiv}
Let $V$ be a set of constants, $\varphi_1$, $\varphi_2$ be two sets of literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$, $y \in V, \Vec{y}\subseteq V$, $x'$ be a constant s.t. $x' \not \in \const(\varphi_1) \cup \const(\varphi_2)$, $V' = V \cup\{x'\}$, and $f(\Vec{y})$ be a term not in $\terms(\varphi_1) \cup \terms(\varphi_2)$. Then,
\begin{enumerate}[(1)]
    \item $\alpha_{V'}(\varphi_1 \land x' \eq y) = \alpha_{V'}(\varphi_2 \land x' \eq y)$
    \item $\alpha_{V'}(\varphi_1 \land x' \eq f(\Vec{y})) = \alpha_{V'}(\varphi_2 \land x' \eq f(\Vec{y}))$
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}[(1)]
\item Let $\beta_1 = \alpha_V(\varphi_1)$ and $\beta_1' = \alpha_{V'}(\varphi_1
  \land x' \eq y)$, and $\beta_2 = \alpha_V(\varphi_2)$ and $\beta_2' =
  \alpha_{V'}(\varphi_2 \land x' \eq y)$. Let $\psi$ be a formula s.t.
  $\const(\psi) \subseteq V'$. We show that $\beta_1' \land \psi \models \bot$
  iff $\beta_2'\land \psi \models \bot$. We show one direction, the other one is
  symmetric.

  Assume $\beta_1' \land \psi \models \bot$. By definition of $V$-abstraction,
  both $\beta_1' \vdash x' \eq y$ and $\beta_2' \vdash x' \eq y$. Since
  $\beta_1'\land \psi \models \bot$ and $\beta_1' \vdash x' \eq y$, we have
  $\beta_1'\land \psi[x'\mapsto y] \models \bot$. By Lemma~\ref{lm:frshvar},
  $\beta_1' \equiv_V \beta_1$. Since $\beta_1'\land \psi[x'\mapsto y] \models
  \bot$, $\const(\psi[x' \mapsto y]) \subseteq V$, and $\beta_1' \equiv_V
  \beta_1$, then $\beta_1 \land \psi[x' \mapsto y] \models \bot$. Since
  $\beta_1 = \beta_2$, $\beta_2 \land \psi[x' \mapsto y] \models \bot$. By
  Lemma~\ref{lm:frshvar}, $\beta_2' \equiv_V \beta_2$. Therefore, $\beta_2'
  \land \psi[x' \mapsto y] \models \bot$. Since $\beta_2' \vdash x' \eq y$ and
  $\beta_2' \land \psi[x' \mapsto y] \models \bot$, $\beta_2' \land \psi \models
  \bot$. Therefore, $\beta_1' \equiv_{V'} \beta_2'$. Therefore,
  $\alpha_{V'}(\beta_1') = \alpha_{V'}(\beta_2')$. By Lemma~\ref{lm:idem},
  $\beta_1' = \beta_2'$.
\item Let $\beta_1 = \alpha_V(\varphi_1)$ and $\beta_1' = \alpha_{V'}(\varphi_1
  \land x' \eq f(\Vec{y}))$, and  $\beta_2 =
  \alpha_V(\varphi_2)$ and $\beta_2' = \alpha_{V'}(\varphi_2 \land \land x' \eq
  f(\Vec{y}))$. Let $\psi$ be a formula s.t. $\const(\psi) \subseteq V'$. We
  have to show that $\beta_1' \land \psi \models \bot$ iff $\beta_2'\land \psi
  \models \bot$. We prove one direction, the other direction is symmetric.
  
  Assume $\beta_1' \land \psi \models \bot$. By definition of $V$-abstraction,
  both $\beta_1' \vdash x' \eq f(\Vec{y})$ and $\beta_2' \vdash x' \eq
  f(\Vec{y})$. Since $\beta_1'\land \psi \models \bot$ and $\beta_1' \vdash x'
  \eq f(\Vec{y})$, then $\beta_1'\land \psi[x'\mapsto f(\Vec{y})] \models
  \bot$. By Lemma~\ref{lm:frshvar}, $\beta_1' \equiv_V \beta_1$. Since
  $\beta_1'\land \psi[x'\mapsto f(\Vec{y})] \models \bot$, $\const(\psi[x'
  \mapsto f(\Vec{y})]) \subseteq V$, and $\beta_1' \equiv_V \beta_1$, then 
  $\beta_1 \land \psi[x' \mapsto f(\Vec{y})] \models \bot$. Since are given that
  $\beta_1 = \beta_2$, $\beta_2 \land \psi[x' \mapsto f(\Vec{y})] \models \bot$.
  By Lemma~\ref{lm:frshvar}, $\beta_2' \equiv_V \beta_2$. Therefore, $\beta_2'
  \land \psi[x' \mapsto f(\Vec{y})] \models \bot$. Since $\beta_2' \vdash x' \eq
  f(\Vec{y})$ and $\beta_2' \land \psi[x' \mapsto f(\Vec{y})] \models \bot$,
  $\beta_2' \land \psi \models \bot$. Therefore, $\beta_1' \equiv_{V'}
  \beta_2'$. Therefore, $\alpha_{V'}(\beta_1') = \alpha_{V'}(\beta_2')$. By
  Lemma~\ref{lm:idem}, $\beta_1' = \beta_2'$.
\end{enumerate}
\end{proof}

\begin{lemma}\label{lm:subset}
  Let $V$ be a set of constants, $\varphi_1$, $\varphi_2$ be two sets of
  literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$. Then, for any $U
  \subseteq V$, $\alpha_U(\varphi_1) = \alpha_U(\varphi_2)$.
\end{lemma}
\begin{proof}
  Follow from $\alpha_U(\alpha_V(\varphi_1)) = \alpha_U(\alpha_V(\varphi_2))$,
  and $\alpha_U(\alpha_V(\varphi_i)) = \alpha_U(\varphi_i)$, for $i \in \{1, 2\}$.
\end{proof}
\iffalse
\begin{lemma}\label{lm:addlit}
If $\varphi_1 \equiv_V \varphi_2$ and $\ell$ is a literal s.t. $\const(\ell) \subseteq V$ then
\[
\varphi_1 \land \ell \equiv_V \varphi_2 \land \ell
\]
\end{lemma}
\begin{proof}
Assume to the contrary that there exists a literal $\ell$, $\const(\ell) \subseteq V$, formulas $\varphi_1$, $\varphi_2$ s.t. $\varphi_1 \equiv_V \varphi_2$ but $\varphi_1 \land \ell$ is not $V$-equivalent to $\varphi_2 \land \ell$. That is, there is a formula $\psi$ s.t. $\const(\psi) \cap (\const(\varphi_1) \cup \const(\varphi_2)) \subseteq V$, $\varphi_1 \land \ell \land \psi \models \bot$ but $\varphi_2 \land \ell \land \psi \not \models \bot$. Since $\varphi_1 \land \ell \land \psi \models \bot$, $\varphi_1 \Rightarrow \neg(\ell \land \psi)$ where $\const(\ell \land \psi) \cap (\const(\varphi_1) \cup \const(\varphi_2)) \subseteq V$. Since $\varphi_2 \land \ell \land \psi \not \models \bot$, $\varphi_1 \not\Rightarrow \neg(\ell \land \psi)$. This contradicts $\varphi_1 \equiv_V \varphi_2$.
\end{proof}
\fi
%\sharon{the proof is not immediate to me.
%I think it may help if we at least highlight what is important.
%For example, give an example where $\ell$ has additional constants and show that the lemma breaks}

\iffalse
\begin{example}
Consider the following abstraction that keeps all literals that have at least one term that is represented by constants in $V$: $\alpha'_V(\Gamma) = \{ \ell \in \Gamma^* \mid \text{there exists } t \in \terms(\ell) \text{ and } v \in V \text{ s.t. } \Gamma^* \vdash v \eq t \}$. This abstraction does not satisfy $\alpha'_V(\Gamma) \equiv^1_V \Gamma$.

Let $\Gamma = x_1 \eq f(p_0, x_0) \land y_1 \eq f(q_0, y_0) \land x_0 \eq y_0$. $\alpha'_V(\Gamma) = x_1 \eq f(p_0, x_0) \land y_1 \eq f(q_0, y_0)$. Let $\psi = p_0 \eq q_0 \land x_1 \deq y_1$. $\Gamma \land \psi$ is unsatisfiable whereas $\alpha'_V(\Gamma) \land \psi$ is satisfiable.

In our case, if $\langle W, \beta, \delta \rangle = extbase(\Gamma, V)$, $\beta = x_1 \eq f(p_0, w) \land y_1 \eq f(q_0, w)$ and $\beta \equiv^1_V \Gamma$.
\end{example}
\fi

Lemma~\ref{lm:sprtrm} and Lemma~\ref{lm:trmingam} outline important properties
of EUF that are useful in the proof of Thm.~\ref{thm:main}.
\begin{lemma}\label{lm:sprtrm}
  Let $\Gamma$ be a set of literals, and $t_1$ and $t_2$ be two terms in $\terms(\Sigma)$ s.t. $\Gamma
  \not\vdash (t_1 \eq t_2)$. Then, $(\Gamma \land a \eq b) \vdash (t_1 \eq
  t_2)$, for some constants $a$ and $b$ in $\consts(\Gamma)$, iff there are two
  superterms, $s_1[a]$ and $s_2[b]$, of $a$ and $b$, respectively, s.t. (i)
  $\Gamma \vdash (t_1 \eq s_1[a])$, (ii) $\Gamma \vdash (t_2 \eq s_2[b])$, and
  (iii) $(\Gamma \land a \eq b ) \vdash (s_1[a] \eq s_2[b])$.
\end{lemma}
\begin{lemma}\label{lm:trmingam}
  Let $\Gamma$ be a set of literals, $v \in \const(\Gamma)$. If $\Gamma \vdash v \eq t$ for some term $t \in \terms(\Sigma)$ then there exists a term $t' \in \terms(\Gamma)$ s.t. $\Gamma \vdash v \eq t'$.
\end{lemma}


\begin{definition}[Purifier]
  \label{def:purifier}
We say that a set of constants $V$ is a \emph{purifier} of a constant $a$ in
$\Gamma$ if $a \in V$, and for every term $t[a] \in \terms(\Gamma)$, there
exists $v \in V$ s.t. $\Gamma \vdash v \eq t[a]$.
\end{definition}

\begin{example}[Purifier]
Let $\Gamma = \{ c \eq f(a), d \eq f(b), d \deq e\}$. Then, $V = \{a, b, c\}$ is
a purifier for $a$, but  not a purifier for $b$ even though $b \in V$.
\end{example}

\begin{lemma}\label{lm:pur}
If $V$ is a purifier for $x$ in $\Gamma$, then $V$ is a purifier for $x$ in $\alpha_V(\Gamma)$.
\end{lemma}
\begin{lemma}\label{lm:Visenough}
  Let $\Gamma$ be a set of literals,  $x$ and $y$ be two constants in
  $\consts(\Gamma)$, $V \subseteq \consts(\Gamma)$ be
  a purifier for $\{x, y\} \subseteq V$, and $\beta =
  \alpha_V(\Gamma)$. Then, for any $u, v \in V$
\[
  (\Gamma \land x \eq y \vdash u \eq v)
  \iff
 ( \beta \land x \eq y \vdash u \eq v)
\]
\end{lemma}
\begin{proof}
  By the definition of $\beta$, $(\Gamma \vdash u \eq v)
  \iff (\beta \vdash u \eq v)$. Thus, assume that $\Gamma \not \vdash u \eq v$.

  The only-if direction is trivial since $\beta$ is weaker than $\Gamma$.

  For the if-direction, By Lemma~\ref{lm:sprtrm}, there are superterms $s_1[x]$
  and $s_2[y]$ of $x$ and $y$, respectively, s.t. $\Gamma \vdash \{u \eq s_1[x],
  v \eq s_2[y]\}$, and $(\Gamma \land x \eq y) \vdash (s_1[x] \eq s_2[y])$. The
  proof proceeds by induction on the maximum depth of $s_1$ and $s_2$. The base
  case, $s_1 = x$ and $s_2 = y$, is trivial.

%W.l.o.g, we can assume that $s_1, s_2 \in
%  \terms(\Gamma)$~(Lemma~\ref{lm:trmingam}).\ag{I don't see how you can assume
%    that the terms are already in $\Gamma$.}
  For the inductive case, we show one sub-cases, others are similar. Assume
  $s_1 = f(t_1[x], \vr)$ and $s_2 = f(t_2[y], \vr)$, for some terms $t_1[x]$,
  $t_2[y]$, $\vr$, and a function $f$. Furthermore, $(\Gamma \land x \eq
  y) \vdash t_1[x] \eq t_2[y]$.

  Since $V$ is a purifier for $\{x, y\}$, there are $x', y' \in V$ s.t.
  $\Gamma \vdash \{x' \eq t_1[x], y' \eq t_2[y]\}$, and $\Gamma \vdash \{u \eq
  f(x', \vr), v \eq f(y', \vr)\}$. By construction, $\beta \vdash \{u \eq
  f(x', \vw), v \eq f(y', \vw)\}$, for some constants $\vw \in \consts(\beta)$. By IH,
  $(\beta \land x \eq y) \vdash x' \eq y'$. Hence, by congruence, $(\beta \land
  x \eq y) \vdash v \eq u$.
  \end{proof}

\iffalse
  \ag{Original pf starts here}
If $\Gamma \not \vdash v \eq u$, according to Lemma~\ref{lm:sprtrm}, $\Gamma
\vdash v \eq t_1[a]$ and $\Gamma \vdash u \eq t_2[b]$. We do induction on the
number of times the congruence axiom is applied to derive $v \eq u$. If we do
not have to apply the congruence axiom, the lemma holds because $V$ is a
purifier for $a$ and $b$, and, by the definition of $\beta$, $\beta \vdash v \eq
a$, $\beta \vdash u \eq b$. Therefore, $\beta \land a \eq b \vdash v \eq u$.

%\sharon{this is because $V$ is a purifier for $a$ and $b$, right? }
For the inductive step, we have $\Gamma \land a \eq b \vdash v \eq u$ where $\Gamma \vdash v \eq f(t_1[a], r_1)$, $\Gamma \vdash u \eq f(t_2[b], r_2)$, and $\Gamma \vdash r_1 \eq r_2$, $r_1, r_2$ are any terms constructed using signature $\Sigma$. We have to prove that $\beta \land a \eq b \vdash v \eq u$. Note that, for readability, we have restricted $f$ to be a 2-ary function. However, the proof applies to any function symbol with any arguments.

Since $V$ is a purifier for both $a$ and $b$ in $\Gamma$, we have constants $v', u' \in V$ s.t. $\Gamma \vdash v' \eq t_1[a]$, $\Gamma \vdash u' \eq t_2[b]$. Our inductive assumption is that if $\Gamma \land a \eq b \vdash v' \eq u'$ then $\beta \land a \eq b \vdash v' \eq u'$.

\sharon{I can't follow the proof. It is very formal but imprecise. You already fixed $v,u$ before. How come it is now forall? if you are being so formal, also be precise and precisely state what you prove by induction. I can't follow what you assume in each step and what you prove. The overall structure of the proof is not clear.}

%\sharon{why $x',y'$ and not $x,y$ from above?}
Since $\Gamma \vdash v \eq f(t_1[a], r_1)$ and $\Gamma \vdash v' \eq t_1[a]$, we have $\Gamma \vdash v \eq f(v', r_1)$. Similarly, we have $\Gamma \vdash u \eq f(u', r_2)$. Since $\Gamma \vdash r_1 \eq r_2$, they must have the same equivalence class. Let $w$ be the representative for this class. By the definition of $\beta$, we have, $\beta \vdash v \eq f(v', w)$, $\beta \vdash u \eq f(u', w)$. By the inductive assumption, we have $\beta \land a \eq b\vdash u' \eq v'$. By applying congruence axiom, we have $\beta \land a \eq b \vdash v \eq u$.
\fi
\begin{lemma}\label{lm:Visenoughdeq}
  Let $\Gamma$ be a set of literals,  $x$ and $y$ be two constants in
  $\consts(\Gamma)$, $V \subseteq \consts(\Gamma)$ be
  a purifier for $\{x, y\} \subseteq V$, and $\langle W, \beta, \delta\rangle =
  \extbase(\Gamma, V)$. Then, for any $u, v \in V$
  \[
    (\Gamma \land x \eq y \vdash u \deq v)
    \iff
    ( \beta \land x \eq y \vdash u \deq v)
  \]
\end{lemma}
\begin{proof}
  By the definition of $\beta$, $(\Gamma \vdash u \deq v) \iff (\beta \vdash u \deq
  v)$. Assume $\Gamma \not \vdash u \deq v$. Then, there is a term $t \in
  \terms(\Sigma)$, s.t. $\Gamma \vdash u \deq t$ and $(\Gamma \land x \eq y)
  \vdash v \eq t$. W.l.o.g, we can assume that $t \in \terms(\Gamma)$~(Lemma~\ref{lm:trmingam}). 
%   By Lemma~\ref{lm:sprtrm}, there are terms $s_1[a]$ and
%   $s_2[b]$ s.t.
%   $\Gamma \vdash \{v \eq s_1[a], t \eq s_2[b]\}$.
%   \hg{justify why $s_2[b]\in \terms(\Gamma)$}
%   %
  Since $V$ is a purifier for $y$, there is a $y' \in V$ s.t. $\Gamma
  \vdash y' \eq t$. Therefore, $(\Gamma \land x \eq y) \vdash v \eq y'$ and
  $\Gamma \vdash u \deq y'$. By Lemma~\ref{lm:Visenough}, $(\beta \land x \eq y)
  \vdash v \eq y'$. By the definition of $\beta$, $\beta \vdash u \deq y'$.
  Therefore, $(\beta \land x \eq y) \vdash u \deq v$.
\end{proof}

\iffalse
\begin{lemma}\label{lm:Visenoughdeq2}
  Let $\Gamma$ be a set of literals, $V \subseteq \consts(\Gamma)$,
  and $\langle W, \beta, \delta\rangle = \extbase(\Gamma, V)$.
  Then, for any $a, b, u, v \in V$
\[
(\Gamma \land a \deq b \vdash u \deq v)
\iff
(\beta \land a \deq b \vdash u \deq v)
\]
\end{lemma}
\begin{proof}
  By the definition of $\beta$, $(\Gamma \vdash u \deq v) \iff (\beta \vdash u
  \deq v)$. Assume $\Gamma \not\vdash u \deq v$.  Then, $\Gamma \vdash \{u \eq a
  , v \eq b\}$. By definition, $\beta \vdash \{u \eq a, v \eq b\}$. Hence,
  \mbox{$(\beta \land a \deq b) \vdash u \deq v$}.
\end{proof}
\fi
\begin{lemma}\label{lm:eqpres1v}
Let $V$ be a set of constants, $\varphi_1$ and $\varphi_2$ be two sets of literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$, and $V$ be a purifier for $\{x, y\}$ in both $\varphi_1$ and $\varphi_2$. Then, $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_2 \land x \eq y)$
\end{lemma}
\begin{proof}
Let $L_{\eq}$ be a set of equalities between constants in $V$,  $L_{\deq}$ be a set of disequalities between constants in $V$, and $L_{\funs}$ is a set of equalities of the form $v \eq f(\Vec{w})$ where $v \in V$, and $\Vec{w}$ is a set of constants, some of which are in $V$, and the rest are not in $\const(\varphi_1)\cup\const(\varphi_2)$. Let $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_1) \cup L_{\eq}\cup L_{\funs} \cup L_{\deq}$.

By Lemma~\ref{lm:Visenough} and Lemma~\ref{lm:Visenoughdeq}, $\alpha_V(\varphi_1)\land x \eq y \vdash \ell$ for all $\ell \in L_{\eq}\cup L_{\deq}$. \hg{TODO: $L_{\funs}$}

We have, for all $\ell \in L_{\eq} \cup L_{\deq} \cup L_{\funs}$, $\alpha_V(\varphi_1) \land x \eq y \vdash \ell$. Hence, $\alpha_V(\varphi_2) \land x \eq y \vdash \ell$ for all $\ell \in L_{\eq} \cup L_{\deq} \cup L_{\funs}$. Therefore, $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_2 \land x \eq y)$.
\end{proof}
\begin{lemma}\label{lm:deqpres1v}
Let $V$ be a set of constants s.t. $x, y \in V$, $\varphi_1$ and $\varphi_2$ be two sets of literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$. Then, $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_2 \land x \deq y)$
\end{lemma}
\begin{proof}
Let $L = \{x \deq u \mid y \eq u \in \alpha_V(\varphi_1), u \in V\}$. By definition, $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_1) \land L$ as well as $\alpha_V(\varphi_2 \land x \deq y) = \alpha_V(\varphi_2) \land L$. Since $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$,  $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_2 \land x \deq y)$.
 %Therefore, proving $\alpha_V(\varphi_1 \land x \deq y) \equiv_V \alpha_V(\varphi_2 \land x \deq y)$ is equivalent to proving $\alpha_V(\varphi_1) \land L \equiv_V \alpha_V(\varphi_2) \land L$ which follows from $\alpha_V(\varphi_1) \equiv_V \alpha_V(\varphi_2)$.
\end{proof}
%\sharon{moved $\alpha_q(\varphi)$ and $\consts(q)$ to earlier.}
%Let $q$ be an environment and $\consts(q) = \{c \mid \exists v \cdot q[v] = c\}$ be the
%set of all constants that represent current variable assignments in $q$.
For a state $q$, we write $\varphi \equiv_q \psi$ %and $\alpha_q(\varphi)$
for $\varphi \equiv_{\consts(q)} \psi$. %and $\alpha_{\consts(q)}(\varphi)$, respectively.

% Given a program configuration $\langle s, q, pc \rangle$, let $Q$ denote the set
% of constants in $q$:
% \[
% Q = \{ c \mid \exists \pv{v} \cdot q[\pv{v}] = c\}
% \]
% Let $\alpha_Q(\Gamma) = \beta$ where $\langle W, \beta, \delta\rangle = extbase(\Gamma, Q)$.

\iffalse
\begin{lemma}\label{lm:cpveqv}
Let $P$ be a coherent program. Let $\langle s, q, pc\rangle$ be a reachable configuration in $P$. Then $\alpha_Q(pc) \equiv_Q pc$.
\end{lemma}
\begin{proof}
We prove this by induction on the number of steps in the derivation sequence for $\langle s, q, pc\rangle$. The lemma clearly holds for the initial configuration. Now we have to prove that if the lemma holds for the configuration $\langle s, q, pc\rangle$, it holds for $\langle s', q', pc'\rangle$ where $\langle s, q, pc\rangle \to \langle s', q', pc'\rangle$. We case split on the statement $s$. We only have to consider the assume and assignment statements.
\hg{The proof for assume statements is incomplete. It proves $\alpha_Q(pc) \land pc' \equiv_Q pc \land pc'$, not $\alpha_Q(pc \land pc') \equiv_Q pc \land pc'$ }
\begin{itemize}
    \item \textbf{assume}$(\pv{x}=\pv{y})$:$q[\pv{x}] = x, q[\pv{y}] = y$. By Lemma~\ref{lm:sprtrm}, all new equalities implied by $x \eq y$ are between terms that are in the equivalence class of superterms of $x$ and $y$. By early assume property, $Q$ is a \emph{purifier} for $x, y$ in $pc$. Therefore, all superterms of $x$ and $y$ are represented by constants in $Q$. Lemmas~\ref{lm:Visenough} and \ref{lm:Visenoughdeq} show that all new equalities and inequalities between constants in $Q$ are captured by $\alpha_Q(pc)$. Combining this with our assumption that $pc \equiv_Q \alpha_Q(pc)$, we get, for every literal $\ell$ s.t. $\const(\ell) \subseteq Q$,
    if $pc \land x \eq y \vdash \ell$, then $\alpha_Q(pc) \land x \eq y \vdash \ell$. If $\alpha_Q(pc) \land x \eq y \vdash \ell$, then $pc \land x \eq y \vdash \ell$ because $\alpha_Q(pc)$ is an abstraction of $pc$.  Therefore, $pc \land x \eq y \equiv_Q \alpha_Q(pc) \land x\eq y$.

    \item \textbf{assume}$(\pv{x}\neq\pv{y})$: $q[\pv{x}] = x, q[\pv{y}] = y$. Adding a disequality does not entail any new equalities. By Lemma~\ref{lm:Visenoughdeq2}, all disequalities introduced because of $x \deq y$ are entailed by $\alpha_Q(pc)$ as well. Therefore, if $pc \equiv_Q \alpha_Q(pc)$ then $pc \land x \deq y \equiv_Q \alpha_Q(pc) \land x\deq y$.

    \item $\pv{x} := \pv{y}$ Follows from lemma \ref{lm:propequiv}.
    \item $\pv{x} := f(\Vec{\pv{y}})$ Let $q[\pv{y}] = y$ for each $\pv{y} \in \Vec{\pv{y}}$. If $f(\Vec{y}) \not \in \terms(pc)$, we can use the third case in Lemma~\ref{lm:propequiv} otherwise, by memoization property, there exists a constant $z \in Q$ s.t. $pc \vdash z \eq f(\Vec{y})$. Since $\Vec{y} \subseteq Q$, we have $\alpha_Q(pc) \vdash z \eq f(\Vec{y})$, in which case we can apply the second case in Lemma~\ref{lm:propequiv}.
\end{itemize}
\end{proof}
\fi

\begin{theorem}
  \label{thm:main}
  Let $\langle s, q, pc\rangle$ be a reachable configuration of a CUP\footnote{coherent
  uninterpreted program} $P$. Then,
\begin{enumerate}[(1)]
    \item $\langle s, q, pc\rangle \to \langle s', q', pc \land pc'\rangle$ iff\\
          $\langle s, q, \alpha_q(pc)\rangle \to \langle s', q', \alpha_{q}(pc) \land
          pc'\rangle$, and
    \item $\alpha_{q'}(pc \land pc') = \alpha_{q'}(\alpha_q(pc) \land pc')$.
\end{enumerate}
\end{theorem}
\begin{proof}
  Throughout the proof, we use $x = q[\pv{x}]$, and $y =
  q[\pv{y}]$.
%
  We only show the proof of part (1) for $s = \textbf{assume}(\pv{x} \bowtie
  \pv{y})$ since the other cases are trivial.
  
  The only-if direction follows since $\alpha_q(pc)$ is weaker than $pc$.
%
  For the if direction, $pc \not\vdash \bot$ since it is part of a reachable configuration. Then, there are two cases:
\begin{itemize}
  \item case $s = \textbf{assume}(\pv{x}=\pv{y})$. 
  Assume $(pc \land x \eq y) \models \bot$. Then, $(pc \land x \eq y) \vdash t_1 \eq t_2$ and $pc \vdash t_1 \deq t_2$ for some $t_1, t_2 \in \terms(pc)$. By Lemma~\ref{lm:sprtrm}, in
    any new equality $(t_1 \eq t_2)$ that is implied by $pc \land (x \eq y)$
    (but not by $pc$), $t_1$ and $t_2$ are equivalent (in $pc$) to superterms of
    $x$ or $y$. By the early assume property of CUP, $\consts(q)$ purifies $\{x,
    y\}$ in $pc$. Therefore, every superterm of $x$ or $y$ is equivalent (in
    $pc$) to some constant in $\consts(q)$. Thus,  $(pc \land x \eq y) \vdash u \eq v$ and $(pc \land x \eq y)  \vdash u \deq v$ for some $u, v \in \consts(q)$.
    By Lemma~\ref{lm:Visenough}, $(\alpha_q(pc) \land x \eq y) \vdash u \eq v$.
    By Lemma~\ref{lm:Visenoughdeq}, $(\alpha_q(pc) \land x \eq y) \vdash u \deq v$. Thus, $(\alpha_q(pc)\land x \eq y) \models \bot$.
  \item case $s = \textbf{assume}(\pv{x}\neq\pv{y})$. $(pc \land x \deq y)
    \models \bot$ if and only if $pc \vdash x \eq y$. Since $x, y \in \consts(q)$,
    $\alpha_q(pc) \vdash x \eq y$.
\end{itemize}

For part (2), we only show the cases for assume and assignment statements, the
other cases are trivial.
\begin{itemize}
\item case $s = \textbf{assume}(\pv{x} = \pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \eq y) = \alpha_{q}(\alpha_q(pc)
  \land x \eq y)$. From the early assumes property, $\const(q)$ 
  purifies $\{x, y\}$ in $pc$.
  By Lemma~\ref{lm:pur}, $\consts(q)$ purifies $\{x, y\}$ in $\alpha_q(pc)$ as well.
  By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  By Lemma~\ref{lm:eqpres1v}, $\alpha_q(pc \land x \eq y) = \alpha_q(\alpha_q(pc) \land x \eq y)$. 
  %\ag{NO CLUE WHAT THIS IS}
\item case $s = \textbf{assume}(\pv{x} \neq \pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \deq y) = \alpha_{q}(\alpha_q(pc)
  \land x \deq y)$. By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$. By Lemma~\ref{lm:deqpres1v},$\alpha_{q}(pc \land x \deq y) = \alpha_{q}(\alpha_q(pc)
  \land x \deq y)$.

\item case $s = \pv{x} \gets \pv{y}$. W.l.o.g., assume $q' = q[\pv{x}\mapsto
  x']$, for some constant $x' \not\in \const(pc)$. 
  %By Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$. 
  By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  By Lemma~\ref{lm:propequiv} (case~1), $\alpha_{\consts(q)
    \cup \{x'\}}(pc \land x' \eq y) = \alpha_{\consts(q)
    \cup \{x'\}}(\alpha_q(pc) \land x' \eq y)$. By Lemma~\ref{lm:subset}, $\alpha_{q'}(pc \land x' \eq y ) = \alpha_{q'}(\alpha_q(pc) \land x' \eq y)$,
  since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$.
\item case $s = \pv{x} \gets f(\Vec{y})$. W.l.o.g., $q' = q[\pv{x}\mapsto
  x']$ for some constant $x' \not\in \const(pc)$. There are two cases: (a) there
  is a term $t \in \terms(pc)$ s.t. $pc \vdash t \eq f(\Vec{y})$ \hg{was $t \eq f(\Vec{y})$ in $pc$.}, (b) there is no
  such term $t$.
  \begin{enumerate}[label=(\alph*)]
  \item By the memoization property of CUP, there is a program variable $\pv{z}$
    s.t. $q[\pv{z}] = z$ and $pc \vdash z \eq f(\Vec{y})$. Therefore, by
    definition of $\alpha_q$, $\alpha_q(pc) \vdash z \eq f(\Vec{y})$. The rest
    of the proof is identical to the case of $s = \pv{x} \gets \pv{z}$.
  \item The term $f(\Vec{y})$ is not in $\terms(pc)$ \hg{changed $pc^*$ to $pc$}\ag{What happens if the term in not in $\terms(pc)$ but there is an equivalent term. For example, say there is $f(z)$ somewhere in the $pc$ and $z \eq y$, which case is that?}\hg{this would be the first case as $pc \vdash f(z) \eq f(y)$. By memoization, since $f(z) \in \terms(pc)$, there has to be a variable in $q$ that stores $f(z)$.} and, therefore, not in
    $\terms(\alpha_q(pc))$.   By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
    %By Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$.
    %\ag{how is the jump to $q'$ justified}
    By Lemma~\ref{lm:propequiv} (case~2), $\alpha_{\const(q)\cup \{x'\}}(pc \land x \eq f(\Vec{y})) = \alpha_{\const(q)\cup \{x'\}}(\alpha_q(pc) \land x \eq f(\Vec{y}))$.
    By Lemma~\ref{lm:subset}, $\alpha_{q'}(pc \land x \eq f(\Vec{y}))
    = \alpha_{q'}(\alpha_q(pc) \land x \eq f(\Vec{y}))$ since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$.
    \end{enumerate}
    \end{itemize}
\end{proof}

\hg{rough statements. Will refine later.}
\begin{corollary}
The relation $R = \{(c, \alpha(c))\}$ is a bisimulation relation for CUP.
\end{corollary}

\begin{corollary}
The relation $R = \{(c, \alpha_r(\alpha(c)))\}$ is a finite bisimulation relation for CUP.
\end{corollary}
\iffalse
\begin{theorem}
  Let $\langle s, q, pc\rangle$ be a reachable configuration of a CUP\footnote{coherent
  uninterpreted program} $P$. Then,
\begin{enumerate}[(1)]
    \item $\langle s, q, pc\rangle \to \langle s', q', pc \land pc'\rangle$ if
      and only if
          $\langle s, q, \alpha_q(pc)\rangle \to \langle s', q', \alpha_{q}(pc) \land
          pc'\rangle$, and
    \item $\alpha_{q'}(pc \land pc') \equiv_{q'} \alpha_{q'}(\alpha_q(pc) \land pc')$.
\end{enumerate}
\end{theorem}
\begin{proof}
  Throughout the proof, $\bowtie \in \{\eq, \deq\}$, $x = q[\pv{x}]$, and $y =
  q[\pv{y}]$.
%
  We only show the proof of part (1) for $s = \textbf{assume}(\pv{x} \bowtie
  \pv{y})$ since the other cases are trivial. If $\alpha_q(pc) \land (x
  \bowtie y) \models \bot$, then, since $\alpha_q(pc)$ is weaker than $pc$, $pc
  \land (x \bowtie y) \models \bot$.

  For the other direction, assume $pc \land (x \bowtie y) \models \bot$. Then,
\begin{itemize}
  \item case $s = \textbf{assume}(\pv{x}=\pv{y})$. By Lemma~\ref{lm:sprtrm}, in
    any new equality $(t_1 \eq t_2)$ that is implied by $pc \land (x \eq y)$
    (but not by $pc$), $t_1$ and $t_2$ are equivalent (in $pc$) to superterms of
    $x$ or $y$. By the early assume property of CUP, $\consts(q)$ purifies $\{x,
    y\}$ in $pc$. Therefore, every superterm of $x$ or $y$ is equivalent (in
    $pc$) to some constant in $\consts(q)$. \ag{the proof breaks at this point.
      will revisit later} Lemma~\ref{lm:Visenough} and
    Lemma~\ref{lm:Visenoughdeq} show that all new (in)equalities between
    constants in $\consts(q)$ are captured by $\alpha_q(pc)$. Therefore, if $pc
    \land x \eq y \models \bot$ then $\alpha_q(pc) \land x\eq y \models \bot$.
  \item case $s = \textbf{assume}(\pv{x}\neq\pv{y})$. $pc \land x \deq y
    \models \bot$ if and only if $pc \vdash x \eq y$. Since $x, y \in \consts{q}$,
    $\alpha_q(pc) \vdash x \eq y$.
\end{itemize}

For part (2), we only show the cases for assume and assignment statements, the
other cases are trivial.
\begin{itemize}
\item case $s = \textbf{assume}(\pv{x}\bowtie\pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \bowtie y) \equiv_{q} \alpha_{q}(\alpha_q(pc)
  \land x \bowtie y)$. This follows from lemmas~\ref{lm:eqpres1v} and \ref{lm:deqpres1v}.

\item case $s = \pv{x} \gets \pv{y}$. W.l.o.g., assume $q' = q[\pv{x}\mapsto
  x']$, for some constant $x' \not\in \const(pc)$. By
  Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$. By
  Lemma~\ref{lm:propequiv} (case~2), $(pc \land x' \eq y) \equiv^1_{\consts(q)
    \cup \{x'\}} (\alpha_q(pc) \land x' \eq y)$. By Lemma~\ref{lm:propequiv}
  (case 1), $(pc \land x' \eq y ) \equiv^1_{q'} (\alpha_q(pc) \land x' \eq y)$,
  since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$. By the definition of
  $1$-depth $V$-equivalence, $\alpha_{q'}(pc \land x \eq y) \equiv_{q'} \alpha_{q'}(\alpha_q(pc) \land x
  \eq y)$.
    %\sharon{I don't see why lemma 2 in the last step. Isn't it the same argument as in the case of assume: "By Lemma~\ref{lm:abspresequiv}, abstracting both sides using $Q$ gives us $Q$-equivalent formulas: $\alpha_Q(pc \land x \circ y) \equiv_Q \alpha_Q(\alpha_Q(pc) \land x \circ y)$.". If so, maybe take it outside of the cases to avoid repetition}
\item case $s = \pv{x} \gets f(\Vec{y})$. W.l.o.g., $q' = q[\pv{x}\mapsto
  x']$ for some constant $x' \not\in \const(pc)$. There are two cases: (a) there
  is a term $t \in \terms(pc)$ s.t. $t \eq f(\Vec{y})$ in $pc$, (b) there is no
  such term $t$.
  \begin{enumerate}[label=(\alph*)]
  \item By the memoization property of CUP, there is a program variable $\pv{z}$
    s.t. $q[\pv{z}] = z$ and $pc \vdash z \eq f(\Vec{y})$. Therefore, by
    definition of $\alpha_q$, $\alpha_q(pc) \vdash z \eq f(\Vec{y})$. The rest
    of the proof is identical to the case of $s = \pv{x} \gets \pv{z}$.
  \item The term $f(\Vec{y})$ is not in $\terms(pc^*)$ and, therefore, not in
    $\terms(\alpha_q(pc))$ \hg{TODO: justify}. By Lemma~\ref{lm:betapreswequiv},
    $pc \equiv^1_Q \alpha_Q(pc)$.
    By Lemma~\ref{lm:propequiv} (case~3), $(pc \land x \eq f(\Vec{y})) \equiv^1_{\const(q)
      \cup \{x'\}} (\alpha_q(pc) \land x \eq f(\Vec{y}))$.
    By Lemma~\ref{lm:propequiv} (case~1), $(pc \land x \eq f(\Vec{y}))
    \equiv^1_{q'} (\alpha_q(pc) \land x \eq f(\Vec{y}))$. By
    Lemma~\ref{lm:betapreswequiv}, $\alpha_q(pc \land x \eq f(\Vec{y})) \equiv_{q'}
    \alpha_{q'}(\alpha_q(pc) \land x \eq f(\Vec{y}))$.
    \end{enumerate}
    \end{itemize}
\end{proof}


We only have to prove the theorem for the rules for assume and assignment statement.
\paragraph{proof of first part} We only have to consider \textbf{assume} statements because none of the other statements are guarded.  According to Lemma~\ref{lm:cpveqv} $pc \equiv_Q \alpha_Q(pc)$. $pc'$ is always over the constants in $Q$. Therefore, by the definition of $\equiv_Q$, $pc \land pc' \models \bot$ if and only if $\alpha_Q(pc) \land pc' \models \bot$. By the same reasoning, $\varphi \land pc' \models \bot$ if and only if $pc \land pc' \models \bot$.
%\sharon{in the case of an assignment, $pc'$ is over the fresh constant which is not in $Q$, but it is in $Q'$. I guess you are only referring to the case of assumes, and then it's ok. But need to explain that in all other cases the transition is always enabled so there is nothing to prove.}
\fi


==> naryequivalence2.tex <==
\section{Proving bisimulation}
 \sharon{title: Soundness and Completeness}
\sharon{(not sure if still relevant)
the signature was mentioned only in the previous section. Need to re-introduce it in this section}

In this section we show that, given a coherent UPL program $P$,
the \ag{finite} abstract transition system $\TSAbs_P = (\Conf, \initconfAbs, \TrAbs)$
is bisimilar to the concrete transition system $\TS_P = (\Conf, \initconf, \Tr)$.
\sharon{we should also show that we get a simulation relation for any program, not just coherent}
%
%\begin{definition}[\cite{DBLP:books/daglib/0067019}]
%$\TS_P = (\Conf, \initconf, \Tr)$ and $\TSAbs_P = (\Conf, \initconfAbs, \TrAbs)$ are bisimilar
%if there exists a relation $B \subseteq \Conf \times \Conf$ s.t.
%(i)~$(\initconf, \initconfAbs) \in B$, and
%(ii)~$B$ is a bisimulation relation, which means that for every $(c,c_\alpha) \in B$,
%\begin{itemize}
%\item if $c \to c'$ then there exists $c_\alpha'$ s.t. $c_\alpha \toAbs c_\alpha'$ and $(c',c_\alpha') \in B$, and
%\item if $c_\alpha \toAbs c_\alpha'$ then there exists $c'$ s.t. $c \to c'$ and $(c',c_\alpha') \in B$.
%\end{itemize}
%\end{definition}

The bisimulation relation is induced by the abstraction function $\alpha$ (\Cref{def:q-abstraction}).
However, since the abstraction introduces fresh constants
(which can be understood as existentially quantified variables),
we relax the relation using a notion of equivalence that we define next. \ag{This sentence needs to be updated to reflect current definition of $\alpha$.}

\sharon{my goal is to eventually  claim that $B = \{(c,c_\alpha) \mid c, c_\alpha \text{ are reachable and } c = \langle s, q, pc \rangle ~\land~ c_\alpha \equiv_{\consts(q)} \alpha(c)\}$ is a bisimulation relation.
Is this correct?}\ag{I would define $B \eqdef \{ (c, \alpha(c)) \mid c \text{ is reachable} \}$}


%\begin{definition}\label{def:vabst}
%Given a conjunction of literals $\Gamma$ and a set of constants $V$, we define the $V$-abstraction, $\alpha_V(\Gamma)$, to be the extended basis of $\Gamma$ relative to $V$:
%\[
%\alpha_V(\Gamma) = \beta \text{ where } \langle W, \beta, \delta\rangle = extbase(\Gamma, V)
%\]
%\end{definition}

%\begin{example}
%Let $\varphi_1 = x \deq y \land f(x) \eq f(y)$, $\varphi_2 = x\deq y \land f(x) \deq f(y)$, $\varphi_3 = \exists x, y\cdot \varphi_1$, and $\varphi_4 = \top$. Let $V = \{z\}$. All $\varphi_i$ are $V$-equivalent.\sharon{I think it's good to have an example, but this one doesn't give me any intuition. also, why quantifiers? I thought we insisted on quantifier-free. }
%\end{example}

Given two \euf formulas $\varphi_1$ and $\varphi_2$ and a set of constants $V$, we say that the formulas are $1$-depth $V$-equivalent, denoted $\varphi_1 \equiv^1_V \varphi_2$, if and only if they have the same $V$-abstractions: $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$.


%Given two \euf formulas $\varphi_1$ and $\varphi_2$ and a set of constants $V$, we say that the formulas are $1$-depth $V$-equivalent, denoted $\varphi_1 \equiv^1_V \varphi_2$, if, for all \euf formulas $\psi$ of depth at most $1$, s.t. $\const(\psi) \subseteq V$, $(\varphi_1 \land \psi) \models \bot$  if and only if $(\varphi_2 \land \psi) \models \bot$.
%\hg{the restrictions on constants of $\psi$ is stronger than the restrictions in $V$-equivalence.}
\begin{example}
Let $\varphi_1 = x \eq f(f(y))$, $\varphi_2 = x \eq f(z)$, and $V = \{x, y\}$. The $V$-abstraction of $\varphi_1$ is $\alpha_V(\varphi_1) = x \eq f(w)$ and that of $\varphi_2$ is $\alpha_V(\varphi_2) = x \eq f(w)$. Therefore, $\varphi_1 \equiv^1_V \varphi_2$ but not $\varphi_1 \equiv_V \varphi_2$.
%\sharon{I don't see the 1-equiv here. $\varphi_1 \land f(y) \eq x \land f(x) \not \eq x \vdash \bot$, but $\varphi_2$ is sat with the same conjunction.}
\end{example}
% From the definition of $V$-abstraction~(Definition~\ref{def:vabst}), it is clear that $\alpha_V(\alpha_V(\Gamma)) = \alpha_V(\Gamma)$. In other words:
% \begin{lemma}\label{lm:betapreswequiv}
% For any set of literals $\Gamma$ and any set of constants $V$, $\alpha_V(\Gamma) \equiv^1_V \Gamma$
% \end{lemma}
% \begin{lemma}\label{lm:ssabs}
% For any set of literals $\Gamma$ and any two sets of constants $U, V$ s.t. $U\subseteq V$, $\alpha_V(\Gamma) \equiv_U \alpha_U(\Gamma)$
% \end{lemma}
% \begin{proof}
% We have to prove that, for any formula $\psi$ s.t. $\const(\psi) \subseteq U$, $\alpha_V(\Gamma) \land \psi \models \bot$ if and only if $\alpha_U(\Gamma) \land \psi \models \bot$. \hg{there is somekind of a subset relation between $\alpha_U(\Gamma)$ and $\alpha_V(\Gamma)$}It is clear that if $\alpha_U(\Gamma) \land \psi \models \bot$, then $\alpha_V(\Gamma) \land \psi \models \bot$. To prove the other direction, assume that $\alpha_V(\Gamma) \land \psi \models \bot$. \hg{TODO}

% %From Lemma~\ref{lm:betapreswequiv}, $\alpha_U(\alpha_V(\Gamma)) \equiv_U \alpha_V(\Gamma)$. Therefore, $\alpha_U(\alpha_V(\Gamma)) \land \psi \models \bot$. By the properties of the abstraction, we have $\alpha_U(\alpha_V(\Gamma)) \equiv \alpha_U(\Gamma)$\hg{modulo w's}. Hence $\alpha_U(\Gamma) \land \psi \models \bot$.
% \end{proof}
\ag{Restructure this section to have the main theorem as early as possible. Followed by all the lemmas. Followed by the proof.}

\begin{lemma}[Idempotence]\label{lm:idem}
  For any set of literals $\Gamma$ and any set of constants $V$,
  $\alpha_V(\Gamma) = \alpha_V(\alpha_V(\Gamma))$.
\end{lemma}
\begin{lemma}\label{lm:frshtrm}
Let $\Gamma$ be a set of literals, $V$ a set of constants, $\Vec{y} \subseteq V$, $x'$ a constant s.t. $x' \not\in \const(\Gamma) \cup V$, $V' = V \cup \{x'\}$, and $f(\Vec{y})$ be a term not in $\terms(\Gamma)$. Then,
\[
\alpha_V(\Gamma) ~\equiv_V~ \alpha_{V'}(\Gamma \land x' \eq f(\Vec{y}))
\]
\end{lemma}
%
\begin{proof}
  Let $\psi$ be a formula s.t. $\const(\psi) \subseteq V$. We show that
  $\alpha_V(\Gamma) \land \psi \models \bot$ iff $\alpha_{V'}(\Gamma \land x'
  \eq t) \land \psi \models \bot$.

  By definition of $V$-abstraction, $\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y})) =
  \alpha_V(\Gamma) \cup X_{def}$, where $X_{def}$ is
  \begin{multline*}
    \{x' \bowtie t \mid \alpha_V(\Gamma) \vdash f(\Vec{y}) \bowtie t, \depth(t) = 1,  \const(t) \cap \const(\Gamma) \subseteq V\}  
  \end{multline*}

Since, $\alpha_V(\Gamma) \subseteq
\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y}))$, if $\alpha_V(\Gamma) \land \psi
\models \bot$, then $\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y})) \land \psi \models
\bot$. For the other direction, assume $\alpha_{V'}(\Gamma \land x' \eq
f(\Vec{y})) \land \psi \models \bot$. Since $\alpha_{V'}(\Gamma \land x' \eq
f(\Vec{y})) \vdash x' \eq f(\Vec{y})$, $\alpha_{V'}(\Gamma \land x' \eq
f(\Vec{y}))[x'\mapsto f(\Vec{y})] \land \psi \models \bot$. Therefore, 
$\alpha_V(\Gamma) \land \psi \models \bot$. Hence, $\alpha_V(\Gamma) ~\equiv_V~
\alpha_{V'}(\Gamma \land x' \eq f(\Vec{y}))$.
\end{proof}
\begin{lemma}\label{lm:frshvar}
Let $\Gamma$ be a set of literals, $V$ be any set of constants, $y \in V$, $x'$ be a constant s.t. $x' \not \in \const(\Gamma) \cup V$, and $V' = V \cup \{x'\}$. Then,
\[
\alpha_V(\Gamma) ~\equiv_V~ \alpha_{V'}(\Gamma \land x' \eq y)
\]
\end{lemma}
\begin{proof}
  Let $\psi$ be a formula s.t. $\const(\psi) \subseteq V$. We show that
  $\alpha_V(\Gamma) \land \psi \models \bot$ iff $\alpha_{V'}(\Gamma \land x'
  \eq y) \land \psi \models \bot$.

%Conjoining the equality $x'\eq y$ with $\Gamma$ is just like adding a new representative to the equivalence class represented by $y$. 
Let $L = \{\ell \mid \ell[x'\mapsto y] \in \alpha_V(\Gamma)\}$. By definition of
$V$-abstraction, $\alpha_{V'}(\Gamma \land x' \eq y) = \alpha_V(\Gamma) \cup L$.

Since $\alpha_V(\Gamma) \subseteq \alpha_{V'}(\Gamma \land x' \eq y)$, if
$\alpha_V(\Gamma) \land \psi \models \bot$, $\alpha_{V'}(\Gamma \land x' \eq y)
\land \psi \models \bot$. For the other direction, assume $\alpha_{V'}(\Gamma
\land x' \eq y) \land \psi \models \bot$. Since $\alpha_{V'}(\Gamma \land x' \eq
y) \vdash x' \eq y$, $\alpha_{V'}(\Gamma \land x' \eq y)[x'\mapsto y] \land \psi
\models \bot$. Therefore, we have $\alpha_V(\Gamma) \land \psi \models \bot$.
Hence $\alpha_V(\Gamma) ~\equiv_V~ \alpha_{V'}(\Gamma \land x' \eq y)$.
\end{proof}
\begin{lemma}\label{lm:propequiv}
Let $V$ be a set of constants, $\varphi_1$, $\varphi_2$ be two sets of literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$, $y \in V, \Vec{y}\subseteq V$, $x'$ be a constant s.t. $x' \not \in \const(\varphi_1) \cup \const(\varphi_2)$, $V' = V \cup\{x'\}$, and $f(\Vec{y})$ be a term not in $\terms(\varphi_1) \cup \terms(\varphi_2)$. Then,
\begin{enumerate}[(1)]
    \item $\alpha_{V'}(\varphi_1 \land x' \eq y) = \alpha_{V'}(\varphi_2 \land x' \eq y)$
    \item $\alpha_{V'}(\varphi_1 \land x' \eq f(\Vec{y})) = \alpha_{V'}(\varphi_2 \land x' \eq f(\Vec{y}))$
\end{enumerate}
\end{lemma}
\begin{proof}
\begin{enumerate}[(1)]
\item Let $\beta_1 = \alpha_V(\varphi_1)$ and $\beta_1' = \alpha_{V'}(\varphi_1
  \land x' \eq y)$, and $\beta_2 = \alpha_V(\varphi_2)$ and $\beta_2' =
  \alpha_{V'}(\varphi_2 \land x' \eq y)$. Let $\psi$ be a formula s.t.
  $\const(\psi) \subseteq V'$. We show that $\beta_1' \land \psi \models \bot$
  iff $\beta_2'\land \psi \models \bot$. We show one direction, the other one is
  symmetric.

  Assume $\beta_1' \land \psi \models \bot$. By definition of $V$-abstraction,
  both $\beta_1' \vdash x' \eq y$ and $\beta_2' \vdash x' \eq y$. Since
  $\beta_1'\land \psi \models \bot$ and $\beta_1' \vdash x' \eq y$, we have
  $\beta_1'\land \psi[x'\mapsto y] \models \bot$. By Lemma~\ref{lm:frshvar},
  $\beta_1' \equiv_V \beta_1$. Since $\beta_1'\land \psi[x'\mapsto y] \models
  \bot$, $\const(\psi[x' \mapsto y]) \subseteq V$, and $\beta_1' \equiv_V
  \beta_1$, then $\beta_1 \land \psi[x' \mapsto y] \models \bot$. Since
  $\beta_1 = \beta_2$, $\beta_2 \land \psi[x' \mapsto y] \models \bot$. By
  Lemma~\ref{lm:frshvar}, $\beta_2' \equiv_V \beta_2$. Therefore, $\beta_2'
  \land \psi[x' \mapsto y] \models \bot$. Since $\beta_2' \vdash x' \eq y$ and
  $\beta_2' \land \psi[x' \mapsto y] \models \bot$, $\beta_2' \land \psi \models
  \bot$. Therefore, $\beta_1' \equiv_{V'} \beta_2'$. Therefore,
  $\alpha_{V'}(\beta_1') = \alpha_{V'}(\beta_2')$. By Lemma~\ref{lm:idem},
  $\beta_1' = \beta_2'$.
\item Let $\beta_1 = \alpha_V(\varphi_1)$ and $\beta_1' = \alpha_{V'}(\varphi_1
  \land x' \eq f(\Vec{y}))$, and  $\beta_2 =
  \alpha_V(\varphi_2)$ and $\beta_2' = \alpha_{V'}(\varphi_2 \land \land x' \eq
  f(\Vec{y}))$. Let $\psi$ be a formula s.t. $\const(\psi) \subseteq V'$. We
  have to show that $\beta_1' \land \psi \models \bot$ iff $\beta_2'\land \psi
  \models \bot$. We prove one direction, the other direction is symmetric.
  
  Assume $\beta_1' \land \psi \models \bot$. By definition of $V$-abstraction,
  both $\beta_1' \vdash x' \eq f(\Vec{y})$ and $\beta_2' \vdash x' \eq
  f(\Vec{y})$. Since $\beta_1'\land \psi \models \bot$ and $\beta_1' \vdash x'
  \eq f(\Vec{y})$, then $\beta_1'\land \psi[x'\mapsto f(\Vec{y})] \models
  \bot$. By Lemma~\ref{lm:frshvar}, $\beta_1' \equiv_V \beta_1$. Since
  $\beta_1'\land \psi[x'\mapsto f(\Vec{y})] \models \bot$, $\const(\psi[x'
  \mapsto f(\Vec{y})]) \subseteq V$, and $\beta_1' \equiv_V \beta_1$, then 
  $\beta_1 \land \psi[x' \mapsto f(\Vec{y})] \models \bot$. Since are given that
  $\beta_1 = \beta_2$, $\beta_2 \land \psi[x' \mapsto f(\Vec{y})] \models \bot$.
  By Lemma~\ref{lm:frshvar}, $\beta_2' \equiv_V \beta_2$. Therefore, $\beta_2'
  \land \psi[x' \mapsto f(\Vec{y})] \models \bot$. Since $\beta_2' \vdash x' \eq
  f(\Vec{y})$ and $\beta_2' \land \psi[x' \mapsto f(\Vec{y})] \models \bot$,
  $\beta_2' \land \psi \models \bot$. Therefore, $\beta_1' \equiv_{V'}
  \beta_2'$. Therefore, $\alpha_{V'}(\beta_1') = \alpha_{V'}(\beta_2')$. By
  Lemma~\ref{lm:idem}, $\beta_1' = \beta_2'$.
\end{enumerate}
\end{proof}

\begin{lemma}\label{lm:subset}
  Let $V$ be a set of constants, $\varphi_1$, $\varphi_2$ be two sets of
  literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$. Then, for any $U
  \subseteq V$, $\alpha_U(\varphi_1) = \alpha_U(\varphi_2)$.
\end{lemma}
\begin{proof}
  Follow from $\alpha_U(\alpha_V(\varphi_1)) = \alpha_U(\alpha_V(\varphi_2))$,
  and $\alpha_U(\alpha_V(\varphi_i)) = \alpha_U(\varphi_i)$, for $i \in \{1, 2\}$.
\end{proof}

Lemma~\ref{lm:sprtrm} and Lemma~\ref{lm:trmingam} outline important properties
of EUF that are useful in the proof of Thm.~\ref{thm:main}.
\begin{lemma}\label{lm:sprtrm}
  Let $\Gamma$ be a set of literals, and $t_1$ and $t_2$ be two terms in $\terms(\Sigma)$ s.t. $\Gamma
  \not\vdash (t_1 \eq t_2)$. Then, $(\Gamma \land a \eq b) \vdash (t_1 \eq
  t_2)$, for some constants $a$ and $b$ in $\consts(\Gamma)$, iff there are two
  superterms, $s_1[a]$ and $s_2[b]$, of $a$ and $b$, respectively, s.t. (i)
  $\Gamma \vdash (t_1 \eq s_1[a])$, (ii) $\Gamma \vdash (t_2 \eq s_2[b])$, and
  (iii) $(\Gamma \land a \eq b ) \vdash (s_1[a] \eq s_2[b])$.
\end{lemma}
\begin{lemma}\label{lm:trmingam}
  Let $\Gamma$ be a set of literals, $v \in \const(\Gamma)$. If $\Gamma \vdash v \eq f(t_1,\ldots,t_n)$ for some term $f(t_1,\ldots,t_n) \in \terms(\Sigma)$ then there exists a term $f(t'_1,\ldots,t'_n) \in \terms(\Gamma)$ s.t. $\Gamma \vdash v \eq f(t'_1,\ldots,t'_n)$ and $\Gamma \vdash t_i \eq t_i'$ for all $1 \leq i \leq n$.
\end{lemma}

\begin{lemma}\label{lm:trmingamdeq}
  Let $\Gamma$ be a set of literals, $v \in \const(\Gamma)$. If $\Gamma \vdash v \deq f(t_1,\ldots,t_n)$ for some term $f(t_1,\ldots,t_n) \in \terms(\Sigma)$ then there exists a term $f(t'_1,\ldots,t'_n) \in \terms(\Gamma)$ s.t. $\Gamma \vdash v \deq f(t'_1,\ldots,t'_n)$ and $\Gamma \vdash t_i \eq t_i'$ for all $1 \leq i \leq n$.
\end{lemma}

\begin{definition}[Purifier]
  \label{def:purifier}
We say that a set of constants $V$ is a \emph{purifier} of a constant $a$ in
a set of literals $\Gamma$ if $a \in V$ and for every term $t \in \terms(\Gamma)$ s.t. $\Gamma \vdash t \eq s[a]$, there exists $v \in V$ s.t. $\Gamma \vdash v \eq t$.
\end{definition}

\begin{example}[Purifier]
Let $\Gamma = \{ c \eq f(a), d \eq f(b), d \deq e\}$. Then, $V = \{a, b, c\}$ is
a purifier for $a$, but  not a purifier for $b$ even though $b \in V$.
\end{example}

\begin{lemma}\label{lm:pur}
If $V$ is a purifier for $x$ in $\Gamma$, then $V$ is a purifier for $x$ in $\alpha_V(\Gamma)$.

\end{lemma}
\begin{lemma}\label{lm:Visenough}
  Let $\Gamma$ be a set of literals,  $x$ and $y$ be two constants in
  $\consts(\Gamma)$, $V \subseteq \consts(\Gamma)$ be
  a purifier for $\{x, y\} \subseteq V$, and $\beta =
  \alpha_V(\Gamma)$. Then, for any $u, v \in V$
\[
  (\Gamma \land x \eq y \vdash u \eq v)
  \iff
 ( \beta \land x \eq y \vdash u \eq v)
\]
\end{lemma}
\begin{proof}
  By the definition of $\beta$, $(\Gamma \vdash u \eq v)
  \iff (\beta \vdash u \eq v)$. Thus, assume that $\Gamma \not \vdash u \eq v$.

  The only-if direction is trivial since $\beta$ is weaker than $\Gamma$.

  For the if-direction, By Lemma~\ref{lm:sprtrm}, there are superterms $s_1[x]$
  and $s_2[y]$ of $x$ and $y$, respectively, s.t. $\Gamma \vdash \{u \eq s_1[x],
  v \eq s_2[y]\}$, and $(\Gamma \land x \eq y) \vdash (s_1[x] \eq s_2[y])$. The
  proof proceeds by induction on the maximum depth of $s_1$ and $s_2$. The base
  case, $s_1 = x$ and $s_2 = y$, is trivial.

%W.l.o.g, we can assume that $s_1, s_2 \in
%  \terms(\Gamma)$~(Lemma~\ref{lm:trmingam}).\ag{I don't see how you can assume
%    that the terms are already in $\Gamma$.}
  For the inductive case, we show one sub-cases, others are similar. Assume
  $s_1 = f(t_1[x], \vr)$ and $s_2 = f(t_2[y], \vr)$, for some terms $t_1[x]$,
  $t_2[y]$, $\vr$, and a function $f$. Furthermore, $(\Gamma \land x \eq
  y) \vdash t_1[x] \eq t_2[y]$. Since $\Gamma \vdash \{u \eq f(t_1[x], \vr), v \eq f(t_2[y], \vr)\}$, by Lemma~\ref{lm:trmingam}, there exists terms $f(t_1', \vr_1), f(t_2', \vr_2) \in \terms(\Gamma)$ s.t. $\Gamma \vdash \{u \eq f(t_1', \vr_1), t_1[x] \eq t_1', \vr \eq \vr_1, v \eq f(t_2', \vr_2), t_2[y] \eq t_2', \vr \eq \vr_2 \}$.

  Since $V$ is a purifier for $\{x, y\}$, there are $x', y' \in V$ s.t.
  $\Gamma \vdash \{x' \eq t_1', y' \eq t_2'\}$, and $\Gamma \vdash \{u \eq
  f(x', \vr), v \eq f(y', \vr)\}$. By construction, $\beta \vdash \{u \eq
  f(x', \vw), v \eq f(y', \vw)\}$, for some constants $\vw \in \consts(\beta)$. By IH,
  $(\beta \land x \eq y) \vdash x' \eq y'$. Hence, by congruence, $(\beta \land
  x \eq y) \vdash v \eq u$.
  \end{proof}


\begin{lemma}\label{lm:Visenoughdeq}
  Let $\Gamma$ be a set of literals,  $x$ and $y$ be two constants in
  $\consts(\Gamma)$, $V \subseteq \consts(\Gamma)$ be
  a purifier for $\{x, y\} \subseteq V$, and $\langle W, \beta, \delta\rangle =
  \extbase(\Gamma, V)$. Then, for any $u, v \in V$
  \[
    (\Gamma \land x \eq y \vdash u \deq v)
    \iff
    ( \beta \land x \eq y \vdash u \deq v)
  \]
\end{lemma}
\begin{proof}
  By the definition of $\beta$, $(\Gamma \vdash u \deq v) \iff (\beta \vdash u \deq
  v)$. Assume $\Gamma \not \vdash u \deq v$. Then, there is a term $t \in
  \terms(\Sigma)$, s.t. $\Gamma \vdash u \deq t$ and $(\Gamma \land x \eq y)
  \vdash v \eq t$. By Lemma~\ref{lm:sprtrm}, $\Gamma \vdash t \eq s[y]$. We case split on whether $s[y]$ is $y$ itself or some superterm of $y$.
 \begin{itemize}
     \item case $s[y] = s$, Since $\Gamma \vdash t \eq y$, $(\Gamma \land x \eq y) \vdash v \eq y$ and $\Gamma \vdash u \deq y$. By Lemma~\ref{lm:Visenough}, $(\beta \land x \eq y) \vdash v \eq y$. By definition $\beta \vdash u \deq y$. Therefore $(\beta \land x \eq y) \vdash u \deq v$.

     \item case $s[y] = f(t_1,\ldots, t_n)$, where atleast one $t_i$ is a superterm of $y$. Since $\Gamma \vdash t \eq f(t_1,\ldots, t_n)$, $\Gamma \vdash u \deq f(t_1,\ldots, t_n)$. By Lemma~\ref{lm:trmingamdeq}, there exists a term $f(t_1',\ldots, t_n') \in \terms(\Gamma)$ s.t., $\Gamma \vdash \{ u \deq f(t_1',\ldots, t_n'), t_1' \eq t_1,\ldots, t_n' \eq t_n\}$. Since $f(t_1',\ldots, t_n') \in \terms(\Gamma)$, $\Gamma \vdash f(t_1',\ldots, t_n') \eq s[y]$, and $V$ is a purifier for $y$ in $\Gamma$, there exists a constant $y' \in V$ s.t. $\Gamma \vdash y' \eq f(t_1',\ldots, t_n')$. Therefore, $(\Gamma \land x \eq y) \vdash v \eq y'$ and $\Gamma \vdash u \deq y'$. By Lemma~\ref{lm:Visenough}, $(\beta \land x \eq y) \vdash v \eq y'$. By the definition of $\beta$, $\beta \vdash u \deq y'$. Therefore, $(\beta \land x \eq y) \vdash u \deq v$.

%   By Lemma~\ref{lm:sprtrm}, there are terms $s_1[a]$ and
%   $s_2[b]$ s.t.
%   $\Gamma \vdash \{v \eq s_1[a], t \eq s_2[b]\}$.
%   \hg{justify why $s_2[b]\in \terms(\Gamma)$}
%   %
 \end{itemize} 
  
\end{proof}


\begin{lemma}\label{lm:eqpres1v}
Let $V$ be a set of constants, $\varphi_1$ and $\varphi_2$ be two sets of literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$, and $V$ be a purifier for $\{x, y\}$ in both $\varphi_1$ and $\varphi_2$. Then, $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_2 \land x \eq y)$
\end{lemma}
\begin{proof}
Let $L_{\eq}$ be a set of equalities between constants in $V$,  $L_{\deq}$ be a set of disequalities between constants in $V$, and $L_{\funs}$ is a set of equalities of the form $v \eq f(\Vec{w})$ where $v \in V$, and $\Vec{w}$ is a set of constants, some of which are in $V$, and the rest are not in $\const(\varphi_1)\cup\const(\varphi_2)$. Let $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_1) \cup L_{\eq}\cup L_{\funs} \cup L_{\deq}$.

By Lemma~\ref{lm:Visenough} and Lemma~\ref{lm:Visenoughdeq}, $\alpha_V(\varphi_1)\land x \eq y \vdash \ell$ for all $\ell \in L_{\eq}\cup L_{\deq}$. 

Next, we prove that for all $\ell \in L_\funs$, $\alpha_V(\varphi_1) \land x \eq y \vdash \ell$. In the following, assume that $u, v \in V$ and $w \not \in \const(\Gamma)\cup V$. We assume that $\ell = v \eq f(u, w)$. All other cases are similar. 
We have $(\alpha_V(\varphi_1 \land x \eq y)) \vdash v \eq f(u, w)$ iff $(\varphi_1 \land x \eq y) \vdash v \eq f(u, t)$ for some term $t \in \terms(\Sigma)$ and there no $v' \in V$ such that $(\varphi_1 \land x \eq y) \vdash v' \eq t$. If $\varphi_1 \vdash v \eq f(u, t)$ then $\alpha_V(\varphi_1) \vdash v \eq f(u, w)$ by definition. Assume that $\varphi_1 \not \vdash v \eq f(u, t)$. By Lemma~\ref{lm:sprtrm}, we have $\varphi_1 \vdash v \eq s_1[x]$ and $\varphi_1 \vdash f(u, t) \eq s_2[y]$ and $\varphi_1 \wedge x \eq y \vdash s_1[x] \eq s_2[y]$. We case split on $s_1[x], s_2[y]$.
\begin{enumerate}
    \item case $s_2[y] = y$. We have $\varphi_1 \vdash f(u, t) \eq y$. From $(\varphi_1 \land x \eq y) \vdash v \eq f(u, t)$ and $\varphi_1 \vdash f(u, t) \eq y$, we have $(\varphi_1 \land x \eq y) \vdash v \eq y$. From Lemma~\ref{lm:Visenough}, we have $(\alpha_V(\varphi_1) \land x \eq y) \vdash v \eq y$. Since $\varphi_1 \vdash f(u, t) \eq y$, $\alpha_V(\varphi_1) \vdash f(u, w) \eq y$ by definition. Hence $(\alpha_V(\varphi_1) \land x \eq y) \vdash v \eq f(u, w)$.
    \item case $s_2[y] = g(b_1,\ldots,b_n)$ where $b_i$ is a superterm of $y$ for atleast one $i$. We have $\varphi_1 \vdash f(u, t) \eq g(b_1,\ldots,b_n)$. It is either the case that there exist a term $t'$ such that $g(b_1,\ldots, b_n) \eq t' \in \varphi_1$ and $\varphi_1 \vdash t' \eq f(u, t)$ or $g = f$ and $\varphi_1 \vdash\{u \eq b_1, t \eq b_2\}$. 
        \begin{enumerate}
            \item case there exist a term $t'$ such that $g(b_1,\ldots, b_n) \eq t' \in \varphi_1$ and $\varphi_1 \vdash t' \eq f(u, t)$. Since $g(b_1,\ldots, b_n) \in \terms(\varphi_1)$ and $V$ is a purifier for $y$ in $\varphi_1$, there should be a $y'\in V$ such that $\varphi_1 \vdash y' \eq g(b_1,\ldots,b_n)$. Therefore, $\varphi_1\vdash y' \eq f(u, t)$ and $(\varphi_1 \land x \eq y) \vdash v \eq y'$. By definition, $\alpha_V(\varphi_1) \vdash y' \eq f(u, w)$. By Lemma~\ref{lm:Visenough}, we have $(\alpha_V(\varphi_1) \land x \eq y) \vdash v \eq y'$. Hence $(\alpha_V(\varphi_1) \land x \eq y) \vdash v \eq f(u, w)$.
            \item case $g = f$ and $\varphi_1 \vdash\{u \eq b_1, t \eq b_2\}$. $s_1[x] \neq x$ \hg{why?}. It has to be the case that $s_1[x] = f(a_1, a_2)$. We have $\varphi_1 \vdash v \eq f(a_1, a_2)$ where $a_1$ or $a_2$ is a superterm of $x$. By Lemma~\ref{lm:trmingam}, we have a term $f(a_1', a_2') \in \terms(\varphi_1)$ s.t. $\varphi_1 \vdash \{v \eq f(a_1', a_2'), a_1' \eq a_1, a_2' \eq a_2\}$.  We case split on whether $a_1$ or $a_2$ is a superterm of $x$:
            \begin{enumerate}
                \item case $a_1$ is a superterm of $x$. We have $(\varphi_1 \land  x \eq y) \vdash a_1 \eq b_1$. Since $\varphi_1 \vdash a_1' \eq a_1$, $a_1' \in \terms(\varphi_1)$, and $V$ is a purifier for $x$ in $\varphi_1$, there must exists a constant $x' \in V$ s.t. $\varphi_1 \vdash x' \eq a_1'$. Since $(\varphi_1 \land  x \eq y) \vdash a_1 \eq b_1$, $(\varphi_1 \land x \eq y) \vdash x' \eq b_1$. From $\varphi_1 \vdash u \eq b_1$, we have $\varphi_1 \land x \eq y \vdash x' \eq u$. By Lemma~\ref{lm:Visenough}, we have $\alpha_V(\varphi_1) \land x \eq y \vdash x' \eq u$. Since $\varphi \wedge v \eq f(a_1', a_2')$ and $\varphi \wedge x' \eq a_1'$, we have $\varphi_1 \vdash v \eq f(x', a_2')$ and hence $\alpha(varphi_1) \vdash v \eq f(x', w)$ be definition. Since $\alpha(varphi_1) \vdash v \eq f(x', w)$ and $\alpha_V(\varphi_1) \land x \eq y \vdash x' \eq u$, $\alpha_V(\varphi_1) \land x \eq y \vdash v \eq f(u, w)$.
                \item case $a_2$ is a superterm of $x$. We have $(\varphi \land x \eq y) \vdash a_2 \eq b_2$. Since $\varphi_1 \vdash a_2' \eq a_2$, $a_2' \in \terms(\varphi_1)$, and $V$ is a purifier for $x$ in $\varphi_1$, there must exists a constant $x' \in V$ s.t. $\varphi_1 \vdash x' \eq a_2'$. Since $(\varphi_1 \land  x \eq y) \vdash a_2 \eq b_2$, $(\varphi_1 \land x \eq y) \vdash x' \eq b_2$. However, $\varphi \vdash b_2 \eq t$ and hence $(\varphi_1 \land x \eq y) \vdash t \eq x'$ which contradicts our assumption that there is no $v' \in V$ such that $(\varphi_1 \land x \eq y) \vdash v' \eq t$ .
            \end{enumerate}
        \end{enumerate}
\end{enumerate}
    
    %\alpha_V(\varphi_1 \wedge x \eq y) \vdash v \eq f(u_1, u_2)$ then $\alpha_V(\varphi_1) \land x \eq y \vdash v \eq 
    % \item case $\ell = v \eq f(u, w)$. $(\alpha_V(\varphi_1 \land x \eq y)) \vdash v \eq f(u, w)$ iff $(\varphi_1 \land x \eq y) \vdash v \eq f(u, t)$ for some term $t \not \in V$. 
    % %In this case, we have to ensure that $(\alpha_V(\varphi_1)\land x \eq y) \vdash v \eq f(u, w)$ for the same constant $w$. That is, if $\alpha_V(\varphi_1 \wedge x \eq y) \vdash v \eq f(u, w_1)$ and $\alpha_V(\varphi_1 \wedge x \eq y) \vdash v \eq f(u, w_2)$, then $\alpha_V(\varphi_1) \land x \eq y \vdash v \eq f(u, w_1)$ and $\alpha_V(\varphi_1) \land x \eq y \vdash v \eq f(u, w_2)$. and $\alpha_V(\varphi_1) \land x \eq y \not \vdash w_1 \eq w_2$. This is obviously true because $\varphi_1 \land x \eq y \not \vdash t_1 \eq t_2$ and $\alpha_V(\varphi_1)$.
    
    %\alpha_V(\varphi_1 \wedge x \eq y) \vdash v \eq f(u, w)$ then $\alpha_V(\varphi_1) \land x \eq y \vdash v
% \end{enumerate}

We have, for all $\ell \in L_{\eq} \cup L_{\deq} \cup L_{\funs}$, $\alpha_V(\varphi_1) \land x \eq y \vdash \ell$. Hence, $\alpha_V(\varphi_2) \land x \eq y \vdash \ell$ for all $\ell \in L_{\eq} \cup L_{\deq} \cup L_{\funs}$. Therefore, $\alpha_V(\varphi_1 \land x \eq y) = \alpha_V(\varphi_2 \land x \eq y)$.
\end{proof}
\begin{lemma}\label{lm:deqpres1v}
Let $V$ be a set of constants s.t. $x, y \in V$, $\varphi_1$ and $\varphi_2$ be two sets of literals s.t. $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$. Then, $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_2 \land x \deq y)$
\end{lemma}
\begin{proof}
Let $L = \{x \deq u \mid y \eq u \in \alpha_V(\varphi_1), u \in V\}$. By definition, $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_1) \land L$ as well as $\alpha_V(\varphi_2 \land x \deq y) = \alpha_V(\varphi_2) \land L$. Since $\alpha_V(\varphi_1) = \alpha_V(\varphi_2)$,  $\alpha_V(\varphi_1 \land x \deq y) = \alpha_V(\varphi_2 \land x \deq y)$.
 %Therefore, proving $\alpha_V(\varphi_1 \land x \deq y) \equiv_V \alpha_V(\varphi_2 \land x \deq y)$ is equivalent to proving $\alpha_V(\varphi_1) \land L \equiv_V \alpha_V(\varphi_2) \land L$ which follows from $\alpha_V(\varphi_1) \equiv_V \alpha_V(\varphi_2)$.
\end{proof}
%\sharon{moved $\alpha_q(\varphi)$ and $\consts(q)$ to earlier.}
%Let $q$ be an environment and $\consts(q) = \{c \mid \exists v \cdot q[v] = c\}$ be the
%set of all constants that represent current variable assignments in $q$.
For a state $q$, we write $\varphi \equiv_q \psi$ %and $\alpha_q(\varphi)$
for $\varphi \equiv_{\consts(q)} \psi$. %and $\alpha_{\consts(q)}(\varphi)$, respectively.

% Given a program configuration $\langle s, q, pc \rangle$, let $Q$ denote the set
% of constants in $q$:
% \[
% Q = \{ c \mid \exists \pv{v} \cdot q[\pv{v}] = c\}
% \]
% Let $\alpha_Q(\Gamma) = \beta$ where $\langle W, \beta, \delta\rangle = extbase(\Gamma, Q)$.



\begin{theorem}
  \label{thm:main}
  Let $\langle s, q, pc\rangle$ be a reachable configuration of a CUP\footnote{coherent
  uninterpreted program} $P$. Then,
\begin{enumerate}[(1)]
    \item $\langle s, q, pc\rangle \to \langle s', q', pc \land pc'\rangle$ iff\\
          $\langle s, q, \alpha_q(pc)\rangle \to \langle s', q', \alpha_{q}(pc) \land
          pc'\rangle$, and
    \item $\alpha_{q'}(pc \land pc') = \alpha_{q'}(\alpha_q(pc) \land pc')$.
\end{enumerate}
\end{theorem}
\begin{proof}
  Throughout the proof, we use $x = q[\pv{x}]$, and $y =
  q[\pv{y}]$.
%
  We only show the proof of part (1) for $s = \textbf{assume}(\pv{x} \bowtie
  \pv{y})$ since the other cases are trivial.
  
  The only-if direction follows since $\alpha_q(pc)$ is weaker than $pc$.
%
  For the if direction, $pc \not\vdash \bot$ since it is part of a reachable configuration. Then, there are two cases:
\begin{itemize}
  \item case $s = \textbf{assume}(\pv{x}=\pv{y})$. 
  Assume $(pc \land x \eq y) \models \bot$. Then, $(pc \land x \eq y) \vdash t_1 \eq t_2$ and $pc \vdash t_1 \deq t_2$ for some $t_1, t_2 \in \terms(pc)$. By Lemma~\ref{lm:sprtrm}, in
    any new equality $(t_1 \eq t_2)$ that is implied by $pc \land (x \eq y)$
    (but not by $pc$), $t_1$ and $t_2$ are equivalent (in $pc$) to superterms of
    $x$ or $y$. By the early assume property of CUP, $\consts(q)$ purifies $\{x,
    y\}$ in $pc$. Therefore, every superterm of $x$ or $y$ is equivalent (in
    $pc$) to some constant in $\consts(q)$. Thus,  $(pc \land x \eq y) \vdash u \eq v$ and $(pc \land x \eq y)  \vdash u \deq v$ for some $u, v \in \consts(q)$.
    By Lemma~\ref{lm:Visenough}, $(\alpha_q(pc) \land x \eq y) \vdash u \eq v$.
    By Lemma~\ref{lm:Visenoughdeq}, $(\alpha_q(pc) \land x \eq y) \vdash u \deq v$. Thus, $(\alpha_q(pc)\land x \eq y) \models \bot$.
  \item case $s = \textbf{assume}(\pv{x}\neq\pv{y})$. $(pc \land x \deq y)
    \models \bot$ if and only if $pc \vdash x \eq y$. Since $x, y \in \consts(q)$,
    $\alpha_q(pc) \vdash x \eq y$.
\end{itemize}

For part (2), we only show the cases for assume and assignment statements, the
other cases are trivial.
\begin{itemize}
\item case $s = \textbf{assume}(\pv{x} = \pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \eq y) = \alpha_{q}(\alpha_q(pc)
  \land x \eq y)$. From the early assumes property, $\const(q)$ 
  purifies $\{x, y\}$ in $pc$.
  By Lemma~\ref{lm:pur}, $\consts(q)$ purifies $\{x, y\}$ in $\alpha_q(pc)$ as well.
  By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  By Lemma~\ref{lm:eqpres1v}, $\alpha_q(pc \land x \eq y) = \alpha_q(\alpha_q(pc) \land x \eq y)$. 
  %\ag{NO CLUE WHAT THIS IS}
\item case $s = \textbf{assume}(\pv{x} \neq \pv{y})$, Since $q' = q$, we need to
  show that $\alpha_{q}(pc \land x \deq y) = \alpha_{q}(\alpha_q(pc)
  \land x \deq y)$. By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$. By Lemma~\ref{lm:deqpres1v},$\alpha_{q}(pc \land x \deq y) = \alpha_{q}(\alpha_q(pc)
  \land x \deq y)$.

\item case $s = \pv{x} \gets \pv{y}$. W.l.o.g., assume $q' = q[\pv{x}\mapsto
  x']$, for some constant $x' \not\in \const(pc)$. 
  %By Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$. 
  By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  By Lemma~\ref{lm:propequiv} (case~1), $\alpha_{\consts(q)
    \cup \{x'\}}(pc \land x' \eq y) = \alpha_{\consts(q)
    \cup \{x'\}}(\alpha_q(pc) \land x' \eq y)$. By Lemma~\ref{lm:subset}, $\alpha_{q'}(pc \land x' \eq y ) = \alpha_{q'}(\alpha_q(pc) \land x' \eq y)$,
  since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$.
\item case $s = \pv{x} \gets f(\Vec{y})$. W.l.o.g., $q' = q[\pv{x}\mapsto
  x']$ for some constant $x' \not\in \const(pc)$. There are two cases: (a) there
  is a term $t \in \terms(pc)$ s.t. $pc \vdash t \eq f(\Vec{y})$, (b) there is no
  such term $t$.
  \begin{enumerate}[label=(\alph*)]
  \item By the memoization property of CUP, there is a program variable $\pv{z}$
    s.t. $q[\pv{z}] = z$ and $pc \vdash z \eq f(\Vec{y})$. Therefore, by
    definition of $\alpha_q$, $\alpha_q(pc) \vdash z \eq f(\Vec{y})$. The rest
    of the proof is identical to the case of $s = \pv{x} \gets \pv{z}$.
  \item Since there is no term $t\in\terms(pc)$ s.t. $pc \vdash t \eq f(\Vec{y})$, $f(\Vec{y}) \not \in\terms(pc)$ as well as $f(\Vec{y}) \not \in \terms(\alpha_q(pc))$. By Lemma~\ref{lm:idem}, $\alpha_q(pc) = \alpha_q(\alpha_q(pc))$.
  %\hg{changed $pc^*$ to $pc$}\ag{What happens if the term in not in $\terms(pc)$ but there is an equivalent term. For example, say there is $f(z)$ somewhere in the $pc$ and $z \eq y$, which case is that?}\hg{this would be the first case as $pc \vdash f(z) \eq f(y)$. By memoization, since $f(z) \in \terms(pc)$, there has to be a variable in $q$ that stores $f(z)$.} and, therefore, not in
    %By Lemma~\ref{lm:betapreswequiv}, $pc \equiv^1_q \alpha_q(pc)$.
    %\ag{how is the jump to $q'$ justified}
    By Lemma~\ref{lm:propequiv} (case~2), $\alpha_{\const(q)\cup \{x'\}}(pc \land x \eq f(\Vec{y})) = \alpha_{\const(q)\cup \{x'\}}(\alpha_q(pc) \land x \eq f(\Vec{y}))$.
    By Lemma~\ref{lm:subset}, $\alpha_{q'}(pc \land x \eq f(\Vec{y}))
    = \alpha_{q'}(\alpha_q(pc) \land x \eq f(\Vec{y}))$ since $\consts(q') \subseteq (\consts(q) \cup \{x'\})$.
    \end{enumerate}
    \end{itemize}
\end{proof}

\hg{rough statements. Will refine later.}
\begin{corollary}
The relation $R = \{(c, \alpha(c))\}$ is a bisimulation relation for CUP.
\end{corollary}

\begin{corollary}
The relation $R = \{(c, \alpha_r(\alpha(c)))\}$ is a finite bisimulation relation for CUP.
\end{corollary}

==> sem-definitions.tex <==
\subsection{Programs}

We consider \emph{uninterpreted programs (UP)}, specified in the \emph{uninterpreted programming language (UPL)}.\sharon{is that the convention we want? it means that we will later write UP program or just UP? a bit strange. I won't change other occurrences until we decide}
The \emph{syntax} of programs in UPL is shown in \Cref{fig:syntax}.
Program variables are taken from a fixed set, denoted $\pvV$.
We use lower case letters in a special font: $\pvx$, $\pvy$, etc. to denote individual
variables in $\pvV$. We write $\Vec{\pvy}$ for a list of program variables.
Function symbols are taken from a fixed set $\funs$.
%
Following~\cite{DBLP:journals/pacmpl/MathurMV19}, while the language does not
allow for Boolean combination of conditionals nor relational symbols, these can
be modelled as described in~\cite{DBLP:journals/pacmpl/MathurMV19}.


%\ag{This paragraph needs TLC}
%We write $\pvV$ to denote a fixed set of all program variables, and lower case
%letters in a special font: $\pvx$, $\pvy$, etc. to denote individual
%variables in $\pvV$. We write $\Vec{\pvy}$ for a list of program variables.
%We assume that a program variable $\pvx$ is always initialized to a constant
%$x_0 \in \consts$ before the start of a program. Let $\vars_{\mathit{init}} =
%\{v_0 \mid \pvv \in \pvV\} \subseteq \consts$ be the set of constants to
%which program variables are initialized. We also assume that all function
%symbols in the program are in $\funs$.


\begin{figure}[t]
\begin{align*}
    \langle stmt \rangle ::=\; &\mathbf{skip} \mid \pvx \gets \pvx \mid \pvx \gets f(\Vec{\pvx}) \mid \\
               &\mathbf{assume}\;(\langle cond \rangle) \mid \langle stmt \rangle \mathbin{;} \langle stmt \rangle \mid \\
               &\mathbf{if}\;(\langle cond \rangle ) \;\mathbf{then} \;\langle stmt \rangle  \;\mathbf{else}\; \langle stmt \rangle \mid \\
               &\textbf{while}\;(\langle cond \rangle) \;\langle stmt \rangle\\
    \langle cond\rangle ::=\; &\langle var \rangle = \langle  var \rangle \mid \langle var  \rangle \neq \langle  var \rangle\\
  \langle var \rangle ::=\; & \pvx \mid \pvy \mid \cdots
\end{align*}
\caption{Syntax of the programming language UPL.}
\label{fig:syntax}
\end{figure}
%The \emph{syntax} of programs is shown in \Cref{fig:syntax}.
%Following~\cite{DBLP:journals/pacmpl/MathurMV19}, while the language does not
%allow for Boolean combination of conditionals nor relational symbols, these can
%be modelled as described in~\cite{DBLP:journals/pacmpl/MathurMV19}.


The small step symbolic operational semantics of UPL is defined by the rules
shown in Fig.~\ref{fig:ssesem}, with respect to a FOL signature $\Sigma = (\consts, \funs, \{\eq, \deq\})$.\sharon{should we re-arrange the rules to first display assume and assignments? these are the only "real" steps}
A program \emph{configuration} is a triple
$\langle s, q, pc \rangle$, where $s$ is a program in UPL to be executed, $q :
\pvV \to \consts$ is a \emph{state} mapping program variables to FOL
constants, and $pc$, called the \emph{path condition}, is a FOL\sharon{EUF?}\ag{We need to decide on EUF, I find it distracting, but maybe it is needed in some places} formula over
$\Sigma$.
%\sharon{why not restrict it to a conjunction of literals?
%(is it because if we apply cover we will no longer have a conjunction of literals?)
%When we define the abstraction we do assume that pc is a conjunction of literals.}
%\ag{Did not think of this}
%
We assume that every program variable $\pvx$ is initialized to a constant
$x_0 \in \consts$ before the start of a program. Let $\vars_{\mathit{init}} =
\{v_0 \mid \pvv \in \pvV\} \subseteq \consts$ be the set of constants to
which program variables are initialized.
%
For a state $q$, we write $q[\pvx \mapsto x']$ for a state $q'$ that
is identical to $q$, except that it maps $\pvx$ to $x'$. We write $\langle e,
q \rangle \Downarrow v$ to denote that $v$ is the value of the expression $e$ in state $q$, i.e.,
the result of substituting each program variable $\pv{x}$ in $e$ with
$q[\pv{x]}$, and replacing functions and predicates with their FOL counterparts.
%\sharon{
%as stated now, the program uses the same function symbols, so we only need to replace equality predicates by their counterparts.
%Do we want to maintain the distinction? or should we just overload these like functions?}
%\ag{We use different fonts for program variable vs logic variable and for program equiality vs logic equality, I wanted to highlight that difference}\sharon{I like the distinction. Except that we don't have it for function symbols. The nicer solution is probably to keep a similar distinction for function symbols. But let's leave it as is, no big deal. }
%In the case of an expression used in an assignment, $\langle e,
%q \rangle \Downarrow v$ is an FOL term, and in the case of a condition used in an assume statement,
%$\langle c, q \rangle \Downarrow v$ is an FOL formula.
The value of $e$ is an FOL term or an FOL formula over $\Sigma$.
For example, $\langle \pvx = \pvy, [\pvx \mapsto x, \pvy \mapsto y]
\rangle \Downarrow x \eq y$. Given two configurations $c$ and $c'$, we write $c
\to c'$ if $c$ reduces to $c'$ using one of the rules in Fig.~\ref{fig:ssesem}.
Note that there is no rule for $\textbf{skip}$ -- the program terminates once it gets into a configuration $\langle \textbf{skip}, q, pc\rangle$.

For a UPL program $P$, the operational semantics induces a transition system
$\TS_P = \tuple{\Conf,\initconf,\Tr}$, where $\Conf$ is the set of configurations
of $P$, $\initconf \eqdef \langle P, q_{\mathit{init}}, \top \rangle$ is the
initial configuration,
$q_{\mathit{init}} \eqdef \{\pvx \mapsto x_0 \mid \pvx \in \pvV\}$
%\sharon{removed $x_0 \in
%\consts$. It was defined earlier, and when adding this to the set def,
%it is interpreted as if we add \emph{all} the pairs regardless of
%the relation between them}
is the initial state, and $\Tr \eqdef \{(c, c') \mid c \to c'\}$.
A configuration $c$ of $P$ is \emph{reachable} if $c$ is reachable from
$\initconf$ in $\TS_P$.
%\sharon{do we need to define executions? complete executions?}
%\ag{We do not need them with current semantics and proofs}
%\hg{rough work, will refine later}
\begin{definition}[The verification problem for UPL programs]
Given a program $P$ in UPL, determine whether the configuration $\langle\textbf{skip}, q, pc\rangle$ is reachable in $P$.
\end{definition}
Our semantics of UPL differs in some respects from the one
in~\cite{DBLP:journals/pacmpl/MathurMV19}. First, we follow a more traditional
small-step operational semantics presentation, by providing semantics rules and
the corresponding transition system. However, this does not change the semantics
conceptually. More importantly, we ensure that the path condition remains
satisfiable in all reachable configurations (by only allowing an assume statement to execute when
it results in a satisfiable path condition). We believe this is a more natural
choice that is also consistent with what is typically used in other symbolic
semantics.

\renewcommand{\final}{\mathbf{skip}}
\begin{figure}
\centering
\begin{gather*}
\prftree{\langle \mathbf{skip}\mathbin{;}s, q, pc \rangle \to \langle s, q, pc \rangle}\\[1ex]
%
\prftree{\langle s_1, q, pc\rangle \to \langle s_1', q', pc'\rangle}%
{\langle s_1\mathbin{;}s_2, q, pc \rangle \to \langle s_1'\mathbin{;}s_2, q', pc' \rangle}\\[1ex]
%
\prftree{\langle c, q\rangle\Downarrow v\qquad}{(pc \land v) \not \models \bot}%
{\langle \mathbf{assume}(c), q, pc \rangle \to \langle \final, q, pc\wedge v\rangle}\\[1ex]
%
\prftree{\langle e, q\rangle \Downarrow v\qquad}{\text{$x' \in \consts(\Sigma)$ is fresh in $pc$}}{\langle \pvx \gets e, q, pc \rangle \to \langle\final, q[\pvx \mapsto x'], pc \land x' = v\rangle}\\[1ex]
%
\begin{aligned}
\langle \mathbf{if}\;(c)\;\mathbf{then}\;s_1\;\mathbf{else}\;s_2, q, pc \rangle &\to \langle \mathbf{assume}(c)\mathbin{;}s_1, q, pc\rangle\\[1ex]
\langle \mathbf{if}\;(c)\;\mathbf{then}\;s_1\;\mathbf{else}\;s_2, q, pc \rangle &\to \langle \mathbf{assume}(\neg c)\mathbin{;}s_2, q, pc\rangle
\end{aligned}\\[1ex]
\begin{multlined}
    \langle \mathbf{while}\;(c)\;s, q, pc \rangle \to{} \\ \qquad\qquad \langle \mathbf{if}\;(c)\;\mathbf{then}\;(s\mathbin{;} \mathbf{while}\;(c)\;s)\;\mathbf{else}\;\mathbf{skip}, q, pc \rangle
\end{multlined}
\end{gather*}
\caption{Small step symbolic operational semantics of UPL, where $\neg c$ denotes $\pvx \neq \pvy$ when $c$ is $\pvx = \pvy$, and
$\pvx = \pvy$ when $c$ is $\pvx \neq \pvy$.}
\label{fig:ssesem}
\end{figure}
%\ag{Using skip program as the final state.} \hg{The semantics have been changed to check assume condition before executing assume. In this case, all reachable configurations are feasible as well. This is not the assumption under which I wrote any of the sections.}
\iffalse
    \infer{\langle \mathbf{if}\;(c)\;\mathbf{then}\;s_1\;\mathbf{else}\;s_2, q, pc \rangle \Downarrow q', pc'}{\langle c, q\rangle \Downarrow v \quad \isSAT(pc \wedge v) \quad \langle s_1, q, pc \wedge v\rangle \Downarrow q', pc'}\\[1ex]
    \infer{\langle \mathbf{if}\;(c)\;\mathbf{then}\;s_1\;\mathbf{else}\;s_2, q, pc \rangle \Downarrow q', pc'}{\langle \neg c, q\rangle \Downarrow v \quad \isSAT(pc \wedge v) \quad \langle s_2, q, pc \wedge v\rangle \Downarrow q', pc'}\\[1ex]
    \infer{\langle \mathbf{while}\;(c)\;\{s\}, q, pc \rangle \Downarrow q', pc'}{\langle c, q\rangle \Downarrow v\quad \isSAT(pc \wedge v)\; \langle s;\mathbf{while}(c)\;\{s\}, q, pc \wedge v\rangle \Downarrow q', pc'}\\[1ex]
     \infer{\langle \mathbf{while}\;(c)\;\{s\}, q, pc \rangle \Downarrow q, pc \wedge v}{\langle \neg c, q\rangle \Downarrow v\quad \isSAT(pc \wedge v)}\\[1ex]
\fi

% An \emph{execution} of a program $P$ is a (possibly infinite) sequence starting
% from the configuration $\langle P, q_{init}, \top\rangle$ such that adjacent
% configurations satisfy the small step execution semantics, where $q_{init}$ maps
% all variables in $\vars$ to corresponding constants in $\vars_{init}$. An
% execution is \emph{complete} if it is either infinite or reaches a terminal
% configuration $\langle \mathbf{skip}, q, pc \rangle$ from which no more rules
% are applicable. A partial execution is a prefix of a complete execution. Since
% all executions are feasible, a configuration is \emph{reachable} in a program if
% it occurs in an execution of the program\footnote{Note that executions can be
%   infeasible in~\cite{DBLP:journals/pacmpl/MathurMV19}}. The \emph{terms} of an
% execution whose last configuration is $\langle s, q, pc \rangle$, is
% $\terms(pc)$, the set of all terms in the path condition $pc$.

% A term $t_1$ is equivalent to $t_2$ modulo condition $pc$ iff  $pc \models t_1 = t_2$. We write $t_1 \cong t_2$ whenever $pc$ is clear from the context. We say that $t_1$ is a superterm of $t_2$ modulo $pc$ iff there exists $t_1'$ such that $pc \models t_1' = t_1$ and $t_1'$ is a superterm of $t_2$.
% \begin{example}[The other definition is weaker]
% An alternate definition of superterm modulo could have been the following: we say that $t_1$ is a superterm of $t_2$ modulo $pc$ iff there exists $t_2'$ such that $pc \models t_2' = t_2$ and $t_1$ is a superterm of $t_2'$. However, this definition is strictly weaker. That is, there exists $t_1, t_2, pc$ such that $t_1$ is a superterm of $t_2$ modulo $pc$ according to our definition but not according to the alternate definition. $t_1 = f(y), t_2 = x, pc = f(x) = f(y)$. To satisfy our definition, we can pick $t_1'$ to be $f(x)$. However, we cannot choose a $t_2'$ to satisfy the alternate definition.\sharon{in the UP paper both $t_1$ and $t_2$ can be replaced by $t_1'$ and $t_2'$. This is showing that only one is needed }

% On the other hand, if we were able to satisfy the alternate definition, we should be able to satisfy our definition as well. Let $t_1 = f(\ldots, t_2',\ldots)$ and $pc \models t_2' = t_2$. According to the alternate definition, $t_1$ is a superterm of $t_2$. Let $t_1' = f(\ldots, t_2, \ldots)$. It holds that $pc \models t_1' = t_1$. Thus, $t_1$ is a superterm of $t_2$ modulo $pc$ according to our definition as well.
% \end{example}

\begin{definition}[Coherent Uninterpreted Program~\cite{DBLP:journals/pacmpl/MathurMV19}]
  \label{def:cup}%
A UPL program $P$ is \emph{coherent} (CUP for short) if all of the reachable
configurations of $P$ satisfy the following two properties:
\begin{description}[topsep=0pt,noitemsep]
\item[Memoizing] for any configuration $\langle \pvx \gets f(\Vec{\pvy}), q,
  pc \rangle$, if there is a term $t \in \terms(pc^*)$ s.t. $pc \models t
  \eq f(q[\Vec{\pvy}])$, then there is $\pvv \in \pvV$ s.t. $pc \models
  q[\pvv] \eq t$. That is, every assigned term  is either
  fresh, or is stored in some variable.
\item[Early assume] for any configuration\\\mbox{$\langle \mathbf{assume}(\pvx =
  \pvy), q, pc \rangle$}, if a term $t \in \terms(pc^*)$ is a superterm of
  $q[\pvx]$ or $q[\pvy]$, then, there is $\pvv \in \pvV$ s.t. $pc
  \models q[\pvv] \eq t$. That is, any superterm of a variable in an assumed
  equality is stored in some variable.
\end{description}
\end{definition}
\hg{The definition of coherence is not what it used to be. We (and the definition from the original paper) cared only about terms in the $pc$, not terms in $pc^*$.}\ag{This was my attempt to avoid talking about terms modulo $pc$. The original definition definitely cares about terms that are equivalent to a superterm, even if they are superterms themselves}
\hg{If $pc = x \eq y$, shouldn't $pc^*$ contain $f(x) \eq f(y), f(f(x))\eq f(f(y))$ etc? Seems to me like the early assumes property, as stated now, requires all of them to be stored in variables.} \ag{Hmm, good point. Then our definition of deductive closure is wrong. Same issue as reflexivity. If $pc = x \eq y$, then I want $pc^* = x \eq y$}

\sharon{I think we should comment about the diff compared to orig def:
since the path condition accumulates the entire history of the execution, we don't need to talk about executions}\ag{I did somewhere already, we can add more}\sharon{I saw you explained it about the semantics, but I thought that we can highlight it again for the def of coherence. Maybe it's not needed, not sure. But I really like that it is now stated as a "non-temporal" safety property (non-temporal in the sense that it is defined by a set of states, no need to talk about executions)}

\begin{example}
Consider the coherent program
\[
\begin{array}{ll}
1.&\mathbf{assume}(\pvx = \pvy);\\
2.&\pvx \gets f(\pvp, \pvx);\\
3.&\pvy \gets f(\pvq, \pvy);\\
4.&\mathbf{assume}(\pvp = \pvq);\\
5.&\mathbf{assume}(\pvx \neq \pvy)
\end{array}
\]

The symbolic state after each line of execution is \ag{Update to follow new
  semantics. Explain what $pc_i$ is. Explain why the program is coherent}
\[
\begin{array}{ll}
1.&\langle [\pvx: x_0,  \pvy: y_0, \pvp: p_0, \pvq: q_0], x_0 = y_0\rangle\\
2.&\langle [\pvx: x_1,  \pvy: y_0, \pvp: p_0, \pvq: q_0], pc_1 \land x_1 = f(p_0, x_0)\rangle\\
3.&\langle [\pvx: x_1,  \pvy: y_1, \pvp: p_0, \pvq: q_0], pc_2 \land y_1 = f(q_0, y_0)\rangle\\
4.&\langle q_3, pc_3 \land p_0 = q_0\rangle\\
5.&\langle q_3, pc_4 \land x_1 \neq y_1 \rangle
\end{array}
\]
\end{example}
% \hg{TODO: State it properly.}
% \begin{theorem}
% For a coherent program $P$, the following does not change semantics:
% \[
% \infer{\langle x:= f(y), q, pc\rangle \to \langle x:= z, q, pc\rangle}{\text{there exists a variable z such that } pc \vdash q[z] \eq f(q[y])}
% \]
% \end{theorem}


==> unaryequivalence.tex <==
\section{Invariants of the abstraction}
Let $\langle q, pc_1\rangle$ and $\langle q, pc_2\rangle$ be two program configurations. We say that $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$ if and only if
\begin{itemize}
    \item $pc_1 \models q[v] \eq t \iff pc_2 \models q[v] \eq t$
    \item $pc_1 \models q[v] \deq t \iff pc_2 \models q[v] \deq t$
\end{itemize}

where $v$ is any program variable and $t$ is any term over signature $\Sigma$.

\begin{lemma}\label{lm:eqprescoh}
If $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$ then for any statement $s$, $\langle s, q, pc_1\rangle$ satisfies both Early Assume and Memoizing property if and only if $\langle s, q, pc_2\rangle$ satisfies them as well.
\end{lemma}
\begin{proof}
Both properties require some term to be stored in a variable.
\end{proof}
\begin{lemma}\label{lm:sprtrmder}
If $\Gamma \wedge X \eq Y \models t_1 \eq t_2$ where $X, Y \in \terms(\Gamma)$, then either $\Gamma \models t_1 \eq t_2$ or $t_1, t_2$ are superterms of $X, Y$ modulo $\Gamma$ respectively. \hg{add $t_1$ can be superterm of $Y$ and $t_2$ can be a superterm of $X$.}
\end{lemma}
\begin{proof}
 Assume that $t_1$ is not a superterm of $X$ (or, equivalently $t_2$ is not a superterm of $Y$). We are going to prove that if $\Gamma \wedge X \eq Y \models t_1 \eq t_2$ then $\Gamma \models t_1 \eq t_2$. We do this by induction on the number of number of times the congruence axioms are used to derive $t_1 \eq t_2$. Clearly, if the axiom is not used then $\Gamma \models t_1 \eq t_2$. Inductive case: assume that $t_1 = f(u_1, \ldots, u_n)$ and $t_2 = f(v_1, \ldots, v_n)$ such that none of the $u_i$'s are superterms of $X$ modulo $\Gamma$ and $\Gamma \models u_i \eq v_i$. Clearly, $\Gamma \models f(u_1,\ldots,u_n) \eq f(v_1,\ldots, v_n)$. 
\end{proof}

\begin{lemma}\label{lm:frshcnst}
If $\Gamma \wedge X \eq t \models \ell$ where $\ell$ is ground and $X \not\in \terms(\Gamma)$, then \begin{itemize}
    \item if $X \not\in\terms(\ell)$ then $\Gamma \models \ell$
    \item else $\Gamma \models \ell[X \mapsto t]$ where $\mapsto$ is syntactic substitution of all occurrences of $X$ with $t$
\end{itemize}
\end{lemma}


\begin{lemma}\label{lm:sprtrmdeqder}
If $\Gamma \wedge X \deq Y \models t_1 \deq t_2$ where $X, Y \in \terms(\Gamma)$, then either $\Gamma \models t_1 \deq t_2$ or both $\Gamma \models X \eq t_1$ and $\Gamma \models Y \eq t_2$.
\hg{add $t_1 \eq Y$ and $t_2 \eq X$.}
\end{lemma}

\begin{lemma}\label{lm:sprtrmdeqeqqder}
If $\Gamma \wedge X \eq Y \models t_1 \deq t_2$ where $X, Y \in \terms(\Gamma)$, then either $\Gamma \models t_1 \deq t_2$ or both $\Gamma \models X \deq t_1$ and $\Gamma \models Y \eq t_2$.
\hg{or $\Gamma \models Y \deq t_1$ and $\Gamma \models X \eq t_2$}
\end{lemma}

\begin{lemma}\label{lm:sprtrmcls}
Let $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$ such that, for all superterms $t_x$ of $x$, there exists variable $v$ such that $pc_1 \models t_x \eq q[v]$ if and only if $pc_2 \models t_x \eq q[v]$. 
Then $t$ is a superterm of $q[x]$ modulo $pc_1$ if and only if $t$ is a superterm of $q[x]$ modulo $pc_2$.
\end{lemma}
\begin{proof}
Proof relies only on the transitivity property. If direction: It has to be the case that $pc_1 \models t \eq t_x$. Therefore, $pc_1 \models q[v] \eq t$. Hence $pc_2 \models q[v] \eq t$ and, by assumption, $pc_2 \models q[v] \eq t_x$. Therefore $pc_2 \models t_x \eq t$.
\end{proof}
\begin{theorem}
Let $P$ be a coherent program and let $\langle q, pc_1 \rangle$ be a reachable configuration in $P$.
If $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$, $\langle s, q, pc_1\rangle \rightarrow \langle s', q', pc_1'\rangle$, and $\langle s, q, pc_2\rangle \rightarrow \langle s', q', pc_2'\rangle$, then $\langle q', pc_1'\rangle \pceq \langle q', pc_2'\rangle$
\end{theorem}
\begin{proof}
By lemma~\ref{lm:eqprescoh}, both configurations are coherent. We only have to prove the theorem for the rules for assume and assignment statement.
\begin{itemize}
    \item assume$(x = y)$: By early assume property and lemmas~\ref{lm:sprtrmcls},~\ref{lm:sprtrmder}, $pc_1' \models q[v] \eq t \iff pc_2' \models q[v] \eq t$. Lemma~\ref{lm:sprtrmdeqeqqder} shows that exactly the same inequalities are produced.
    \item assume$(x\neq y)$. No new equalities are produced, therefore, $pc_1' \models q[v] \eq t \iff pc_2' \models q[v] \eq t$. By lemma~\ref{lm:sprtrmdeqder}, $pc_1' \models q[v] \deq t \iff pc_2' \models q[v] \deq t$.
    \item $x := e$: Let $\langle e, q\rangle \Downarrow t_e$, $q' = q[x \mapsto X]$. We have to show that $pc_1 \wedge X \eq t_e \models q'[v]\eq t$ if and only if $pc_2 \wedge X \eq t_e \models q'[v] \eq t$. We prove the if direction.
    \begin{itemize}
        \item if $v$ is not the variable $x$. $q[v] = q'[v]$. Consider the two cases in lemma~\ref{lm:frshcnst}. If $t$ does not contain $X$, the proof is trivial. Otherwise, $pc_1 \models  q'[v] \eq t[X \mapsto t_e]$. By our assumption $pc_2 \models q'[v] \eq t[X \mapsto t_e]$. Hence $X = t_e \wedge pc_2 \models q'[v] \eq t$.
        \item if $v = x$. If $pc_1 \wedge X \eq t_e \models q[x] \eq t$, it has to be the case that $pc_1 \models t_e \eq t$. By memoization property, there has to be a variable $u$ such that $pc_1 \models q[u] \eq t_e$ and therefore $pc_1 \models q[u] \eq t$. Hence $pc_2 \models q[u] \eq t \wedge q[u] \eq t_e$, therefore, $pc_2 \models t_e \eq t$. Hence $pc_2 \wedge X = t_e \models q[x] \eq t$. The same argument can be used to show that if $pc_1 \wedge X \eq t_e \models q[x] \deq t$ then $pc_2 \wedge X \eq t_e \models q[x] \deq t$ as well.
    \end{itemize}
\end{itemize}
\end{proof}
Throughout the rest of this section, we assume that all non-constant function symbols the signature $\Sigma$ are unary. 
Given a program configuration $\langle q, pc \rangle$, let $S_q$ denote the set of constants in $q$: 
\[
S_q = \{ c \mid \exists v \cdot q[v] = c\}
\]
\begin{theorem}
Let $P$ be a coherent program. Let $\langle s, q, pc\rangle$ be a reachable configuration in $P$. Then $\langle q, pc\rangle \pceq \langle q, \alpha^1_{S_q}(pc)\rangle$
\end{theorem}

\begin{theorem}
Let $P$ be a coherent program. Let $\langle s, q, pc\rangle$ be a reachable configuration in $P$. Then $\langle q, pc\rangle \pceq \langle q, \alpha^2_{S_q}(pc)\rangle$
\end{theorem}

==> unaryequivalence2.tex <==
\section{Invariants of the abstraction}
Throughout this section, we assume that all non-constant function symbols in the signature $\Sigma$ are unary. 

Lemmas~\ref{lm:sprtrm} to \ref{lm:frshcnst} outline important properties of EUF that are useful in our proofs. \hg{talk about symmetry} Lemma~\ref{lm:sprtrm} states that introducing an equality between two constants only affects their superterms. 
\begin{lemma}\label{lm:sprtrm}
Let $\Gamma$ be a set of literals, $a, b$ be constants in $\Gamma$. Let $t_1, t_2$ be terms constructed using signature $\Sigma$ such that $\Gamma \not\vdash t_1 \eq t_2$. Then $\Gamma \wedge a \eq b \vdash t_1 \eq t_2$ if and only if $\Gamma \vdash t_1 \eq f^k(a)$ and $\Gamma \vdash t_2 \eq f^k(b)$, $k \geq 0$.
\end{lemma}
The following lemma specialises lemma~\ref{lm:sprtrm} to the case of constants and function applied to constants:
\begin{lemma}\label{lm:sprtrm2}
Let $\Gamma$ be a set of literals, $a, b$ be constants in $\Gamma$. Let $u, v$ be constants in $\Gamma$ such that $\Gamma \not\vdash v \eq f(u)$. Then $\Gamma \wedge a \eq b \vdash v \eq f(u)$ if and only if $\Gamma \vdash v \eq f^k(a)$ and $\Gamma \vdash u \eq f^{k - 1}(b)$, $k \geq 1$.
\end{lemma}
Let $V$ be a set of constants. We denote by $V^1$ the set of terms obtained by applying function symbols atmost once on the constants in $V$:
\[
V^1 = \{f(c) \mid c \in V\} \cup V
\]
We denote by $\Gamma^{V}$ the set 
\[
\{v \eq t \in \Gamma^* \mid t \in V^1, v \in V\} \cup \{ v\deq u \in \Gamma^* \mid u, v \in V\}
\]

\hg{TODO: come up with a better name than represents. Something that says all superterms have representatives in this set.}
We say that a set of constants $V$ \emph{represents} a constant $a$, in a set of literals $\Gamma$ if, $a \in V$ and for every term $f^k(a) \in \terms(\Gamma)$~($k \geq 1$), there exists $v \in V$ such that $\Gamma \vdash v \eq f^k(a)$. It follows that there exists a variable $u \in V$ such that $\Gamma \vdash u \eq f^{k - 1}(a)$ and that $\Gamma \vdash v \eq  f(u)$. Moreover, if $k \geq 2$, there exists a constant $u' \in V$ such that $\Gamma \vdash u' \eq f^{k - 2}(a)$ and so on.
\begin{example}
Let $\Gamma = \{ c \eq f(a), d \eq f(b), d \deq e\}$. The set of constants $V_1 = \{a, b, c\}$ is represents $a$ but not $b$.
\end{example}
\begin{lemma}\label{lm:Visenough}
Let $\Gamma$ be a set of literals and $a, b$ be constants in $\Gamma$. Let $V$ be a set of constants that represents both $a, b$ in $\Gamma$. If
\[
\Gamma \wedge a \eq b \vdash v \eq u
\]
then
\[
\Gamma^V \wedge a \eq b \vdash v \eq u
\]
where $u, v \in V$.
\end{lemma}
\begin{proof}
By the definition of $\Gamma^V$, if $\Gamma \vdash v \eq u$ then $\Gamma^V \vdash v \eq u$. 

If $\Gamma \not \vdash v \eq u$, according to lemma~\ref{lm:sprtrm}, $\Gamma \vdash v \eq f^k(a)$ and $\Gamma \vdash u \eq f^k(b)$. 
We do induction on $k$. If $k = 0$ the lemma holds by the definition of $\Gamma^V$.

For the inductive step, we have $\Gamma \wedge a \eq b \vdash v \eq u$ where $\Gamma \vdash v \eq f^k(a)$ and $\Gamma \vdash u \eq f^k(b)$. Assume that the lemma holds for some $k - 1$. That is, for every $u', v' \in V$, if $\Gamma \vdash v' \eq f^{k - 1}(a)$, $\Gamma \vdash u' \eq f^{k - 1}(b)$ then $\Gamma^V \wedge a \eq b \vdash v' \eq u'$.

Since $V$ represents both $a, b$ in $\Gamma$, we have $\Gamma \vdash v \eq f(v'')$ and $\Gamma \vdash u \eq f(u'')$ for some $u'', v'' \in V$. Therefore, $\Gamma^V \vdash v \eq f(v'')$ and $\Gamma^V \vdash u \eq f(u'')$. By the inductive assumption, we have $\Gamma^V \wedge a \eq b\vdash u'' \eq v''$. By applying congruence axiom, we have $\Gamma^V \wedge a \eq b \vdash v \eq u$.
\end{proof}
\begin{lemma}\label{lm:Visenough2}
Let $\Gamma$ be a set of literals and $a, b$ be constants in $\Gamma$. Let $V$ be a set of constants that represents both $a, b$ in $\Gamma$. If
\[
\Gamma \wedge a \eq b \vdash v \eq f(u)
\]
then
\[
\Gamma^V \wedge a \eq b \vdash v \eq f(u)
\]
where $u, v \in V$.
\end{lemma}
\begin{proof}
By the definition of $\Gamma^V$, if $\Gamma \vdash v \eq f(u)$ then $\Gamma^V_{\{a, b\}} \vdash v \eq f(u)$. 
Now, according to lemma~\ref{lm:sprtrm2}, $\Gamma \vdash v \eq f^k(a)$ and $\Gamma \vdash u \eq f^{k - 1}(b)$. 
Since $V$ represents $a$ in $\Gamma$, there exists a constant $v' \in V$ such that $\Gamma \vdash v \eq f(v')$ and $\Gamma \vdash v' \eq f^{k -1}(a)$. By the definition of $\Gamma^V$, we have $\Gamma^V \vdash v \eq f(v')$. By lemma~\ref{lm:Visenough}, we have $\Gamma^V \wedge a \eq b \vdash v' \eq u$. Therefore, $\Gamma^V\wedge a \eq b \vdash v \eq f(u)$. 
\end{proof}

\begin{lemma}\label{lm:Visenoughdeq}
Let $\Gamma$ be a set of literals and $a, b$ be constants in $\Gamma$. Let $V$ be a set of constants that represents both $a, b$ in $\Gamma$. If
\[
\Gamma \wedge a \eq b \vdash v \deq u
\]
then
\[
\Gamma^V \wedge a \eq b \vdash v \deq u
\]
where $u, v \in V$.
\end{lemma}
\begin{proof}
By the definition of $\Gamma^V$, if $\Gamma \vdash v \deq u$ then $\Gamma^V \vdash v \deq u$. If $\Gamma \not \vdash v \deq u$, it has to be the case that there is a term $t$ over the signature $\Sigma$ such that $\Gamma \vdash t \deq u$ and $\Gamma \wedge a \eq b \vdash v \eq t$. According to lemma~\ref{lm:sprtrm}, we have $\Gamma \vdash v \eq f^k(a)$ and $\Gamma \vdash t \eq f^k(b)$. \hg{justify why $f^k(b)\in \terms(\Gamma)$} Since $V$ represents $b$, there exists $u' \in V$ such that $\Gamma \vdash u' \eq f^k(b)$. Therefore, $\Gamma \wedge a \eq b \vdash v \eq u'$ and $\Gamma \vdash u' \deq u$. By the definition of $\Gamma^V$, we have $\Gamma^V \vdash u' \deq u$ and, according to lemma~\ref{lm:Visenough}, we have $\Gamma^V \wedge a \eq b \vdash v \eq u'$. Hence $\Gamma^V \wedge a \eq b \vdash v \deq u$.
\end{proof}

\begin{lemma}\label{lm:Visenoughdeq2}
Let $\Gamma$ be a set of literals. Let $V$ be a set of constants including $a, b$. If
\[
\Gamma \wedge a \deq b \vdash v \deq u
\]
then
\[
\Gamma^V \wedge a \deq b \vdash v \deq u
\]
where $u, v \in V$.
\end{lemma}
\begin{proof}
By the definition of $\Gamma^V$, if $\Gamma \vdash v \deq u$ then $\Gamma^V \vdash v \deq u$. If$\Gamma \not\vdash v \deq u$ and $\Gamma \wedge a \deq b \vdash v \deq u$, it has to be case that $\Gamma \vdash v \eq a$ and $\Gamma \vdash u \eq b$. Therefore, $\Gamma^V \vdash v \eq a$ as well as $\Gamma^V \vdash u \eq b$. Therefore $\Gamma^V \wedge a \deq b \vdash v \deq u$. 
\end{proof}

\begin{lemma}\label{lm:frshcnst}
If $\Gamma \wedge v \eq t \vdash \ell$ where $\ell$ is ground, $v$ is a fresh constant: $v \not\in \terms(\Gamma) \cup \terms(t)$, then \begin{itemize}
    \item if $v \not\in\terms(\ell)$ then $\Gamma \vdash \ell$
    \item if $\ell = v \circ t_2$, then $\Gamma \vdash t \circ t_2$, $\circ \in \{\eq, \deq\}$
    \item else $\Gamma \vdash \ell[v \mapsto t]$ where $v \mapsto t$ is syntactic substitution of all occurrences of $v$ with $t$
\end{itemize}
\end{lemma}

Given a program configuration $\langle q, pc \rangle$, let $Q$ denote the set of constants in $q$: 
\[
Q = \{ c \mid \exists \pv{v} \cdot q[\pv{v}] = c\}
\]
Let $Q^1 = \{f(c) \mid c \in Q\} \cup Q$.

Let $\langle q, pc_1\rangle$ and $\langle q, pc_2\rangle$ be two program configurations. We say that $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$ if
\begin{itemize}
    \item $pc_1 \vdash q[v] \eq t$ if and only if $pc_2 \vdash q[v] \eq t$ for any $t \in Q^1$
    \item $pc_1 \vdash q[v] \deq t$ if and only if $pc_2 \vdash q[v] \deq t$ for any $t \in Q$
\end{itemize}
where $v$ is any program variable.

\begin{lemma}\label{lm:pceqprop}
Let $\langle q, pc_1\rangle$ and $\langle q, pc_2\rangle$ be two program configurations such that $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$. 
\begin{itemize}
    \item $pc_1^Q \subseteq pc_2$ and $pc_2^Q \subseteq pc_1$.
    \item $Q$ represents $v$ in $pc_1$ if and only if $Q$ represents $v$ in $pc_2$, for any constant $v$.
\end{itemize}
\end{lemma}


\begin{theorem}
Let $P$ be a coherent program and let $\langle q, pc_1 \rangle$ be a reachable configuration in $P$.
If $\langle q, pc_1\rangle \pceq \langle q, pc_2\rangle$, $\langle s, q, pc_1\rangle \rightarrow \langle s', q', pc_1'\rangle$, and $\langle s, q, pc_2\rangle \rightarrow \langle s', q', pc_2'\rangle$, then $\langle q', pc_1'\rangle \pceq \langle q', pc_2'\rangle$
\end{theorem}
\begin{proof} We only have to prove the theorem for the rules for assume and assignment statement.
\begin{itemize}
    \item \textbf{assume}$(\pv{x}=\pv{y})$: Let $q[\pv{x}] = x, q[\pv{y}] = y$. By early assume property, $Q$ \emph{represents} $x, y$ in $pc_1$. By lemma~\ref{lm:Visenough}~and~\ref{lm:Visenough2}, we have, if $pc_1 \wedge x \eq y \vdash q[\pv{v}] \eq t$ then $pc_1^Q \wedge x \eq y \vdash q[\pv{v}] \eq t$ for any $t \in Q^1$. By lemma~\ref{lm:pceqprop}, $pc_1^Q \subseteq pc_2$. Therefore, $pc_2 \wedge x \eq y \vdash q[\pv{v}] \eq t$ as well.  The other direction can be established using the same lemmas.
    For the inequalities, we can apply lemma~\ref{lm:Visenoughdeq}.
    \item \textbf{assume}$(\pv{x}\neq\pv{y})$: Let $q[\pv{x}] = x, q[\pv{y}] = y$. Then $pc_1' = pc_1 \wedge x \deq y$ and $pc_2' = pc_2 \wedge x \deq y$. The equality relation $pc_1' \vdash q[\pv{v}] \eq t$ if and only if $pc_2' \vdash q[\pv{v}] \eq t$ for any $t \in Q^1$, holds because no new equalities are introduced because of the new inequality. We can apply lemma~\ref{lm:Visenoughdeq2} to show that $pc_1' \vdash q[\pv{v}] \deq t$ if and only if $pc_2' \vdash q[\pv{v}] \deq t$ for any $t \in Q$
    \item $\pv{x} := \pv{y}$: Let $q[\pv{y}] = y$, $q' = q[\pv{x} \mapsto x]$, $x$ is fresh.  We have to show that $pc_1 \wedge x \eq y \vdash q'[\pv{v}]\eq t$ if and only if $pc_2 \wedge x \eq y \vdash q'[\pv{v}] \eq t$, $t \in (Q')^1$. We prove the if direction. The other direction follows from symmetry.
    \begin{itemize}
        \item if $\pv{v}$ is not the variable $\pv{x}$. $q[\pv{v}] = q'[\pv{v}]$. Consider the first and third cases in lemma~\ref{lm:frshcnst}. If $t$ does not contain $x$, the proof is trivial. Otherwise, $pc_1 \vdash  q'[\pv{v}] \eq t[x \mapsto y]$. By our assumption $pc_2 \vdash q'[\pv{v}] \eq t[x \mapsto y]$ as well. Hence $pc_2 \wedge x \eq y\vdash q'[\pv{v}] \eq t$.
        \item if $\pv{v} = \pv{x}$. $q'[\pv{x}] = x$. If $pc_1 \wedge x \eq y \vdash x \eq t$, it has to be the case that $pc_1 \vdash y \eq t$. Therefore, $pc_2 \vdash y \eq t$. Hence $pc_2 \wedge x \eq y \vdash x \eq t$.
    \end{itemize}
    \item $\pv{x} := \pv{f(y)}$: Let $q[\pv{y}] = y$, $q' = q[\pv{x} \mapsto x]$. Assume that $pc_1 \wedge x \eq f(y) \vdash z \eq t$ where $z \in Q'$ and $t \in (Q')^1$. We need to prove that $pc_2 \wedge x \eq f(y) \vdash z \eq t$. We split based on whether $f(y) \in \terms(pc_1)$.
    \begin{itemize}
        \item $f(y) \not \in \terms(pc_1)$. The only possibility for $t$ is $f(u)$ where $u \in Q'$ and $pc_1 \vdash y \eq u$. Since $x$ is fresh in $pc_1$, $u \neq x$. In this case $pc_2 \vdash y \eq u$ as well. If $z \neq x$, we are in case 1 of lemma~\ref{lm:frshcnst} and the proof holds trivially. If $z = x$ then, $pc_1 \vdash f(y) \eq f(u)$. Since $pc_2 \vdash y \eq u$, $pc_2 \vdash f(y) \eq f(u)$. Hence, by case 2 of lemma~\ref{lm:frshcnst} $pc_2 \wedge x \eq f(y) \vdash x \eq f(u)$ as well.
        \item $f(y) \in \terms(pc_1)$. Because of memoization $pc_1 \vdash u \eq f(y)$ for some $u \in Q$. Therefore, this is just like $pc_1 \wedge x \eq u$.
    \end{itemize}
    \hg{rewrite}
\end{itemize}
\end{proof}

The theorem only works when $\langle s, q, pc\rangle$ satisfies both memoization and early assumes property. 
\begin{theorem}
Let $P$ be a coherent program. Let $\langle s, q, pc\rangle$ be a reachable configuration in $P$. Then $\langle q, pc\rangle \pceq \langle q, \alpha^1_{S_q}(pc)\rangle$
\end{theorem}

\begin{theorem}
Let $P$ be a coherent program. Let $\langle s, q, pc\rangle$ be a reachable configuration in $P$. Then $\langle q, pc\rangle \pceq \langle q, \alpha^2_{S_q}(pc)\rangle$
\end{theorem}\textbf{}
